An Algorithmic Framework for Approximating Maximin Share Allocation of Chores

In this paper, we consider the problem of how to fairly dividing $m$ indivisible chores among $n$ agents. The fairness measure we considered here is the maximin share. The previous best known result is that there always exists a $\frac{4}{3}$ approximation maximin share allocation. With a novel algorithm, we can always find a $\frac{11}{9}$ approximation maximin share allocation for any instances. We also discuss how to improve the efficiency of the algorithm and its connection to the job scheduling problem.

==> EC 21 submission/alg_frame.tex <==
In this section, we present a general algorithm framework for dividing chores. The algorithmic framework is building on a reduction and a heuristic. The reduction is from the work~\cite{bouveret2016characterizing}, which allows  us to focus on IDO instances. 
%The algorithmic framework has two parts. In the first part, we show how to reduce general instances to IDO instances, which is from the work~\cite{bouveret2016characterizing}. 
Then, we demonstrate a heuristic  for IDO instances, which is similar to  First Fit Decreasing algorithm for bin packing problem~\cite{johnson1973near}.
%that is useful to find a proper approximation of \mmax~allocation for chores. This strategy shares some similarity with First Fit Decreasing algorithm for bin packing problem~\cite{johnson1973near}.



%\subsection{Reduction from general to identical ordinary preference}\label{sec-reduce}
%In this section, we formally state a reduction technique which is introduced by Bouveret and Lema{\^\i}tre~\cite{bouveret2016characterizing}. By this reduction, we only need to take care of instances such that all agents share the same ordinary preferences.
%And this technique has been successfully applied in the work \cite{barman2017approximation} to simplify the proof of approximation of maximin share allocation for goods.



The reduction from general instances to IDO instances is captured by the following lemma. The original statement is for goods.  As the setting of chores  is slightly different from goods, we give a full detail in Appendix \ref{apd-sec-reduce} for the completeness.

\begin{lemma}\label{lem-general}
Suppose that there is an algorithm $G$  running in $T(n,m)$ time and returning an \amMS{\alpha} allocation for all identical ordinary preference instances. Then, we have an algorithm running in time $T(n,m)+O(nm\log m)$ outputting an \amMS{\alpha} allocation for all instances.
\end{lemma}

%Please refer Appendix \ref{apd-sec-reduce} for detail.




%%%%%%%%%%%%
%%%%%%%%%%%%
%%%%%%%%%%%%




%\subsection{Algorithm for identical ordinary preference}\label{sec-ido-alg}
With the above reduction, we can focus on the identical ordinary preference. We introduce a heuristic which is a key part of our approximation algorithm.
%In this section, we demonstrate an algorithmic framework for approximating \mmax allocation.
The high level idea is that we setup a threshold for each agent, and then allocate large chores first and allocate them as much as possible with respect to the threshold.
%\xin{Add explanation for algortihm}

\begin{algorithm}[H]
\KwIn{An IDO instance $\inst$, threshold values of agents $(\alpha_1,\dots,\alpha_n)$}
\KwOut{An allocation $\allocs$}
\BlankLine
	%Suppose the \mmax of each agent is 1\;
	Let $R=\items$ and $T=\agents$ and $\allocs=(\emptyset,\dots,\emptyset)$\;
	\For(\tcp*[f]{Loop to generate bundles}\label{inalg-loop}){$k=1$ \KwTo $n$}
	{
		$\alloc=\emptyset$\;
		\For(\tcp*[f]{From the largest chore to the smallest}){ $j=1$ \KwTo  $|R|$}
		{
			\If{$\exists i\in T, \vai{\alloc\cup R[j]}\le \alpha_i$}
			{
				$\alloc=\alloc\cup R[j]$\;% and $R=R\setminus R[j]$\;
			}	
		}
		$R=R\setminus \alloc$\;
		Let $i\in T$ be an agent  such that $\vai{\alloc}\le\alpha_i$\;\label{inalg-select}
		$\alloci=\alloc$ and $T=T\setminus i$\;
	}
	\Return {$\allocs$}
\caption{Algorithm for \amMS{\alpha}}\label{alg-approx}	
\end{algorithm}

For this algorithm we have the following observation.

\begin{lemma}\label{lem-not-left}
Suppose that the inequality $\alpha_i\le\alpha\cdot\mMSi$ holds for each $i$. If all chores are allocated by the algorithm, then the allocation returned by Algorithm \ref{alg-approx} is an \amMS{\alpha} allocation.
\end{lemma}

To analyze the algorithm, we only need to focus on what threshold values $(\alpha_1,\dots,\alpha_n)$ will make the algorithm allocate all chores.








==> EC 21 submission/discussion.tex <==
%\xin{1. Discuss our framework and FFD algorithm.  2. Mention there is a gap between upper and lower bound. 3. How to covert the existence result to an algorithm.} 

At the first glance, our algorithm is quite similar to FFD algorithm for the bin packing problem. However, technically they are two different problems. 1) The bin packing problem is fixing the size of each bin and then try to minimize the number of bins. Our problem can be viewed as fixing the number of bins but try to minimize the size of each bin. 2) The optimal approximation of FFD algorithm for the bin packing problem is $\frac{11}{9}\cdot OPT+\frac{6}{9}$. To the best of our knowledge, there is no reduction between the approximation ratio of these two problems.  3) The lower bound Example \ref{exm-lower-bound}  does not make sense to the bin packing problem, and the lower bound example of bin packing problem does not make sense to our problem. 

%There is a gap of the lower and upper bound for the algorithmic framework in our analysis. We believe that the algorithmic framework can do better than 11/9 in approximating  \mmax~allocation for chores. We have tried to push this ratio a step further. It looks very plausible that the true power of the algorithmic framework is better than we have proven. However, along the idea of our current proof, the complexity of case analysis makes us unable to give a complete proof for it. So we leave the best approximation ratio of the algorithmic framework as an open problem for further study. 

For the analysis of our algorithmic framework, there is a gap between the lower and the upper bound of the approximation ratio. It will be interesting to close this gap. 
Another interesting direction is that how to convert the existence result from our algorithmic framework into an efficient algorithm. Suppose that $\alpha$ is the best approximation ratio of existence of our algorithmic framework. By combining a PTAS for job scheduling ~\cite{alon1998approximation}, we can have a PTAS for $\alpha+\epsilon$ approximation of \mmax~allocation. Nevertheless, such PTAS can hardly to be considered as efficient in practical use.  In section \ref{sec-poly}, we show one way to get a polynomial time algorithm for 5/4 approximation from our existence result. It is still possible to design an efficient algorithm for  $\alpha$-approximation.   %It will be cool if we can get an efficient algorithm for a better approximation ratio.  %It is possible to do better. The idea of getting a reasonable lower bound instead of an accuracy \mmax~could be reused to design efficient algorithm.% It will be best to have a general method to get an efficient algorithm for $\alpha$ approximation of \mmax~allocation whenever the algorithmic framework can show the existence of $\alpha$ approximation of \mmax~allocation. 
%We need to mention that the non-monotonicity of the algorithmic framework (Example \ref{exm-no-monoton}) would prevent some easy trials on this direction.

In section \ref{sec-special}, we try to explore the power of our algorithmic framework on the job scheduling problem.   It may worth to exploring more on the relationship of the algorithmic framework with other scheduling problems. %As we notice that, our Algorithm \ref{alg-approx} is similar to First Fit Decreasing algorithm for bin packing problem. It is possible to connect these problems together. 

==> EC 21 submission/existence.tex <==
In this section, we show that an $\frac{11}{9}$-approximation \mmax~allocation always exists by our algorithmic framework. %by verifying that Algorithm \ref{alg-approx} indeed allocates all the chores. 
%This is done by a careful comparison between the algorithm's allocation and the \mmax~allocation.   
To achieve this goal, it is sufficient to consider IDO instances solely (see Lemma \ref{lem-general}). For simplicity, we only deal with IDO instances for all proofs in this section.

%This improves previous best result of $\frac{4}{3}$ approximation~\cite{barman2017approximation}.  %By the discussion in section \ref{sec-frame}, we only need to show that, for all IDO instances, on input threshold value  $\frac{11}{9}\cdot\mMSi$ to Algorithm \ref{alg-approx}, all chores will be allocated. %Then by Lemma \ref{lem-not-left}, the conclusion is easily implied.
% From the existence result, we can obtain a PTAS for $\frac{11}{9}+\epsilon$ approximation. After exploring  the limitation of our technique, we construct an example to show that $\frac{20}{17}$ is a lower bound of our algorithmic framework.


\begin{theorem}\label{thm-exist}
For any chore division instance $\inst$, there always exists an \amMS{\frac{11}{9}} allocation.
\end{theorem}

By Lemma \ref{lem-not-left}, it is sufficient to prove that on inputting threshold value $\alpha_i=\frac{11}{9}\cdot \mMSi$ to Algorithm \ref{alg-approx}, all chores will be allocated.
To prove that, we focus on the agent who gets the last bundle in the execution of Algorithm \ref{alg-approx} (the agent  was chosen in line \ref{inalg-select} of Algorithm \ref{alg-approx},  when $k=n$ in the loop of line \ref{inalg-loop}). Let $\last$ be a special index for this agent. The whole proof will take the view from agent $\last$'s perspective. If we can prove that all remaining chores will be allocated to agent $\last$, then the correctness of theorem is implied.  For the simplicity of the presentation, we assume  that $\mMSi[\last]=1$.
%Suppose that agent $\last$ is the last one who gets the bundle in the execution of Algorithm \ref{alg-approx}. Without loss of generality, we assume that $\mMSi[\last]=1$. Now let us focus on the view of agent $\last$. If agent $\last$ always gets all remaining chores for the last bundle, then the correctness of theorem is implied.

Our proof has two parts: First we prove that all ``small" chores will be allocated, and then in the second part we analyze what happened to ``large" chores. 

Here we give a formal definition of ``small" and ``large". Notice that these notions will also be used in other sections.
\begin{definition}\label{def-big-little}
With a parameter $\alpha$ and an index $i\in\agents$, we define the set of ``large" chores as  $$\larg{i,\alpha}=\{c\in\items\mid\vai{c}>\alpha\}$$ and define the set of ``small" chores as  $$\smal{i,\alpha}=\{c\in\items\mid\vai{c}\le\alpha\}.$$
\end{definition}


First we prove that, from the last agent $\last$'s view, there is no small chore remained after the algorithm terminates.%With parameter $\alpha$, let $G(\alpha)=\{c\mid \vai[\last]{c}>\alpha\}$ denote the set of \emph{big} chores and $L(\alpha)=\{c\mid \vai[\last]{c}\le\alpha\}$ denote the set of \emph{little} chores.
\begin{lemma}\label{lem-no-less-2/9}
If we input threshold value $\alpha_i=\frac{11}{9}\cdot \mMSi$ to Algorithm \ref{alg-approx}, then all chores in the set $ \smal{\last, 2/9}$ will be allocated after the algorithm terminates.
\end{lemma}
\begin{proof}
We will prove the statement by contradiction. %Without loss of generality, we assume that $\mMSi[\last]=1$.
 Suppose that there was a chore $c\in \smal{\last, 2/9}$ remained. For any bundle $\alloci$, we have the inequality  $\vai[\last]{\alloci\cup c}>11/9$, otherwise Algorithm \ref{alg-approx} would allocate the chore $c$ to the bundle $\alloci$. As the valuation $\vai[\last]{c}\le 2/9$, we get the inequality $\vai[\last]{\alloci}>1$ for all $i\in\agents$. Recall that the value  $\mMSi[\last]$ is 1 by our assumption. So the total valuation should not exceed $n$. When we add up the valuations of all bundles, we have $\sum_{i\in\agents}\vai[\last]{\alloci}>n$, which is a contradiction. Therefore, there is no chore $c\in \smal{\last, 2/9}$ remained.
\end{proof}

%\xin{Try to give an example for large chores and swapping process}

Next we will analyze the allocation of large chores. Notice that the algorithm always gives the priority of large chores over small chores. In other words, no matter what kind of small chores we have and how they are allocated, they do not influence the allocation of large chores. Thus, we can focus on large chores without considering any small chores. 

Before presenting the details of the proof, here we give a high level idea of the proof. Suppose that $\allocs$ is the allocation returned by Algorithm \ref{alg-approx} and $\bundles$ is a \mmax~allocation for agent $\last$. We try to imagine that the allocation $\allocs$  is generated round by round from the allocation $\bundles$. In each round $k$, we swap some chores so that bundle $\bundlei[k]$ equals  bundle $\alloci[k]$, and then we will not touch this bundle anymore.  %Notice that every bundle is upper bound by the \mmax~of agent $\last$. 
Our goal is to prove that during the swapping process no bundle becomes too large. Then, when we come to the last bundle, agent $\last$ could take all remaining chores. To achieve this goal, we choose proper parameters and carefully specify the swap operation so that only two types of swaps are possible. 

Suppose that in round $k$, we swap chores between bundle $\bundlei[k]$ and bundle $\bundlei[j]$ where $j>k$. The target of the swapping is to make bundle $\bundlei[k]$ close to bundle $\alloci[k]$, and meanwhile bundle $\bundlei[j]$ will not increase too much. See Figure \ref{fig-type}.
\begin{itemize}
\item  %There is an index $j>k$ such that chore $c_j\in\bundlei[j]$, chore $c_k\in\bundlei[k]$ and the valuation $c_j$ larger than $c_k$.  
Type 1:  We will swap  chore $c_j\in\bundlei[j]$ with chore $c_k\in\bundlei[k]$ such that $\vai[\last]{c_j}\ge\vai[\last]{c_k}$ (possibly $c_k=\emptyset$). %A bundle swaps a larger chore to  bundle $\bundlei[k]$ and gets a smaller chore back (possiblly gets nothing back). 
After this swapping, the valuation of the bundle $\bundlei[j]$ would not increase.  
\begin{figure}
\centering
\includegraphics[scale=0.4]{Swap}
\caption{Two types of swaps. Blue squares are chores. Red doted squares are chores for swapping.}
\label{fig-type}
\end{figure}
\item  Type 2: We will swap chore $c_j\in\bundlei[j]$ with two  chores $c_{k_1},c_{k_2}\in\bundlei[k]$. We have that $\vai[\last]{c_{k_1}}\le\vai[\last]{c_j}$ and $\vai[\last]{c_{k_2}}\le\vai[\last]{c_j}$. However, it is possible that  $\vai[\last]{\{c_{k_1},c_{k_2}\}}>\vai[\last]{c_j}$.  This swap could make the bundle $\bundlei[j]$ larger. By a delicate choice of the parameter, this kind of increment can be well upper bounded and would not accumulate, i.e., there is at most one Type 2 swap involving  bundle $\bundlei[j]$ for any $j$. 
\end{itemize}
%Clearly, both types of swaps are good for our proof. \xin{Rephrase}

\begin{lemma}\label{lem-no-larger-2/9}
If we input threshold value $\alpha_i=\frac{11}{9}\cdot \mMSi$ to Algorithm \ref{alg-approx}, then after the algorithm terminates, all chores of the set $ \larg{\last,2/9}$ will be allocated.
\end{lemma}
\begin{proof}
%Please see Appendix \ref{apd-no-2/9} for the full proof. 
Suppose that $\allocs$ is the allocation returned by the algorithm and $\bundles$ is a \mmax~allocation for the last agent $\last$. We try to swap chores in \mmax~allocation $\bundles$ so that it will become the allocation $\allocs$. The proof is to analyze what happened in this swapping process. 

%Without loss of generality, we assume that $\mMSi[\last]=1$. 
Recall that the value  $\mMSi[\last]$ is 1 by our assumption. 
We only care about large chores here.  %As we have shown in Lemma \ref{lem-no-less-2/9}, we do not need to consider small chores.
 So let us define the bundle $\alloci^*$ as $\alloci\cap \larg{\last,2/9}$ and the bundle  $\bundlei^*$ as $\bundlei\cap \larg{\last,2/9}$.
For the simplicity of the proof, we assume that all bundles are ordered by the largest chore in each bundle, i.e., $\alloci[i]^*[1]\ge \alloci[j]^*[1]$  for all $i<j$. Notice that for the allocation $\allocs$, this order is exactly the order from the  for-loop in line \ref{inalg-loop} of Algorithm \ref{alg-approx}.

%Without loss of generality, we can assume the bundles in $\allocs$ are sorted as following: For any $j$, the bundle $\alloci[j]\in\allocs$ is generated by the algorithm when $k=j$ of the for loop in line \ref{inalg-loop}. %And define the bundle $\alloci^*$ as $\alloci\cap \larg{\last,2/9}$ and the bundle  $\bundlei^*$ as $\bundlei\cap \larg{\last,2/9}$.
%\xin{Write more explanation before the definition}

%To prove this lemma, we will start with bundles $\bundlei^*$ and then generate bundles $\bundlei$ by swapping chores between bundles.
We start with bundle collection $\bundles^{(0)}=\left(\bundlei[1]^*,\dots,\bundlei[n]^*\right)$  for our swapping process. Bundle collection $\bundles^{(0)}$ is an allocation of large chores such that $\vai[\last]{\bundlei[i]^*}\le 1$ for all $i\in\agents$. There are $n$ rounds  of the swapping process in total. In each round $t$, we generate a bundle collection $\bundles^{(t)}$ by swapping some chores in bundle collection $\bundles^{(t-1)}$, so that  bundle $\bundlei[t]^{(t)}=\alloci[t]^*$. Notice that we do not need to touch bundles with index strictly less than $t$ to fix bundle $\bundlei[t]^{(t)}$.  So we have $\bundlei^{(t)}=\alloci^*$ for all $i\le t$.
%At the beginning of the swapping process, Let bundle collection $\bundles^{(0)}=\left(\bundlei[1]^*,\dots,\bundlei[n]^*\right)$ include all $\bundlei^*$. Notice that $\larg{\last,2/9}=\cup_i\bundlei^*$.  Our target is to generate bundle collection $\bundles^{(t)}$ from $\bundles^{(t-1)}$ by  swapping chores between bundles, so that $\bundlei^{(t)}=\alloci^*$ for all $i\le t$. If this process can successfully proceed, then $\bundles^{(n)}=\left(\alloci[1]^*,\dots,\alloci[n]^*\right)$ which means all chores $c\in \larg{\last,2/9}$ are allocated.

If this swapping process could be successful to the round $n$, then all large chores are allocated in allocation $\allocs$, which implies the lemma.   To show this, we carefully specifiy the swapping process so that bundle collection $\bundles^{(t)}$ satisfies a good property. %We will prove this by induction.
%To prove this, we will show that, for $i>t$, bundles $\bundlei^{(t)}$  satisfies a good property by induction.

%The definitions of ``good" properties are in the below. Here we give a high level intuition for why ``good" bundle is good. There are two conditions. A bundle will be considered as ``good"  if it satisfies any of two conditions. 
%\begin{itemize}
%\item The fist condition states that the value of the bundle is upper bounded. It makes sure the number of large chores would not be greater than 4. This will make the case analysis possible.  Another good thing is that all initial bundles satisfy this condition. So we have the basis for the induction. 
%\item The second condition is about the sum of the largest chore and the least chore in a bundle. This condition could help us to analyze the number of chores after swapping. And we restrict the number of chores must be 4 before swapping. These two conditions could ensure that the swapping process would always swap a less valued chore to another bundle. 
%\end{itemize}
 % 1. contains all bundles at the beginning. 2. at most 4 large chores, wouldn't cause too much trouble. The second condition 1. though the swapping process, there is only such case that bundle could larger than 1. 2. we focus on the sum of largest and smallest chores, because in this way we can make sure 3 largest + 1 smallest will not exceed 11/9.

To introduce the good property, we need some definitions. Let $$U(\bundle)=\min_{c\in \bundle} \vai[\last]{c}+\max_{c\in\bundle}\vai[\last]{c}$$ denote the sum of largest and smallest chore in the bundle.

\bigskip
{\bf Good bundle:} A bundle $\bundle$ is \emph{good} if 1) $\vai[\last]{\bundle}\le1$ or, 2) $U(\bundle)<5/9\text{ and }|\bundle|=4.$ %\xin{Write down the intuition for the definition}
\bigskip

The second condition of the good bundle definition is related to the Type 2 swap which is mentioned in the high level idea. This condition can help us bound and control the damage which is caused by the second type swap. 

Here we slightly abuse the concept ``good" for bundle collection.

\bigskip
{\bf Good bundle collection:}  A bundle collection $\bundles^{(t)}$ is \emph{good} if $\bundlei^{(t)}=\alloci^*$ for all $i\le t$, and  each bundle $\bundlei^{(t)}$ is good for $i>t$.
\bigskip

Clearly, the bundle collection $\bundles^{(0)}$ is good. %Suppose when $t=k$, the bundle collection $\bundles^{(t)}$ is good. We will prove, when $t=k+1$,  by swapping some chores from $\bundles^{(k)}$, we can construct a good bundle collection $\bundles^{(k+1)}$.
This would be the basis for our induction. Now we need to describe the swapping process.
To  do it precisely, we introduce two operations $SWAP$ and $MOVE$, where the operation $SWAP$ would swap two chores and the operation $MOVE$ would move a set of chores  from their original bundles to a target  bundle.
%Here we introduce two operations that are very helpful in construction $\bundles^{(k+1)}$ from $\bundles^{(k)}$.

Given a bundle collection $\bundles$ and two chores $c_1$ and $c_2$, the $SWAP$ operation will generate a new bundle collection $\bundles^{\#}=SWAP(\bundles,c_1,c_2)$ such that: If $c_1=c_2$ or, $c_1$ and $c_2$ are in the same bundle, then $\bundles^{\#}=\bundles$; otherwise, we swap these two chores.
\begin{equation*}
 \bundlei^{\#}=
  \begin{cases}
   \bundlei & \text{if } c_1,c_2\notin \bundlei  \\
   (\bundlei\setminus c_1)\cup c_2       & \text{if } c_1\in\bundlei \\
   (\bundlei\setminus c_2)\cup c_1  & \text{if } c_2\in\bundlei
  \end{cases}
\end{equation*}
%This operation swaps chore $c_1$ and $c_2$.

Given a bundle collection $\bundles$, an  index $j\in\agents$ and a subset of chores $T\subseteq\items$, the $MOVE$ operation will generate a new bundle collection $\bundles^{\#}=MOVE(\bundles,j,T)$ such that
 \begin{equation*}
  \bundlei^{\#}=
   \begin{cases}
    \bundlei\setminus T & \text{if } i\neq j \\
    \bundlei\cup T      & \text{if } i=j \\
   \end{cases}
 \end{equation*}
 Notice that chores set $T$ could contain chores from different bundles. 
%This operation moves chores set $T$ from their original bundles to the bundle indexed by $j$.

%Let bundle $\bundlei^{(k+1)}=\alloci^*$ for $i\le k+1$. We will show how to construct remaining bundles i.e. $\bundlei^{(k+1)}$ where $i>k+1$.
%\xin{Give a reminder, but simplify this paragraph} 
%contains the largest chore among chores $\cup_{i\ge k+1} \bundlei^{(k)}$ (we can rename the bundle containing the largest chore to $\bundlei[k+1]^{(k)}$). %Let $\bundle(j)$ denote the $j$-th largest chore in the $\bundle$ from agent $\last$'s view.
%It is easy to see that $\bundlei[k+1]^{(k)}[1]=\alloci[k+1]^*[1]$, as Algorithm \ref{alg-approx} always allocates the largest chore of remaining to a new bundle. So, we only need  to take care of remaining chores from both bundles.

%\xin{Define two types swapping here, make argument easy?}
Now we describe and prove the correctness of  the swapping process by induction. Suppose that bundle collection $\bundles^{(k)}$ is good. We will swap and move some chores between bundle $\bundlei[k+1]^{(k)}$ and bundles with index greater than $k+1$, so that the bundle $\bundlei[k+1]^{(k)}$ becomes bundle $\alloci[k+1]^*$.  Without loss of generality, we can assume that the largest chore in  bundle $\bundlei[k+1]^{(k)}$ and  bundle $\alloci[k+1]^*$ are the same, i.e., chore $\bundlei[k+1]^{(k)}[1]=\alloci[k+1]^*[1]$. This is the largest chore among  the set $\bigcup_{i\ge k+1} \bundlei^{(k)}$ by our assumption of the order of allocation $\allocs$ (The assumption made at the beginning of the whole proof).   
 By the condition of good bundle collection and the value of large chores, we know that  bundle $\bundlei[k+1]^{(k)}$ contains at most $4$ chores.
%For each chore $c\in \cup_i\bundlei^*$, we  know the valuation $\val[\last](c)>\frac{2}{9}$ and the valuation $\vai[\last]{\bundlei^*}\leq 1$. This implies that each $\bundlei^*$ contains at most $4$ chores. %During the swapping process, we keep the property that for $i>t$ each bundle $\bundlei^{(t)}$ contains at most $4$ chores. 
 
 Before the case analysis, here we give a  claim which can help us combine several cases into one. 
\begin{claim}\label{claim-4chores}
For the cases $\cadin{ \bundlei[k+1]^{(k)}}=\mbox{1, 2, and }4$, we have the inequalities $\cadin{\alloci[k+1]^*}\ge \cadin{\bundlei[k+1]^{(k)}}$ and $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$ for $j\le\cadin{\bundlei[k+1]^{(k)}}$.
\end{claim}
 Please read Appendix \ref{apd-no-2/9} for the proof of Claim \ref{claim-4chores}.
 
  Based on the size of bundle $\bundlei[k+1]^{(k)}$, we have the following case analysis.

%Now we show a delicate to swap some chores to make $\bundlei[k+1]^{(k)}$ to become $\bundlei[k+1]$. We show it in case analysis:
\begin{itemize}
\item $\cadin{\bundlei[k+1]^{(k)}}=1,2,\mbox{ and } 4$:  Let $d=\cadin{\bundlei[k+1]^{(k)}}$ be the cardinality of the bundle. 
By Claim \ref{claim-4chores}, we have  $\cadin{\alloci[k+1]^*}\ge \cadin{\bundlei[k+1]^{(k)}}$ and $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$ for all $j\le d$.   We swap each pair of chores $\bundlei[k+1]^{(k)}[j]$ and $\alloci[k+1]^*[j]$ for $j\le d$. Here all swaps are Type 1 (described in high level idea) swap. %Since we have the inequality $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$, after these swaps, no bundle with index larger than $k+1$  become larger.  
 If the cardinality $\cadin{\alloci[k+1]^*}>d$, then we just move the remaining chores  to bundle $\bundlei[k+1]^{(k)}$.  Please see Figure \ref{fig-case124} for this process.


Mathematically, let bundle collection $G^{(1)}=\bundles^{(k)}$. The swapping of the first $d$ chores  could be represented as the following form  $G^{(j)}=SWAP\left(G^{(j-1)},\bundlei[k+1]^{(k)}[j],\alloci[k+1]^*[j]\right)$ for $2\le  j\le d$. The bundle collection $G^{(d)}$ is the resulting bundle after these swaps.  And the moving operation to generate bundle collection $\bundles^{(k+1)}$ is equivalent to 
$$\bundles^{(k+1)}=MOVE\left(G^{(d)},k+1,\alloci[k+1]^*\right).$$ 

It is not hard to see after all these operations, no bundle with index larger than $k+1$  becomes larger nor gets more chores. 
 A good bundle will still be a good bundle. Therefore, when we get the  bundle collection $\bundles^{(k+1)}$, it is a good bundle collection. 
 
 \begin{figure}[h]
\centering
\includegraphics[scale=0.4]{case124}
\caption{When $j\le d$, the operation would be a Type 1 swapping (type is described in high level idea). For the case $d'>d$, the operation would be  the move operation.}
\label{fig-case124}
\end{figure}

%For chores in bundle $\alloci[k+1]^*$, we move them  from their current bundles  to  bundle $\bundlei[k+1]^{(k)}$.
%Mathematical equivalently, for the bundle collection $\bundles^{(k+1)}$, we have  %$$\bundlei^{(k+1)}=\bundlei^{(k)}\setminus \alloci[k+1]^*\text{ for } i>k+1.$$
%Formally, we have
%$$\bundles^{(k+1)}=MOVE\left(\bundles^{(k)},k+1,\alloci[k+1]^*\right).$$

%The bundle with index larger than $k+1$ either does not change or remove some chores. Thus a good bundle is still good. This gives that bundle collection $\bundles^{(k+1)}$ is good.

%\xin{Write a new statement: $|\alloci[k+1]^*|\ge |\bundlei[k+1]^{(k)}|$ and $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$ }

%\item $|\bundlei[k+1]^{(k)}|=2$: First we have the cardinality  $|\alloci[k+1]^*|\ge 2$. Because Algorithm \ref{alg-approx}  can at least allocate chore $\bundlei[k+1]^{(k)}[2]$ to bundle $\alloci[k+1]^*$ as the second chore. This observation also implies valuation $\vai[\last]{\bundlei[k+1]^{(k)}[2]}\le\vai[\last]{\alloci[k+1]^*[2]}$. If chore $\bundlei[k+1]^{(k)}[2]\neq\alloci[k+1]^*[2]$, then we swap these two chores. And if there are more chores in bundle $\alloci[k+1]^*$ i.e. $|\alloci[k+1]^*|>2$, then we just move remaining chores from their current bundles  to $\bundlei[k+1]^{(k)}$. Mathematical equivalently,% for $i>k+1$, 
%we have
\begin{comment}
\begin{equation*}
 \bundlei^{(k+1)} =
  \begin{cases}
   \bundlei^{(k)}\setminus \alloci[k+1]^* & \text{if }  \alloci[k+1]^*[2]\notin  \bundlei^{(k)}\\
   \left(\bundlei^{(k)}\cup\bundlei[k+1]^{(k)}[2]\right)\setminus \alloci[k+1]^*      & \text{if } \alloci[k+1]^*[2]\in  \bundlei^{(k)} \\
  \end{cases}
\end{equation*}
\end{comment}
%$$\bundles^{(k+1)}=MOVE\left(SWAP\left(\bundles^{(k)},\bundlei[k+1]^{(k)}[2],\alloci[k+1]^*[2]\right),k+1,\alloci[k+1]^*\right).$$

%The bundle with index larger than $k+1$ either does not change or remove some chores. Thus a good bundle is still good. This gives that bundle collection $\bundles^{(k+1)}$ is good. \xin{Is it better to make it a claim?}

\item $\cadin{\bundlei[k+1]^{(k)}}=3$: As chore $\bundlei[k+1]^{(k)}[1]$ equals chore $\alloci[k+1]^*[1]$ and $\vai[\last]{\left\{\bundlei[k+1]^{(k)}[1],\bundlei[k+1]^{(k)}[2]\right\}}<11/9,$ we can at least allocate chore $\bundlei[k+1]^{(k)}[2]$ with chore  $\alloci[k+1]^*[1]$ in the algorithm.
Thus, we have $\cadin{\alloci[k+1]^*}\ge 2$. Let $$G=SWAP\left(\bundles^{(k)},\bundlei[k+1]^{(k)}[2],\alloci[k+1]^*[2]\right)$$ be the bundle collection that  swap chore $\bundlei[k+1]^{(k)}[2]$ and chore $\alloci[k+1]^*[2]$.  Now we consider the following inequality:
\begin{equation}\label{ineq-2-3}
\vai[\last]{\left\{\alloci[k+1]^*[1],\alloci[k+1]^*[2], \bundlei[k+1]^{(k)}[3]\right\}}\le 11/9
\end{equation}

If the Inequality \ref{ineq-2-3} holds,  then we have $\cadin{\alloci[k+1]^*}\ge 3$ and $\vai[\last]{\bundlei[k+1]^{(k)}[3]}\le\vai[\last]{\alloci[k+1]^*[3]}$. For this case, we will swap chore $\bundlei[k+1]^{(k)}[3]$ and chore $\alloci[k+1]^*[3]$ and move remaining chores in bundle $\alloci[k+1]^*$ to bundle $\bundlei[k+1]^{(k)}$, i.e.,
$$\bundles^{(k+1)}=MOVE\left(SWAP\left(G,\bundlei[k+1]^{(k)}[3],\alloci[k+1]^*[3]\right),k+1,\alloci[k+1]^*\right).$$
The operations for this subcase are exactly the same situation as above (see Figure \ref{fig-case124}). %the bundle with index larger than $k+1$ either does not change or remove some chores. Thus a good bundle is still good. This gives that bundle collection $\bundles^{(k+1)}$ is good.
By a similar argument,  bundle collection $\bundles^{(k+1)}$ is good.



If the Inequality \ref{ineq-2-3} does not hold, then we move chore $\bundlei[k+1]^{(k)}[3]$ to the bundle where chore $\alloci[k+1]^*[2]$ comes from. And then move  other chores in bundle $\alloci[k+1]^*$  to bundle $\bundlei[k+1]^{(k)}$. Please see Figure \ref{fig-case3} for this process.

 \begin{figure}[h]
\centering
\includegraphics[scale=0.4]{case3}
\caption{There would be one operation of the Type 2 swap for chores $\alloci[k+1]^*[2],\bundlei[k+1]^{(k)}[2]$ and $\bundlei[k+1]^{(k)}[3]$. For the case $d'>2$, the operation would be the move operation.}
\label{fig-case3}
\end{figure}
Let $j$ be an index of a bundle such that $\alloci[k+1]^*[2]\in\bundlei[j]^{(k)}$. Then, formally this process is
$$\bundles^{(k+1)}=MOVE\left(MOVE\left(G,j,\bundlei[k+1]^{(k)}[3]\right),k+1,\alloci[k+1]^*\right).$$

This is the most complicated case since bundle $\bundlei[j]^{(k+1)}$ contains more items than bundle $\bundlei[j]^{(k)}$. 
We prove that  bundle $\bundlei[j]^{(k+1)}$ is good in Claim \ref{claim-two-one}. And for other bundles with index larger than $k+1$, it either does not change or removes some chores.  Therefore, bundle collection $\bundles^{(k+1)}$ is good.

%\item $|\bundlei[k+1]^{(k)}|=4$:
%Using the property of good bundle,  we prove that $|\alloci[k+1]^*|\ge 4$ and $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$ for $j\le4$ in Claim \ref{claim-4chores}. For the first 4 chores, we swap them one by one. If the cardinality $|\alloci[k+1]^*|>4$, then we just move remaining chores from their original bundles  to $\bundlei[k+1]^{(k)}$.

%Formally the process is described as following.Let bundle collection $G^{(0)}=\bundles^{(k)}$ and bundle collection  $G^{(j)}=SWAP\left(G^{(j-1)},\bundlei[k+1]^{(k)}[j],\alloci[k+1]^*[j]\right)$ for $1\le  j\le 4$. We have
%$$\bundles^{(k+1)}=MOVE\left(G^{(4)},k+1,\alloci[k+1]^*\right).$$ 

%The bundle with index larger than $k+1$ either does not change or remove some chores. Thus a good bundle is still good. This gives that bundle collection $\bundles^{(k+1)}$ is good.
\end{itemize}


\begin{claim}\label{claim-two-one}
 Let $j$ be the index such that the chore $\alloci[k+1]^*[2]\in\bundlei[j]^{(k)}$. For the case $\cadin{\bundlei[k+1]^{(k)}}=3$ and Inequality \ref{ineq-2-3} does not hold, %$\vai[\last]{\alloci[k+1]^*[1]\cup\alloci[k+1]^*[2]\cup \bundlei[k+1]^{(k)}[3]}> 11/9$,
after all $SWAP$ and $MOVE$ operations, bundle $\bundlei[j]^{(k+1)}$ is good.
\end{claim}
Please read Appendix \ref{apd-no-2/9} for the proof of Claim \ref{claim-two-one}.

%\xin{Rewrite here }It is easy to see that, for a good bundle, if we replace one chore with a smaller chore, it is still good. The only case, which may increase the number of chores or increase the value of chores, is concluded in claim \ref{claim-two-one}. Thus we can keep this process to $\bundles^{(n)}$.
By this case analysis, we show that the bundle collection will keep the good property until the last one $\bundles^{(n)}$. So we prove the lemma.


\end{proof}

Using the  above two lemmas, now we can show the  correctness of theorem \ref{thm-exist}.

\begin{proof}[Proof of Theorem \ref{thm-exist}]

Combing Lemma \ref{lem-no-less-2/9} and Lemma \ref{lem-no-larger-2/9}, we have that Algorithm \ref{alg-approx} will output a \amMS{11/9} allocation with input such that $\alpha_i=\frac{11}{9}\cdot \mMSi$.
\end{proof}

We can easily transfer the existence result of Theorem \ref{thm-exist} to a polynomial  approximation scheme. The only computational hardness part of our algorithmic framework is the valuation of \mmax~for each agent. 
Notice that computing \mmax~of an agent is exactly the makespan of a job scheduling problem, which is a famous NP-hard problem. 
%The difficulty of computation lies in computing the value of \mmax~of each agent. Notice that computing \mmax~of an agent is exactly the makespan of a job scheduling problem.  
This can be solved by a PTAS from job scheduling literature~\cite{jansen2016closing}. Therefore, from the result of existing 11/9 approximation \mmax~allocation, we have a PTAS for $11/9+\epsilon$ approximation \mmax~allocation. The constant 11/9 could be improved if anyone can prove a better existence ratio of our algorithmic framework.

Given the above result, it is natural to ask what is the best approximation ratio of our algorithmic framework. Though we cannot prove the best ratio now, we present the following example to show a lower bound of our technique.
%For the lower bound of our algorithmic framework, we give the following example.
\begin{exmp}\label{exm-lower-bound}
In this example, we consider an instance of 14 chores and 4 agents with an identical valuation (not just ordinal, but cardinal is also same). The valuation of each chore is demonstrated by the \mmax~allocation.
%Their valuations are: one chore is valued as $\frac{9}{17}$, one chore is valued as $\frac{7}{17}$, one chore is valued as $\frac{6}{17}$ and two chores are valued as $\frac{5}{17}$ and 9 chores are valued as $\frac{4}{17}$.

A \mmax~allocation of this instance is that $$\alloci[1]=\left\{\frac{9}{17},\frac{4}{17},\frac{4}{17}\right\}, \alloci[2]=\left\{\frac{7}{17},\frac{6}{17},\frac{4}{17}\right\}\text{ and }\alloci[3]=\alloci[4]= \left\{\frac{5}{17},\frac{4}{17},\frac{4}{17},\frac{4}{17}\right\},$$ where the numbers are valuations of each chore. Obviously, the \mmax~of each agent is 1. 

For any $\alpha$ such that $1\le \alpha<20/17$, if we input  threshold values $(\alpha,\alpha,\alpha,\alpha)$  to Algorithm \ref{alg-approx}, then we will get the first bundle $\alloci[1]^*=\{\frac{9}{17},\frac{7}{17}\}$, the second bundle $\alloci[2]^*=\{\frac{6}{17},\frac{5}{17},\frac{5}{17}\}$ and the third bundle $\alloci[3]^*=\{\frac{4}{17},\frac{4}{17},\frac{4}{17},\frac{4}{17}\}$. When we come to the last bundle, the total valuation of remaining chores is $\frac{20}{17}$. Since the threshold $\alpha<20/17$, we cannot allocate all chores.
%However, if we input $\alpha_i<20/17$ to Algorithm \ref{alg-approx}, then not all chores could be allocated.
\end{exmp}

Example \ref{exm-lower-bound} implies the following result.
\begin{theorem}\label{thm-lower-bound}
Algorithm \ref{alg-approx} cannot guarantee to find an \amMS{\alpha} allocation when $\alpha<20/17$.
%The best approximation ratio $\alpha$ of \mmax~by Algorithm \ref{alg-approx} with inputting threshold value $\alpha\cdot\mMSi$ cannot be less than $20/17$.
\end{theorem}



==> EC 21 submission/intro.tex <==
% (Note for myself) History for cake cutting problem, and then history for indivisible goods, and then give some sense of important of chore division.

It is an important research theme in social science, economics and computer science to study how to allocate items among a number of different agents in a fair manner. The items could be something people like such as a house, cake or other resources which are called goods, or something people dislike such as tasks or duties which are called chores.  The rigorous study of the fair allocation problem dates back to the 1940's starting from the seminal work of~\cite{steinhaus1948problem}. At the beginning, researchers were interested in valuable divisible resources and nicknamed this problem ``Cake Cutting". Two well known fairness notions are defined and explored: 1) Envy freeness -- each agent prefers her own share of the cake over any other agent's~\cite{foley1967resource}; 2) Proportionality -- each agent gets a share  at least as valuable as the average of the whole cake~\cite{steinhaus1948problem}.


%The problem of how to fairly allocate indivisible items receive much attention recently in computer science and economic community (cite some papers here).  This agenda is commonly appear in daily life (list some applications). Many research are focus on goods.

However, when researchers began to study the indivisible setting, the story changed dramatically. The reason is that, for indivisible items, envy-free and proportional allocations may not exist, and  even approximation is impossible.  A simple and somewhat awkward example is that of two agents with the same valuation for one single item. No matter how you allocate the item, there is one agent getting nothing. 

So how should we divide indivisible items fairly?  We need a more delicate fairness concept.  Budish~\cite{budish2011combinatorial} proposed a relaxation of proportionality, which is called maximin share. It is considered as  one of most successful fairness concepts for studying indivisible items. %It was proposed by Budish~\cite{budish2011combinatorial} from the study of a combinatorial assignment problem with competitive equilibrium. 
The idea of maximin share comes from the cut-and-choose protocol.  In the cut-and-choose protocol, there is a cutter dividing the whole set of resources  and the cutter must be the last one to choose her share. As the cutter may get the worst share, the maximin share for an agent  is the best value that the agent can guarantee if she is the cutter. An allocation is a \emph{maximin share allocation} if everyone gets a bundle at least as valuable as her maximin share.


%For the indivisible items setting, envy-free and proportional allocations may not exist  and cannot even be approximated. A simple and somewhat awkward example is that two agents with a same valuation to one single item. No matter how you allocate the item, there is one agent getting nothing. From the study of a combinatorial assignment problem with competitive equilibrium, Budish~\cite{budish2011combinatorial} propose the fairness notion of maximin share, which can be considered as a relaxation of proportionality to  the indivisible setting. The idea of maximin share is from the cut-and-choose protocol.  In the cut-and-choose protocol, there is a cutter dividing the whole set of resources  and the cutter must be the last one to choose her share. So the cutter may get the worst share. The maximin share for an agent  is the best value that the agent can guarantee if she is the cutter. And an allocation is maximin share allocation if everyone gets a bundle at least her maximin share.

%\xin{History and recent study of maximin share}
Recently, the notion of maximin share attracted a lot of attention from the computer science community since the seminal work of~\cite{procaccia2014fair}. For goods, Kurokawa et al.~\cite{procaccia2014fair} show that a maximin share allocation may not exist. On the other hand, they demonstrate an exponential time algorithm for $\frac{2}{3}$ approximation of maximin share allocation. A line of works~\cite{DBLP:journals/talg/AmanatidisMNS17,barman2017approximation,ghodsi2018fair,DBLP:conf/soda/GargMT19,garg2019improved}  follow up to design efficient algorithms  and improve the approximation ratio. For chores, Aziz et al.~\cite{aziz2017algorithms}  show that maximin share allocation may not exist  and demonstrate a polynomial time algorithm for $2$ approximation. Later Barman and Khrishna Murthy
~\cite{barman2017approximation} improved this result  to a polynomial time algorithm for $\frac{4}{3}$ approximation.

%\xin{Try to propose questions: what is the best approximation ratio, how efficient we can approximate}
%Kurokawa et al.~\cite{procaccia2014fair} first studied maximin share fairness from a computer science perspective. They showed that maximin share allocation may not exist. On the other hand, they demonstrate an exponential time
%algorithm for $\frac{2}{3}$ approximation of maximin share allocation.  This discovery ignites people's interest in designing efficient algorithms and push
%the approximation ratio for maximin share allocation. A line of works~\cite{barman2017approximation,ghodsi2018fair,garg2019improved}  follow up and improve the approximation ratio to
%$\frac{3}{4}$ and computable by a poly-time algorithm.
%The seminal work~\cite{procaccia2014fair} analysis the maximin share fairness in a typical computer science perspective.

%introduce to chore
So far, most efforts in this area are devoted to studying how to divide goods. The parallel problems for chores are less discussed in the community. We have two reasons to pay attention to indivisible chores setting.  1) Technically, it may betray some people's expectation that the problems for chores and goods are intrinsically different.  For example,  maximum Nash welfare allocation is  Pareto optimal with  certain fairness  for goods~\cite{caragiannis2016unreasonable,DBLP:journals/corr/BogomolnaiaMSY17}, however no single valued rule can be efficient with good fairness guarantee for chores~\cite{DBLP:journals/corr/BogomolnaiaMSY17}.
%maximum Nash social welfare allocation is envy-free and efficient for divisible goods. However, for chores, no single valued rule can be envy-free and efficient~\cite{DBLP:journals/corr/BogomolnaiaMSY17}. This could explain why maximum Nash welfare allocation is  Pareto optimal with  certain fairness  for indivisible goods~\cite{caragiannis2016unreasonable}, but we cannot derive a similar result for indivisible chores by this kind of approach. 
%there is a pseudo-polynomial time algorithm for  Pareto optimal allocation with certain fairness for indivisible goods~\cite{barman2018finding}, but the existence of this kind of allocation for indivisible chores is still unclear. 
In this paper, we will show an algorithmic framework that is suitable for chores but has no direct implication for goods.
2) Practically, there are many applications in daily life in which allocating indivisible chores is involved. For example, household chores dividing, assignment of TA duties and the famous problem job scheduling etc. And this problem is also closely related to bin packing problem.


%apply the maximin share notion to chores.  They
We focus on two questions: What is the best ratio for which an approximation allocation exist? Can we design an efficient algorithm with a better approximation ratio? We make significant contributions to these questions in this paper.
%From a computer science perspective, there are two interesting questions regarding \mmax~allocation of indivisible chores: What is the best ratio that an approximation allocation exist? Can we design an efficient algorithm with a good approximation ratio? Though we cannot solve it completely, we will give positive answers  to both questions.

%Our work follows this direction to analyze the approximation ratio and design efficient algorithms for maximin share allocation under indivisible chores setting.




%To study fair allocation problem, a suitable fairness notion is vital. Proportionality is a well accepted fairness notion in many areas. It requires that every agent should get an average share in their own perspectives. However, in the indivisible setting, it is probably that no allocation can satisfy this requirement.

%In this paper, we focus on the fairness notion \mmax~allocation.  This notion could be considered as an indivisible version of proportionality.
%Discussion on fairness notion: 1. the origin of mms. 2. mms on goods receive many attentions. 3. recently people also care about chores

%We can define the minimax notion for chores symmetrically.


\subsection{Our results and techniques}
%\paragraph{Analysis of our algorithmic framework}
All of our results rely on a novel algorithmic framework which combines some existent ideas.
The first building block of our framework is a technique by Bouveret and Lema{\^\i}tre \cite{bouveret2016characterizing}, which allows us to focus on the class of  instances where agents share the same ordinal preference. This technique has been successfully applied to approximation of maximin share for goods~\cite{barman2017approximation,garg2019improved}. Interestingly, we identify a similarity between our algorithmic framework and well-known First Fit Decreasing (FFD) algorithm for the bin packing problem~\cite{johnson1973near}.
%Based on this technique, we develop the following algorithmic framework for chores: Given each agent a threshold value, try to construct bundle one by one. When constructs a bundle, try to allocate the largest under the constraint that some agent may tolerate the bundle according to threshold value
%And all of our results rely on this algorithmic framework.
The core ideas of this part are simple: 1. As long as the bundle is within the bin size, add as many items as possible to the bundle;
2. Try to allocate large items first (as they're more problematic).
%So the process of the algorithmic framework

Under this algorithmic framework, we prove our main result.
\begin{reptheorem}{thm-exist}
For any chore division instance $\inst$, there always exists an $\frac{11}{9}$ approximation maximin share allocation.
\end{reptheorem}


To combine the above two ideas, the algorithm proceeds as follows: %is very simple: 
Order the chores in decreasing order (using the reduction from a general instance to an instance such that all agents share the same ordinary preference~\cite{bouveret2016characterizing}), and fill a bundle with as many chores as possible in a greedy fashion, as long as some agent thinks it is within
$\frac{11}{9}$ of her maximin share. Then one such agent takes the bundle and leaves the game. We repeat this $n$ times, where $n$ is the number of agents.
It is clear that each agent gets at most $\frac{11}{9}$ of her maximin share. To verify that it is indeed an $\frac{11}{9}$ maximin share allocation,
we only need to prove that all the chores are allocated during the process. This is however highly non-trivial.
We need to maintain some invariant property during the process and argue that it will allocate all the chores.

If one replaces  $\frac{11}{9}$ with a smaller ratio, can we still show that it will allocate all the chores? We do not know. We show by an example that one cannot make the ratio as small as $\frac{20}{17}$, but leave the tightness of the ratio as an interesting open question.

The above algorithm is quite simple, but needs to know the maximin share of each agent. Computing that value is precisely a job scheduling/load balancing problem, which is NP-hard. Since there is a PTAS for the job scheduling problem~\cite{jansen2016closing}, we have a PTAS for $\frac{11}{9}+\epsilon$ approximation of maximin share allocation.


%Here the approximation ratio $11/9$ is not tight. In Theorem \ref{thm-lower-bound}, we show a $20/17$ lower bound of our framework in proving the existence of approximation of \mmax~allocation. We believe that the upper bound $11/9$ of the algorithmic framework can be improved. However, to get an improvement on $11/9$ with our current proof idea, it may require a significant effort on doing case analysis.  We want to mention that the approximation ratio of FFD algorithm for bin packing problem is tight to 11/9. However, from the view of  mathematical proof, they are intrinsic different. You cannot deduce one from another directly and we believe that the ratio on dividing chores can be further improved
%
%
%As the existence result is from an algorithm, it is natural to ask the complexity of our algorithm. The only obstacle to transfer the existence result to an efficient algorithm is that we need to know \mmax~of each agent. Computing that value is exactly a job scheduling/load balancing problem which is NP-hard. Since there is a quite fast PTAS for job scheduling problem~\cite{jansen2016closing}, we have a good PTAS for $11/9+\epsilon$ approximation of \mmax~allocation. However, it may not be considered as an efficient algorithm for some practical application even if we demand a slightly good approximation ratio like $5/4$.

However, the PTAS may not be considered as an efficient algorithm for some practical applications if $\epsilon$ is small.  To get a truly efficient algorithm, we notice that it may not be necessary to get an accurate value of maximin share. What we need is a reasonable lower bound of maximin share for each agent. %to make the algorithmic framework execute correctly. 
This kind idea has already been applied to design efficient algorithms for fair allocation of indivisible goods~\cite{garg2019improved}. With this idea, we try to pre-allocate all chores in an appropriate and easy-to-implement way according to one particular agent's valuation, and then from this pre-allocation we can estimate a lower bound of maximin share for this particular agent. This complicates the argument, and it is not clear if we can get the same ratio of $\frac{11}{9}$. In this paper, we show that a slightly worse ratio of $\frac{5}{4}$ is achievable. We leave the problem of giving a polynomial time $\frac{11}{9}$ approximation algorithm as an open problem.

%
%However, our estimation of the lower bound cannot get  $11/9$ approximation of \mmax~allocation.
%After compromising the approximation ratio a little, we have the following result.
%\begin{reptheorem}{thm-poly}
%If all valuations are integers, we have an efficient polynomial time algorithm for 5/4 approximation minimax share allocation.
%\end{reptheorem}
%
%
%
%\paragraph{Special cases and relationship with other areas}
%Besides the above results for general instances, we analysis the performance of our algorithmic framework on two important special cases. Fist we study two-agent case, the following is our result.
%\begin{reptheorem}{thm-2-agent}
%For two-agent case, our algorithmic framework can find an \amMS{\frac{[8]}{7}} allocation, and ratio $8/7$ is tight.
%\end{reptheorem}
%Notice that the ratio $8/7$ is less than our lower bound $20/17$ for general instance. And unlike the general instance, here we get a tight ratio.

 One special case of our problem is that all agents have the same valuation for chores. We notice that the problem of job scheduling on identical machines is exactly this special case. Based on our algorithm,  we can design a very efficient $O(m\log m+n)$ time algorithm to get a  $\frac{11}{9}$ approximation of optimal scheduling. To the best of our knowledge, except for the PTAS which is not so efficient in practice,  there is no algorithm approximating optimal better than $\frac{4}{3}$.

%
%
%\begin{reptheorem}{thm-schedul}
%For scheduling problem, we have an algorithm output a \amMS{11/9} approximation of optimal scheduling in $O(m\log m+n)$ time.
%\end{reptheorem}



\subsection{Related work}
%Please revise the focus of related work from EFX to MMS.


The topic of fair division has a long history; it originates from the work of Steinhaus~\cite{steinhaus1948problem} in the 40s, which triggered vast literatures on this subject -- we refer the reader to the books~\cite{robertson1998cake,Moulin03} for an overview. Most of the literature in this area focuses on the divisible setting,
including very recent breakthroughs like the envy-free cake-cutting protocol of Aziz and McKenzie~\cite{AM16} and a similar result for chores~\cite{DBLP:conf/soda/DehghaniFHY18}. In contrast, fairly allocating indivisible items among agents has not been similarly popular, until very recently. The delayed interest is likely caused by the lack of suitable fairness notions.
%Most probably, the reason for this delay is that the beautiful fairness notions of envy-freeness and proportionality, that have received so much attention in the literature on divisible items, are not always achievable with indivisible items. %To give an embarrassing example, just consider a single item and two agents with identical valuations for the item.




The recent interest for the indivisible items setting was sparked by the definition of fairness notions that approximate envy-freeness and proportionality. In particular, the notions of  EF1 and EFX, defined by  Budish~\cite{budish2011combinatorial}  and Caragiannis et al.~\cite{caragiannis2016unreasonable} can be thought of as an approximate version of envy-freeness and have received much attention recently. Some works explore their existence~\cite{plaut2018almost,DBLP:conf/ec/CaragiannisGH19,DBLP:conf/soda/ChaudhuryKMS20,DBLP:conf/sigecom/ChaudhuryGM20}, others investigate the relationship with efficiency~\cite{caragiannis2016unreasonable,barman2018finding}.
Besides the concepts of EF1 and EFX mentioned above, approximate versions of envy-freeness include epistemic envy-freeness~\cite{ABCGL18} or notions that require the minimization of the envy-ratio~\cite{lipton2004approximately} and degree of envy~\cite{CEEM07,NR14} objectives.


The notion of maximin fair share (MMS) was first proposed by Budish~\cite{budish2011combinatorial} and inspired a line of works.  %see~\cite{procaccia2014fair,AMNS17,barman2017approximation,ghodsi2018fair}.
In the seminal work of~\cite{procaccia2014fair}, the authors prove that MMS fairness may not exist, but a $\frac{2}{3}$ approximation of MMS  can be guaranteed. Due to their work, the best approximation ratio of MMS and a polynomial time algorithm for finding it becomes an intriguing problem.  A line of works~\cite{barman2017approximation,DBLP:conf/soda/GargMT19,DBLP:journals/talg/AmanatidisMNS17} tries to design an efficient algorithm for a $\frac{2}{3}$ approximation of MMS allocation.
%Barman et al.~\cite{barman2017approximation} discovered the first polynomial time algorithm for $\frac{2}{3}$ approximation of MMS. 
Ghodsi et al. \cite{ghodsi2018fair} further improve the existence ratio of MMS to $\frac{3}{4}$. Shortly after, Grag and Taki~\cite{garg2019improved} show a polynomial time algorithm for $\frac{3}{4}$ approximation of MMS by combining all previous techniques for this problem.%, which is developed from the framework in~\cite{DBLP:conf/soda/GargMT19}.

For the chores setting, Aziz et al.~\cite{aziz2017algorithms} initiate the research on maximin share notion and provide a polynomial algorithm for 2 approximation. Utilizing the technique for goods, Barman et al.~\cite{barman2017approximation} also showed a polynomial time algorithm for $\frac{4}{3}$ approximation of MMS for chores. To the best of our knowledge, the ratio $\frac{4}{3}$ was the state of art before this paper.

Except maximin fairness, recently a line of study explores the problem fair division of indivisible chores from different perspectives. Aziz et al.~\cite{aziz2018fair} proposed a model for handling mixture of goods and chores. The paper~\cite{aziz2019strategyproof} showed
that strategyproofness would cost a lot on maximin fairness for chores. Aziz et al.~\cite{aziz2019weighted} considered the case that agents have different weights in the allocation process.
%Mix goods and chores~\cite{aziz2018fair} weighted version~\cite{aziz2019weighted} strategy proof~\cite{aziz2019strategyproof}

The problem of job scheduling/load balancing is a special case of allocating indivisible chores.  It is a fundamental discrete optimization problem, which has been intensely studied since the seminal work~\cite{graham1966bounds}. Graham~\cite{graham1969bounds} showed that the famous Longest Processing Time rule can give a $\frac{4}{3}$ approximation to the optimal. Later Hochbaum and Shmoys~\cite{hochbaum1987using} discovered a PTAS for this problem. A line of follow up works~\cite{alon1998approximation,jansen2010eptas,jansen2016closing} try to improve the running time by developing new PTAS algorithms.

Our algorithmic framework is similar to First Fit Decreasing (FFD) algorithm for the bin packing problem. Johnson in his doctoral thesis~\cite{johnson1973near} first showed the performance of FFD for the bin packing problem is tight to $\frac{11}{9}$ upon an additive error. To simplify the proof and tighten the additive error, subsequent works~\cite{baker1985new,yue1991simple,dosa2007tight} were devoted to this problem and finally got optimal parameters.   A modified and more refined version of FFD was proposed and proved to be approximately tight up to the ratio $\frac{71}{60}$~\cite{DBLP:journals/jc/JohnsonG85}.


%Please cite \cite{caragiannis2016unreasonable,barman2018finding} for EF1 and PO. Cite \cite{plaut2018almost,DBLP:conf/ec/CaragiannisGH19} for existence of EFX and \cite{caragiannis2016unreasonable,ABM18} for approximation of EFX.

%As mentioned earlier, EF1 is easy to achieve with several different methods. What is really challenging is to achieve EF1 and Pareto-optimality simultaneously. This was proved to be possible in \cite{caragiannis2016unreasonable}, by an allocation of maximum Nash welfare. %The popular website Spliddit \cite{GP14}, available at \url{www.spliddit.org}, returns such allocations as part of its ``Divide goods'' application.
%Following \cite{caragiannis2016unreasonable}, Barman et al.~\cite{barman2018finding} investigate whether EF1 and Pareto-optimal allocations can be computed efficiently and present a pseudo-polynomial-time algorithm.

%Unlike EF1, the existence of EFX allocations is still a mystery, even for three agents with additive valuations. Plaut and Roughgarden \cite{plaut2018almost} prove the existence of EFX allocations for setting with two agents only or with more agents and identical valuations. In addition, they present an algorithm for computing an $1/2$-EFX allocation, where the value of each agent from her bundle is at least half of what the EFX property requires it to be. Caragiannis et al.~\cite{caragiannis2016unreasonable} and Amanatidis et al.~\cite{ABM18} consider different approximations of EFX (namely, approximations of the strongly related pairwise MMS fairness concept).





\subsection{Organization}
In section \ref{sec-pre}, we introduce some basic notations and concepts for the paper. In section \ref{sec-frame}, we demonstrate our algorithmic framework which is the foundation of this work. We prove the existence of an $\frac{11}{9}$-approximation allocation by the algorithmic framework in section \ref{sec-exist}. Following the existence result, in section \ref{sec-poly} we push further to have an efficient polynomial time algorithm for \amMS{\frac{5}{4}} allocation. %Then we analysis the limit of our algorithmic framework in section \ref{sec-limit}.
In section \ref{sec-special}, we connect our problem with the job scheduling problem and obtain an efficient algorithm.  Finally, in section \ref{sec-dis} we discuss some future directions and open problems for our algorithmic framework.


==> EC 21 submission/limit.tex <==
In this section, we discuss the limitation of our framework.  %The previous best known result is 4/3 approximation~\cite{barman2017approximation}. We show that their technique cannot give a ratio better than 4/3. 
For our algorithm framework, we show a 20/17 lower bound. In section \ref{sec-poly}, we design a threshold testing algorithm. At the first look, people may wonder is there a more natural approach to do threshold testing.  Here we give an example to show that, for Algorithm \ref{alg-approx}, suppose  a set of $\{\alpha_i\}$ make the algorithm allocate all chores,   if we increase the value of $\alpha_i$, it is possible that chores cannot be all allocated. 


% The lower bound   Please refer the literature of LPT algorithm for load balancing 
%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
Define base allocation and show that such base allocation cannot break 4/3 barrier. 
\begin{exmp}
Set $\epsilon=\frac{1}{6(n-1)}$.

Base allocation  $\{2/3-2\epsilon, 1/3\}$, $\{2/3-3\epsilon,1/3+\epsilon\}$,$\dots$ $\{1/2,1/2-2\epsilon\}$ and $\{1/2,1/2-\epsilon\}$, and $1/3-\epsilon$ remaining

Optimal allocation $\{1/3-\epsilon,1/3,1/3+\epsilon\}$, $\{2/3-2\epsilon,1/3+2\epsilon\}$, $\{2/3-3\epsilon,1/3+3\epsilon\}$, $\dots$, $\{1/2+\epsilon,1/2-\epsilon\}$ and $\{1/2,1/2\}$
\end{exmp}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%


For the lower bound of our algorithmic framework, we give the following example. 
\begin{exmp}
In this example, we consider an instance of 14 chores and 4 agents with an identical valuation (not just ordinal, but cardinal is also same). The valuation of each chore is demonstrated by the optimal allocation. 
%Their valuations are: one chore is valued as $\frac{9}{17}$, one chore is valued as $\frac{7}{17}$, one chore is valued as $\frac{6}{17}$ and two chores are valued as $\frac{5}{17}$ and 9 chores are valued as $\frac{4}{17}$.

An optimal allocation of this instance is that $$\alloci[1]=\{\frac{9}{17},\frac{4}{17},\frac{4}{17}\}, \alloci[2]=\{\frac{7}{17},\frac{6}{17},\frac{4}{17}\}\text{ and }\alloci[3]=\alloci[4]= \{\frac{5}{17},\frac{4}{17},\frac{4}{17},\frac{4}{17}\},$$ where the numbers are valuations of each chore. Obviously, the \mmax~of each agent is 1. However, if we input $\alpha_i<20/17$ to Algorithm \ref{alg-approx}, then not all chores could be allocated. 
\end{exmp}

\begin{theorem}\label{thm-lower-bound}
Algorithm \ref{alg-approx} cannot show the existence of \amMS{\alpha} for $\alpha<20/17$.
\end{theorem}



Intuitively, people may think if Algorithm \ref{alg-approx} can allocate all chores on input of threshold values $\{\alpha_i\}$, then  Algorithm \ref{alg-approx} should allocate all chores with larger threshold values. Here we give a counter example for this monotonicity. 
\begin{exmp}\label{exm-no-monoton}
In this example, we consider an instance of 17 chores and 4 agents with an identical valuation. The valuation of each chore is demonstrated by the optimal allocation. 

An optimal allocation of this instance is that $$\alloci[1]=\{5.1,1.2,1.2\}, \alloci[2]=\alloci[3]=\{2.75,2.75,1,1\}\text{ and }\alloci[4]=\{2.5,1,1,1,1,1\},$$ where the numbers are valuations of each chore.  The \mmax~of each agent is 7.5. You can verity that if we input threshold value $7.5$ to Algorithm \ref{alg-approx}, all chores will be allocated. And the allocation is exactly the optimal allocation we give here. 

However, if we input threshold value  7.6 to Algorithm \ref{alg-approx}, we have $$\alloci[1]=\{5.1,2.5\}, \alloci[2]=\alloci[3]=\{2.75,2.75,1.2\}\text{ and }\alloci[4]=\{1,1,1,1,1,1,1,1,1\}.$$ There are 2 chores remained. 
\end{exmp}



==> EC 21 submission/notations.tex <==
\newcommand{\mMS}{\mbox{MMS}} %shortcut for minmax share
\newcommand{\mMSi}[1][i]{\mMS_{#1}} %for maximin value of agent i
\newcommand{\amMS}[1]{$#1$-\mMS} %for alpha approximation of maximin allocation 
\newcommand{\mmax}{maximin share} %name of maximin allocation

\newcommand{\mbR}{\mathbb R}

\newcommand{\inst}{\mathcal{I}}

\newcommand{\bundle}{B} %symbol for bundle
\newcommand{\bundlei}[1][i]{\bundle_{#1}} %for bundle i
\newcommand{\bundles}{\mathcal{\bundle}} %for bundle collection

\newcommand{\alloc}{A} %symbol for allocation
\newcommand{\allocs}{\mathbf \alloc} %for a whole allocation 
\newcommand{\allocsmi}{\allocs_{-i}} %for allocation without i
\newcommand{\alloci}[1][i]{\alloc_{#1}} %for agent i's allocation, e.g. \alloci for A_i, and \alloci[j] for A_j
\newcommand{\alloclist}[1][n]{\left(\alloc_1,\dots,\alloc_{#1}\right)} %for full writing of an allocation

\newcommand{\agents}{\mathcal{N}} %for set of agents
\newcommand{\items}{\mathcal{M}} %for set of items

%definitions for valuations
\newcommand{\va}{\mathcal{V}} %symbol for valuation
\newcommand{\val}[1][i]{v_{#1}} %for agent i's valuation function e.g. \val for v_i and \val[j] for v_j
\newcommand{\vai}[2][i]{v_{#1}\left(#2\right)} %for agent i's valuation function on a set of items e.g. \vai{M} for v_i(M), and \vai[j]{M} for v_j(M)
\newcommand{\valist}[1][n]{\left(\val[1],\dots,\val[#1]\right)}

\newcommand{\larg}[1]{\mathcal{L}\left(#1\right)}
\newcommand{\smal}[1]{\mathcal{S}\left(#1\right)}

\newcommand{\last}{\omega} 

\newcommand{\argmin}{\operatornamewithlimits{arg\ min}}

\newcommand{\nitest}[1]{\mathsf{NT}\left(#1\right)}

\newcommand{\cadin}[1]{\left\lvert#1\right\rvert}

==> EC 21 submission/polytime.tex <==
To run our algorithm for $\frac{11}{9}$-approximation maximin share allocation, we need to know the \mmax~of each agent. The computation of the maximin share is NP-hard. Though we have a PTAS for $\left(\frac{11}{9}+\epsilon\right)$-approximation, even if we want to get a $\frac54$-approximation with currently best PTAS for job scheduling~\cite{jansen2016closing}, the running time could be more than $2^{39000}+poly(n,m)$. This is not acceptable for a real computation task. 
%In this section, assuming all valuations are integers, we show that how to design an efficient polynomial time algorithm for 5/4 approximation \mmax~ allocation.
To attack this computational embarrassment, we give a trial on designing an efficient polynomial time algorithm for $\frac54$-approximation \mmax~allocation when valuations are all integers.


The design of the efficient algorithm relies on an observation: It is not necessary to know the exact value of \mmax. A reasonable lower bound of \mmax~could serve the same end. This kind of observation was successfully applied to the goods setting~\cite{garg2019improved}.

From this observation, the basic idea of the design is to find a good lower bound of \mmax. And from the lower bound, we compute a  proper threshold value for executing  Algorithm \ref{alg-approx}. To make this idea work, we have two problems to solve: 1) How to find a proper lower bound of \mmax? 2) How to use this lower bound to get a good threshold value for the algorithm? 

We find that a threshold testing algorithm could be an answer to these problems. The threshold testing algorithm tries to allocate relative large chores in a certain way to see whether the threshold is large enough for an agent or not. 
For the first problem, we can use the threshold testing algorithm as an oracle to do binary search for finding a reasonable lower bound of \mmax~of each agent. For the second problem, 
the allocation generated by the threshold testing algorithm could serve as a benchmark to help us find a good threshold value.
%\xin{Rephrase} we will try to mimic the  proof  of Lemma \ref{lem-no-larger-2/9} to see what  threshold value could make the proof work. The allocation of large chores generated from the threshold testing algorithm is very helpful to establish the proof. Let us call such allocation base allocation.  The base allocation serves as a benchmark which plays similar role of the \mmax~allocation in the proof of Lemma \ref{lem-no-larger-2/9}. %\xin{Not clear enough}
%Let base allocation be the allocation of large chores generated from the threshold testing algorithm. The base allocation serves as a benchmark which plays similar role of the \mmax~allocation in the proof of Lemma \ref{lem-no-larger-2/9}. %\xin{What you mean?} For obtaining a good threshold value, we just try to see what threshold value could make the proof work.


%If threshold testing algorithm can allocate all relative large chores, then the the threshold value is large enough for the agent; Otherwise if some large chore does not get allocated, it means the threshold value is too small. \xin{This paragraph is difficult to understand}

%Regarding the second problem, please recall the swapping process in the proof of Lemma \ref{lem-no-larger-2/9}.   The allocation of large chores, which is from the threshold testing algorithm, can play a similar  role of \mmax~allocation in the swapping process.

%We will present a threshold testing algorithm first. \xin{Please rephrase this paragraph} Upon giving a threshold value and an agent, we want to finish a special allocation for that particular agent. This special allocation would help us to design and analysis the true algorithm.
%The threshold testing algorithm can test whether the threshold is  large enough or not for the special allocation. %After the analysis of threshold testing algorithm, we show the main algorithm.
%The main algorithm first use the threshold testing algorithm as an oracle to do binary search for finding a reasonable lower bound of \mmax~of each agent. And then plug in a certain threshold value of each agent to the algorithmic framework which is introduced in section \ref{sec-frame}.


\subsection{Difficulties on threshold testing}\label{subsec-failure}
To explain some key points of the threshold testing, we introduce a simple trial -- \emph{naive test}  which is  building on Algorithm \ref{alg-approx} straightforwardly.  The naive test gives a  polynomial-time $\frac{11}{9}$-approximation algorithm for the job scheduling problem (see Section \ref{sec-special}).  However, we construct a counter example which is an IDO instance for the naive test in this section. %In addition, we try to extract some intuitions from this failure  to design a threshold testing for general instances.% \xin{Discuss why we don't use algorithm 2 as a threshold testing. Key point: monotonicity, optimal allocation of 1/2 large chores}

%\xin{Rename threshold and something others to make it clear.}
%Given an agent $i$ and a threshold $s_i$, we consider an instance consists of $n$ identical agents with the valuation $\val$. And then input $n$ copies of threshold $\frac{11}{9}\cdot s_i$ to  Algorithm \ref{alg-approx}. If all chores are allocated, then the threshold $s_i$ pass the test.
 

 
%Now we introduce the simple trial of the threshold testing. 
Basically, the naive test tries to run Algorithm \ref{alg-approx} directly on a single agent. 
Suppose that we have an instance $\inst=\langle\agents,\items,\va\rangle$.  Let $\nitest{i,s_i}$  denote a naive test, where $i$ is an agent  and $s_i$ is a threshold. The naive test $\nitest{i,s_i}$ will first construct an instance $ID=\langle\agents,\items,\va'\rangle$ such that $\va'=(\val,\dots,\val)$, i.e., valuations are all same as $\val$. Then it will run Algorithm \ref{alg-approx} with the $ID$ instance and threshold values $\left( s_i,\dots, s_i\right)$. If all chores are allocated in Algorithm \ref{alg-approx}, then the naive test $\nitest{i,s_i}$ returns ``Yes", otherwise returns ``No".

 
 
 
 Given an agent $i$, let $s^*_i=\min_{s_i}\left\{s_i\mid\nitest{i,s_i} \text{returns ``Yes"}\right\}$ be the minimal value passing the naive test. %be the minimal value passing the naive test. %such that all chores will be allocated if we input a threshold $\frac{11}{9}\cdot s_i$ to Algorithm \ref{alg-approx}.%\footnote{A normal instance with $n$ different agents would be a  trouble for testing task. Here we consider an instance consists of $n$ identical agents with the valuation $\val$. And then input $n$ copies of threshold $\frac{11}{9}\cdot s_i$ to  Algorithm \ref{alg-approx}.} 
 By the proof of Theorem \ref{thm-exist}, it is not hard to see that the value $s^*_i$ satisfies $s^*_i\le\frac{11}{9}\cdot\mMSi$.  %By Lemma \ref{lem-monotone}, we can binary search for the value $s^*_i$.
%How to compute the value of $s^*_i$ is not what we want discuss here. Assume that we can find such minimal value $s^*_i$.
Based on this observation, it is natural to try the following.

\bigskip
{\bf Trial approach}: First, compute the minimal threshold $s^*_i$ for each agent.\footnote{How to compute the value of $s^*_i$ is not important for our discussion on the properties of threshold testing.}  Then run Algorithm \ref{alg-approx} with thresholds $\{ s^*_i\}_{i\in\agents}$ to get an allocation.
\bigskip

If the following conjecture is true, then this approach would work. 
% \begin{definition}
% Given an agent $i$ and a threshold $s_i$, let oracle $O$ be an algorithm such that: Input $n$ copies of valuation $\val$ and threshold $\frac{11}{9}\cdot s_i$ to  Algorithm \ref{alg-approx}. If Algorithm \ref{alg-approx} allocates all chores, the oracle will return ``Yes"; otherwise, returns ``No". 
% \end{definition}
% Let $s^*_i$ be  the minimal value $s_i$ such that oracle $O$ would return ``Yes".
% From \xin{put a reference}, we know that the value $s_i$ is a lower bound of $\mMSi$. A natural idea is to put $\frac{11}{9}\cdot s_i$ to Algorithm \ref{alg-approx}

\begin{conj}\label{conj-mon}
Montonicity: If Algorithm \ref{alg-approx} can allocate all chores with threshold values $\{\alpha_i\}_{i\in\agents}$, then  Algorithm \ref{alg-approx} should allocate all chores with any threshold values $\{\beta_i\}_{i\in\agents}$  such that $\beta_i\ge\alpha_i$ for all $i$. 
 \end{conj}
For the naive test, this conjecture implies that if the test $\nitest{i,s_i}$ returns ``Yes", then the test $\nitest{i,s'_i}$ returns ``Yes" for any $s'_i\ge s_i$.
Unfortunately, Conjecture \ref{conj-mon} is not true even for the naive test (all agents have the same valuation). 
Here we give a counter example.
\begin{exmp}\label{exm-no-monoton}


In this example, we consider an instance of 17 chores and 4 agents. All agents have the same valuation. The valuation of each chore is demonstrated by the \mmax~allocation. 

The \mmax~allocation of this instance is that $$\alloci[1]=\{5.1,1.2,1.2\}, \alloci[2]=\alloci[3]=\{2.75,2.75,1,1\}\text{ and }\alloci[4]=\{2.5,1,1,1,1,1\}.$$ The numbers are valuations of each chore.  The \mmax~and value $s^*_i$ of each agent is 7.5. It is easy to verity that all chores will be allocated if we input the threshold values $(7.5, 7.5, 7.5, 7.5)$ to Algorithm \ref{alg-approx}. And the allocation is exactly the  allocation we give here. 

However, if we input threshold values $(7.6,7.6,7.6,7.6)$ to Algorithm \ref{alg-approx}, we will have $$\alloci[1]=\{5.1,2.5\}, \alloci[2]=\alloci[3]=\{2.75,2.75,1.2\}\text{ and }\alloci[4]=\{1\}\times 7.$$ There are 2 chores remained. 

So for this example, naive test $\nitest{i,7.5}$ will return ``Yes", but $\nitest{i,7.6}$ will return ``No".
\end{exmp}
This example reveals a surprising fact about Algorithm \ref{alg-approx}. When we have more spaces to allocate chores, it could be harmful. The connection between Conjecture \ref{conj-mon} and the trial approach is that: In terms of  the last agent's perspective, when we do the trial approach,  the effect of heterogeneous valuations would act as enlarging threshold. Next we construct an example based on Example \ref{exm-no-monoton} to show how the trial approach failed. 

\begin{exmp}\label{exm-fail}
We construct an IDO instance consists of 4 agents and 17 chores. For those 4 agents, three of them (agents $t_1$, $t_2$ and $t_3$) have exact the same valuation as Example \ref{exm-no-monoton}. Agent $t_4$ is a special agent. The valuation of agent $t_4$ is demonstrated by the \mmax~allocation: 
$$\alloci[1]=\{5.1,2.4\}, \alloci[2]=\alloci[3]=\{2.75,2.75, 2\}\text{ and }\alloci[4]=\{5/6\}\times 9.$$ 
By our construction, it is easy to verify that the value $s^*_i$ equals  7.5 for any agent $i$.  The trial approach will  input the threshold (7.5,7.5,7.5,7.5) to Algorithm \ref{alg-approx}. 

Notice, this is an IDO instance. For agents $t_1$, $t_2$ and $t_3$, the largest 4 chores are valued at $\{5.1,2.75,2.75,2.5\}$. For agent $t_4$, the largest 4 chores are valued at $\{5.1,2.75,2.75,2.4\}$.  When we do the trial approach,  agent $t_4$ will get the first bundle, which is $\alloc=\{5.1,2.4\}$ for agent $t_4$.  And this bundle contains chores $\{5.1,2.5\}$ in terms of the valuation of other agents. Just like Example \ref{exm-no-monoton}, there will be 2 chores unallocated at the end. So the trial approach fails. 
\end{exmp}
%For this valuation, it is easy to verify that if we input the threshold 7.5 to Algorithm \ref{alg-approx} to do the testing
% \xin{rephrase here}  If we use Algorithm \ref{alg-approx} to do threshold testing, then it is possible that we get a 7.5 as threshold for the agent in above example. We  can construct another agent that can take the largest and the fourth largest chores as an accepting bundle. Now let us put 3 agents with valuation as above example and this constructed agent together. 

%\xin{Rethink.  Too full, easily to have a non optimal , even when we have more space, it is  we need more space for }

%Here we give a possible answer to this failure. The naive test could find an  allocation which is too full with respect to the threshold. Since the trial approach directly uses that threshold,  heterogeneous valuations may result in some non optimal allocations. Even though we have enough space to pass the test, the deviation from the optimal allocation could cause much damage. So we need some space to tolerate such kind of errors.



%From these examples, we can see that the monotonicity is quite crucial for 

%Example \ref{exm-fail} does not use the fact that Conjecture \ref{conj-mon} is not true. Different agents work like enlarge threshold value. 
%A possible answer to this failure is that this method does not allow any space for the error caused by a miss allocation. 
%\xin{rephrase here} we try to do a partial allocation strictly less than $\frac{11}{9}\cdot s_i$ to get a space for the error. 


\subsection{Threshold testing}
Before we present the threshold testing algorithm, let us summarize the issue of the naive test by Figure \ref{fig-axis}. The naive test will return a threshold value $\alpha$ (a red value in Fig \ref{fig-axis} between $\mMSi$ and $\frac{11}{9}\mMSi$). When we run Algorithm \ref{alg-approx}, the effect of other agents can be viewed as increasing the threshold $\alpha$. Let us call the threshold after increasing \emph{effective threshold}. If the effective threshold is a blue value, then Algorithm \ref{alg-approx} could be failed. To resolve this situation, we need to find a threshold $\alpha'$ such that every value  larger than $\alpha'$ will pass the test.

  \begin{figure}[h]
\centering
\includegraphics[scale=0.4]{axis}
\caption{The $x$-axis is the threshold value for the naive test. Blue means the value does not pass the test. Red means the value pass the test.}
\label{fig-axis}
\end{figure}

From this idea, we try to find a  value $s_i$, which is a  lower bound on $\mMSi$. Then scale it large enough ($\frac{5}{4}\cdot s_i$) so that no larger value will fail the test. This can be done by allocating chores with valuation larger than $s_i/4$ in a special way.

 %In Section \ref{subsec-failure}, we see some difficulties in designing a valid testing algorithm. The threshold returned by the naive test is too tight in some sense. We will demonstrate a solution in this section.  %\xin{Rephrase all}
%\xin{ 1. find a clue for how much space we need }
%The idea is that, when we do the allocation, we leave enough space for possible errors. %The naive test is not suitable for this task. \xin{Rephrase}
%The problem is that the performance of naive test is unstable. If we run it with the valuation in Example \ref{exm-lower-bound}, then it will return a threshold above $\frac{20}{17}\cdot \mMS$. If we run it with the valuation in Example \ref{exm-no-monoton}, then it will return a threshold which equals  $\mMS$. So we cannot easily decide how much extra space is necessary. 
  %A resolve  is that, when we do the testing, do not allocate too full regarding to the threshold. In other words, we will allocate some bundles strictly less than the threshold to tolerate the error. 
  


%Here is a simple description of our threshold testing algorithm. Given a threshold $s_i$, the threshold testing algorithm will focus on the chores with value larger than $s_i/4$: 
%\begin{enumerate}[Step 1.]
%\item Try to allocate part of these chores in an optimal way, i.e., allocate them into bundles not larger than $s_i$; 

%\item  Allocate the remaining chores into the bundles not larger than $\frac{5}{4}\cdot s_i$. 
%\end{enumerate}
%If we try to target at $\frac{5}{4}\cdot s_i$, then each bundle in Step 1 will have  $\frac{1}{4}\cdot s_i$ extra space for potential errors. %We should mention  that $5/4$ may not be the optimal parameter
%We will show this would work.  


%In detail, a test would try to allocate part of large chores into bundles with valuations upper bounded by $s_i$ and allocate other chores into bundles with valuations upper bounded by $\frac{5}{4}\cdot s_i$. In this way, when allocate that part of large chores, we leave each bundle a  $\frac{1}{4}\cdot s_i$ space for the error. 
%we try to allocate some large chores in an optimal way and allocate other chores with a bar allowing enough error. 
%And we have the following observation helps us to do the partial allocation of large chores: In a \mmax~allocation, there is only one way to allocate chores larger than 1/2 of \mmax~and part of chores larger than 1/4 of \mmax. 

Here is a detailed description of our threshold testing algorithm.

\begin{algorithm}[H]
\KwIn{Index $i$ of an agent, a threshold value $s_i$}
\KwOut{Yes/No}
\BlankLine
	%Suppose $\vai{c_1}\ge\vai{c_2}\dots\ge\vai{c_m}$\;
	 Let $k=|\larg{i,s_i/2}|$ \tcp*[l]{Please refer to  Definition \ref{def-big-little}}
	 Initialize an allocation  $\allocs$ such that  bundle $\alloci[j]=\{\items[j]\}$ for $j\le k$ and  bundle $\alloci[j]=\emptyset$ for $j>k$\tcp*[l]{Allocate chores in the set $\larg{i,s_i/2}$} \label{inalg-allocate}
	%Let $\allocs=(\emptyset,\dots,\emptyset)$ {\bf and} $T=\items$\;
	Let $R= \larg{i,s_i/4}\setminus \larg{i,s_i/2}$ denote the set of remaining large chores\;% \tcp*[l]{Only large chores matter}
	%\tcp*[h]{We try to allocate as many as possible chores from $R$ to first $k$ bundles}\;
        %$j=0$\;% \tcp*[l]{Initial the counter for the largest chore in $R$}
        
	\For(\tcp*[h]{Try to fill up the first $k$ bundles}\label{inalg-pre-big}){$t= k$ \KwTo $1$}
	{
	     	%$j=1$\tcp*[l]{Counter for the largest available chore}
		%\If{$\exists t\le k$ such that $ \vai{\alloci[t]\cup R[j]}\le s_i$}{
		\For(\tcp*[h]{Search the largest chore could allocate}){$j= 1$  \KwTo $|R|$}
		{
		\If{$ \vai{\alloci[t]\cup R[j]}\le s_i$}{
			$\alloci[t]=\alloci[t]\cup R[j]$\;
			$R=R\setminus R[j]$\;
			%break\tcp*[l]{At most one more large chore could be allocated} 
			}
		%$j=j+1$\;
		}
	}
	%$R=R\setminus\left(\bigcup_{t\le k}\alloci[t]\right)$\;
%	Let $R$ denote the set of unallocated chores.]
	\tcp{The following for-loop is similar to Algorithm \ref{alg-approx}}
	\For(\label{inalg-after-big}){$t=k+1$ \KwTo $n$}
	{
		%$\alloci[t]=\emptyset$\;
		\For{$j= 1$  \KwTo $|R|$}
		{
			\If(\label{inalg-if-11/9}){$\vai{\alloci[t]\cup R[j]}\le \frac{5}{4}\cdot s_i$}
			{
				$\alloci[t]=\alloci[t]\cup R[j]$\;
				
			}
		}
		$R=R\setminus \alloci[t]$\;
	}
	\eIf(\tcp*[h]{Whether all large chores are allocated or not}){$R=\emptyset$}{\Return Yes\;}{\Return No\;}
\caption{Threshold testing}\label{alg-proper}
\end{algorithm}



%At the first look of this threshold testing algorithm, people may wonder why we design it like this. Here is a remark for it:
%\begin{itemize}
%\item \xin{Put this remark ahead of the algorithm} People may wonder why we don't just use Algorithm \ref{alg-approx} with input of valuations $(\val,\dots,\val)$ and thresholds $(s_i,\dots,s_i)$  as threshold testing? The threshold obtained by Algorithm \ref{alg-approx} can guarantee that for each agent $i$, when input the same valuation $(\val,\dots,\val)$ and the same threshold $(s_i,\dots,s_i)$ to Algorithm \ref{alg-approx}, all chores will be allocated. To get a full allocation, we need put all agents' valuations and thresholds together to  Algorithm \ref{alg-approx}. However, this step may not work. Please see the discussion of Example \ref{exm-no-monoton}.
%Actually, when we have different valuations, from a particular agent $i$'s view, the effect is somewhat like increasing the threshold.
%Actually, Example \ref{exm-no-monoton} shows a more surprising fact about Algorithm \ref{alg-approx}. Intuitively, people may think the following monotonicity should hold: for any $s_i'\ge s_i$ when we input valuations $(\val,\dots,\val)$ and thresholds $(s_i',\dots,s_i')$ to Algorithm \ref{alg-approx}, all chores should be allocated. However, the following Example \ref{exm-no-monoton} disproves this monotonicity.

%\item
%We will use threshold testing to design a binary search to find a proper lower bound of \mmax.  For the correctness of binary search, we need monotonicity of the algorithm i.e. threshold testing for agent $i$ should return YES on all values larger than $\mMSi$.  Otherwise, the binary search may not terminate correctly to return a lower bound of $\mMSi$. This monotonicity in general does not hold, please refer Example \ref{exm-no-monoton}.

%\item The ratio 11/9 in line \ref{inalg-if-11/9} can be any number between 11/9 and 5/4. Actually, Algorithm \ref{alg-proper} only considers the large chores in $\larg{i,s_i/4}$. So a smaller constant would not be  helpful.  The choice of this constant only need to satisfy two properties: 1) When the threshold $s_i\ge\mMSi$, the process should allocate all chores; 2) The final allocation can serve as a benchmark for the proof of 5/4 approximation to \mmax~allocation.
%\end{itemize}

To get a lower bound of \mmax~by a binary search,
%For the correctness of binary search, 
we need monotonicity of the algorithm, i.e., threshold testing should return ``Yes" on all values larger than $\mMSi$  for any agent $i$.  %Otherwise, the binary search may not terminate correctly to return a lower bound of $\mMSi$. 
Though Example \ref{exm-no-monoton} shows monotonicity does not hold in general,
we prove that by the choice of parameters, the following monotonicity holds.
\begin{lemma}\label{lem-monotone}
For any $\alpha_i\ge\frac{11}{9}\cdot\mMSi$, if we input the threshold $\alpha_i$ to Algorithm \ref{alg-approx}, then all chores will be allocated.
\end{lemma}
\begin{proof}
Notice that, if we replace the condition of $\alpha_i$ from $\alpha_i=\frac{11}{9}\cdot\mMSi$ to $\alpha_i\ge\frac{11}{9}\cdot\mMSi$ in Lemma \ref{lem-no-less-2/9} and Lemma \ref{lem-no-larger-2/9}, the proof of those two lemmas work in the same way. This observation would directly implies this lemma.
%The proof of Lemma \ref{lem-no-less-2/9} and Lemma \ref{lem-no-larger-2/9} work for all values larger than $\mMSi$. The only requirement on value $\alpha_i$ to make proof work is that: there is an allocation $\allocs$ such that $\vai{\alloci[j]}\le\frac{9}{11}\cdot\alpha_i$ for all $j$. In addition, this is certainly true for any $\alpha_i\ge\frac{11}{9}\cdot\mMSi$.
\end{proof}

Next we prove that our threshold testing algorithm has the following monotone property. %This property will guarantee, when we use Algorithm \ref{alg-proper} to do binary search, we will correctly get a lower bound of \mmax.
\begin{lemma}\label{lem-mms-ok}
If we input an index $i$ and a threshold $s_i\ge\mMSi$ to Algorithm \ref{alg-proper}, then the algorithm will return ``Yes". Therefore, when we use Algorithm \ref{alg-proper} to do binary search, we will correctly get a lower bound of \mmax.
\end{lemma}
\begin{comment}
%Please refer Appendix \ref{apd-lem-mms-ok} for the proof.
\begin{proof}[Proof sketch]
Please refer Appendix \ref{apd-lem-mms-ok} for the proof. We give some key points of the proof here.
When the threshold $s_i\ge\mMSi$, we know that there is an allocation $\allocs^*$ such that $\vai{\alloci[j]^*}\le s_i$ for all $j$. We will try to argue that, for chores being allocated before line \ref{inalg-after-big} of Algorithm \ref{alg-proper}, they are optimally allocated by comparing with allocation $\allocs^*$. Also by comparing with allocation $\allocs^*$, there is an allocation of remaining chores (chores that are not allocated before line \ref{inalg-after-big}) such that no bundle would exceed the threshold $ s_i$. Thus, we can allocate the remaining chores just like Algorithm \ref{alg-approx} with a larger threshold $\frac54\cdot s_i$.  This is exactly what the algorithm did after line \ref{inalg-after-big}.

\end{proof}
\end{comment}

\begin{proof}
As Algorithm \ref{alg-proper}  deal with  the chores in set $\larg{i,s_i/4}$ only,  let us assume that the chores set $\items=\larg{i,s_i/4}$ in this proof.

When the inequality $s_i\ge\mMSi$ holds, there is an allocation $\allocs^*$ such that $\vai{\alloci[j]^*}\le s_i$ for all $j$. We will compare the allocation $\allocs^*$ with the allocation generated in Algorithm  \ref{alg-proper} to show that %in some sense bundles constructed before line \ref{inalg-after-big}   are optimally allocated. 
 the remaining chores after line \ref{inalg-after-big} do not  greater than the chores in the allocation  $\allocs^*$.% have a \mmax~not greater than $s_i$, which means 
Then we can allocate them in a way like Algorithm \ref{alg-approx}. So the threshold $s_i$ will pass the test. 

We introduce some notations for the proof. Let $H$ denote the set of chores which are allocated before line \ref{inalg-after-big}. Let $Q$ be the set of chores of bundles containing a really large chore from allocation $\allocs^*$, i.e.,   $$\left\{\bigcup \alloci[j]^*\mid \alloci[j]^*\in\allocs^*\mbox{ and }\alloci[j]^*\cap\larg{i,s_i/2}\neq\emptyset\right\}.$$ 


 Let $\allocs$ be the allocation generated in  Algorithm \ref{alg-proper} when we input agent $i$ and value $s_i$. Suppose that for allocation $\allocs$, the indices of the bundles  are the same as in Algorithm \ref{alg-proper}. Let  $k=\cadin{\larg{i,s_i/2}}$ be the number of really large chores. 
Notice that no two chores in the set $\larg{i,s_i/2}$ will be allocated to one bundle i.e., all these chores  are allocated separately. So we have  $H=\bigcup_{j\le k}\alloci[j]$. Without loss of generality, we can assume that the $j$-th largest chore $\items[j]\subseteq\alloci[j]^*$ for all $j\le k$. Then we have $Q=\bigcup_{j\le k}\alloci[j]^*$.

Since the set of chores $\larg{i,s_i/2}$ is contained in both set $H$ and set $Q$, we can simply let function $f(c)=c$ for any chore $c\in\larg{i,s_i/2}$. Let us consider the set of chores $Q'=Q\setminus\larg{i,s_i/2}$. 

\bigskip
{\bf Index:} If chore $c\in\alloci[j]^*$, we call $j$ the \emph{index} of chore $c\in Q'$. %Similar, let $H'=H\setmiuns\larg{i,s_i/2}$ and call $j$ to be the index of chore $c\in H'$
\bigskip

Recall that we have assumed that the set of all chores $\items=\larg{i,s_i/4}$. So there are no two chores in $Q'$ sharing one index.  

%Missing proofs for the following claims are in Appendix \ref{apd-lem-mms-ok}.
\begin{claim}\label{claim-assume}
Without breaking the condition $\vai{\alloci[j]^*}\le s_i$ for all $j\le k$,  we can assume that:
\begin{enumerate}[1)]
\item For any two chores $c_1,c_2\in Q'$, if $\vai{c_1}>\vai{c_2}$, then the index of chore $c_1$ greater than the index of chore $c_2$. 
\item  Indexes of chores in set $Q'$ are consecutive and end at the index $k$, i.e., the set of indexes equals the set $[j,k]$ (here $[j,k]$ is the set of  all integers between $j$ and $k$).
\end{enumerate}
\end{claim}
\begin{proof}%[\bf Proof of Claim \ref{claim-assume}]
Recall that  the chore $\items[j]\in\alloci[j]^*$ for each $j\le k$. It means that when index becomes larger, there is more space to allocate a chore in $Q'$ without exceeding the threshold $s_i$. So we have the following observation. If  condition 1) breaks, we can swap two chores without violating \mmax~condition. If condition 2) breaks, then there is an index $j$ for a chore $c\in Q'$ and an index $d$ such that $d>j$ and there is no chore corresponding to index $d$. In this case, we can reallocate chore $c$ to bundle $\alloci[d]^*$ and it is still a \mmax~allocation. These two observations imply we can make above two assumptions.
\end{proof}


Suppose that the assumptions in Claim \ref{claim-assume} hold, we prove the following claim. 

\begin{claim}\label{claim-lessthan}
There is an injection $f:Q\rightarrow H$ such that $\vai{c}\le\vai{f(c)}$ for any chore $c\in Q$ . 
\end{claim}
\begin{proof}%[\bf Proof of Claim \ref{claim-lessthan}]
%We will prove that there is an injection $f:Q\rightarrow H$ such that for any chore $c\in Q$, we have $\vai{c}\le\vai{f(c)}$. This will imply that the remaining chores ($\items\setminus H$) are smaller  to the remaining chores of \mmax~allocation ($\items\setminus Q$).



Since the set of chores $\larg{i,s_i/2}$ is contained in both set $H$ and set $Q$, we can simply let function $f(c)=c$ for any chore $c\in\larg{i,s_i/2}$. Now we consider the chores $Q'=Q\setminus\larg{i,s_i/2}$. 


Similarly, let $H'=H\setminus\larg{i,s_i/2}$ and call $j$ to be the index of chore $c\in H'$. Notice that, by Algorithm \ref{alg-proper}, the allocation $\allocs$ and set $H'$ satisfy these two conditions as well. For any chore $c\in Q'$, let $f(c)=c'$ where chore $c$ and chore $c'\in H'$ have a same index.

Now we prove that $\vai{c}\le\vai{f(c)}$. Let $j$ be the index for chore $c$.  When Algorithm \ref{alg-proper} allocates chore $f(c)$ to bundle $\alloci[j]$, it will choose the largest possible chore $c'$ such that $\vai{\items[j]\cup c'}\le s_i$. Deduce from our assumption for the index of chore $c$, we know that chore $c$ has not been allocated when  Algorithm \ref{alg-proper} deal with bundle $\alloci[j]$. Thus, we have $\vai{c}\le\vai{f(c)}$.
\end{proof}


%From Claim \ref{claim-lessthan}, we can prove the following.
%So far we prove there is a desirable injective  function $f:Q\rightarrow H$. Notice that both set $Q$ and $H$ are subsets of set $\items$. 
Next we analysis the remaining chores from sets $\items\setminus H$ and $\items\setminus Q$.
\begin{claim}\label{claim-injective}
There is an injective function $g:\items\setminus H\rightarrow \items\setminus Q$ such that  $\vai{c}\le\vai{g(c)}$ for any chore $c\in \items\setminus H$.
\end{claim}  
\begin{proof}%[\bf Proof of Claim \ref{claim-injective}]
By Claim \ref{claim-lessthan}, suppose that $f:Q\rightarrow H$ is an injective function such that  $\vai{c}\le\vai{f(c)}$ for any chore $c\in Q$. Let $f^{0}:\items\rightarrow \items$ be an identity function.  For any integer $k>0$, let $f^{k}(c)=f(f^{k-1}(c))$ if $f^{k-1}(c)\in Q$. We construct $g$ such that $$g(c)=f^{w}(c)\text{ s.t. } w=\min\{k\mid f^{k}(c)\in \items\setminus Q\}.$$

First, we prove that for any $c\in\items\setminus H$, the mapping $g(c)$ is well-defined. For any chore $c\in\items\setminus(Q\cup H)$, we have $f^{0}(c)=c\in\items\setminus Q$. So for those chores, we have $g(c)=c$. For any chore $c\in Q\setminus H$, we prove that there must exist a $k$ such that $f^{k}(c)\in\items\setminus Q$. Suppose that there is no such $k$. There must exist two integers $k_1<k_2$ such that  $f^{k_1}(c)=f^{k_2}(c)$. Since function $f$ is injective, we have that $$c=f^{0}(c)=f^{k_1-k_1}(c)=f^{k_2-k_1}(c)\in H.$$ Because we have assumed that $c\in\items\setminus H$, it is a contradiction. Therefore, function $g$ is well-defined. 


Second, we prove that the function $g$ is injective. Suppose that there are two chores $c_1,c_2\in \items\setminus H$ such that $g(c_1)=g(c_2)$. Then there exist two integers $k_1,k_2$ such that $g(c_1)=f^{k_1}(c_1)=f^{k_2}(c_2)=g(c_2)$. Recall that $f$ is injective. If $k_1=k_2$, then $c_1=c_2$. It is impossible. Let us assume that $k_1<k_2$. Then, we have  $c_1=f^{0}(c_1)=f^{k_2-k_1}(c_2)\in H$. It is a contradiction to the range of chore $c_1$. Thus, function $g$ is injective. 

As  $\vai{c}\le\vai{f(c)}$ for any chore $c$, we have $\vai{c}\le \vai{f^{w_i}(c)}=\vai{g(c)}$.
\end{proof}


The set $\items\setminus Q$ is exactly the set $\bigcup_{j>k}\alloci[j]^*$. By Claim \ref{claim-injective}, we are able to allocate set $\items\setminus H$ into $n-k$ bundles such that no bundle with valuation more than $s_i$. Then by Lemma \ref{lem-monotone}, Algorithm \ref{alg-proper} will allocate all remaining chores by the threshold $s_i$. So Algorithm \ref{alg-proper} will return ``Yes" on the threshold $s_i$.


\end{proof}


\begin{comment}
\begin{proof}

%Without loss of generality, we assume $\mMS{i}=1$.
Let $H$ denote the set of chores which are allocated in the for-loop of line \ref{inalg-after-big}.   Let  $k=|\larg{i,s_i/2}|$ be the number of really large chores.  Let $\allocs$ be the allocation output by Algorithm \ref{alg-proper} on input agent $i$ and threshold $s_i$.  After line \ref{inalg-after-big} of threshold testing, the set of remaining chores is $Q=\larg{i,s_i/4}\setminus(H\cup \larg{i,s_i/2})$ i.e. the chores that are valued between $s_i/4$ and $s_i/2$ and have not filled in bundles with chores in $\larg{i,s_i/2}$. Equivalently, the set $Q=\cup_{j>k}\alloci[j]$. To prove the statement, we will prove the following property is true.

\bigskip
{\bf Property $P$:} The chores in the set $Q$ could be allocated to $n-k$ bundles such that no bundle is greater than $s_i$. 
\bigskip

  Since the for-loop in line  \ref{inalg-after-big} is similar to Algorithm \ref{alg-approx}, by Lemma \ref{lem-monotone} and the proof of Theorem \ref{thm-exist}, it is easy to see that all chores can be allocated in the testing.

%Without loss of generality, we assume that $\mMS{i}=1$. 
Let $\allocs'$ be an allocation such that $\max_j\vai{\alloci[j]'}\le s_i$. By our assumption, such kind allocation $\allocs'$ exists. Let bundle collection $\bundles^{0}=\allocs'\cap \larg{i,s_i/4}$. Notice that there is no bundle of allocation $\allocs'$ containing two chores from $\larg{i,s_i/2}$, if $s_i\ge\mMSi$. So we can assume that each chore $\items[j]$ is contained in bundle $\bundlei[j]$, for $j\le k$.  From the code in line \ref{inalg-allocate},  we have $\bundlei[j]^{0}[1]=\alloci[j][1]$ for $j\le k$.%, where $\{\alloci[j]\}_{j\le k}$ are bundles generated by the threshold testing algorithm  before the line \ref{inalg-after-big}. 
%Let $H^*=(\cup_{j\le k}\bundlei[j])\setminus(\cup_{j\le k}\bundle[j][1])$ be the set of chores  that are valued between $s_i/4$ and $s_i/2$ and allocated with with a chore in $\larg{i,s_i/2}$ in allocation $\allocs'$.
%\begin{claim}\label{claim-H-is-large}
%For the set $H$ and $H^*$, we have $|H^*|\le |H|$ and $\vai{H^*[j]}\le \vai{H[j]}$ for all $j\le |H^*|$.
%\end{claim}
%\begin{proof}
%We first prove $|H^*|\le |H|$ by the contradiction. Suppose $|H^*|> |H|$.
%\end{proof}

%We will construct bundles $\bundlei[j]^*$ for $j>k$ such that $$\vai{\bundlei[j]^*}\le\vai{\bundlei[j]}\text{ and }Q=\cup_{j>k}\bundlei[j]^*.$$


We will iteratively construct bundle collection $\bundles^{h}$ such that no bundle will greater than $s_i$ and when $h=|H|$ we have $\cup_{j>k}\bundlei[j]^{|H|}=Q$. Please recall the definitions of $MOVE$ operation and $SWAP$ operation in Lemma \ref{lem-no-larger-2/9}.
%We  will show that we can swap chores so that bundle $\bundlei[j]=\alloci[j]$ and $\vai{\bundlei[j]}\le s_i$ for all $j>k$.  
  We do the following to construct $\bundles^{h}$ from $\bundles^{h-1}$: Let $j=h$ and $\alloci[j']$ be the bundle containing the chore $H[j]$ in allocation $\allocs$. And then,
\begin{itemize}
\item $|\bundlei[j']^{h-1}|=1$:  Bundle collection $\bundles^{h}=MOVE(\bundles^{h-1}, j',H[j]).$  %Move the chore $H[j]$ to bundle $\bundlei[j']$.
\item $|\bundlei[j']^{h-1}|=2$:   Bundle collection $\bundles^{h}=SWAP(\bundles^{h-1},\bundlei[j']^{h-1}[2],H[j]).$  %Swap the chore $\bundlei[j'][2]$ with the chore $H[j]$.
\end{itemize}
Notice that in each construction step, we make $\bundlei[j']^{h}=\alloci[j']$.
%Notice that $j'\le k$ and from the construction process we should have $|\bundlei[j']^{h-1}|\le 2$.  

First we show that, except chores in set $H$, there is no other chore in set  $\larg{i,s_i/4}\setminus \larg{i,s_i/2}$ in bundle $\bundlei[j]^{|H|}$ for $j\le k$. Notice that bundle $\bundlei[j']^{|H|}=\alloci[j']$ for all $j'$ that bundle $\alloci[j']$ contains a chore in set $H$.
Suppose there is a chore $c$ such that $c\in\bundlei[j']^{|H|}$ for some $j\le k$ and $c\in \larg{i,s_i/4}\setminus \larg{i,s_i/2}\setminus H$. The testing algorithm should allocate chore $c$ in bundle $\bundlei[j']^{|H|}$ at  the for-loop in line \ref{inalg-pre-big}, as there is  enough space to allocate it. Thus, it is impossible. This implies that bundle $\bundlei[j']^{|H|}=\alloci[j]$ for all $j\le k$, which means $\cup_{j>k}\bundlei[j]^{|H|}=Q$.

Now we show that no bundle in bundle collection $\bundles^{h}$  is greater than $s_i$.
It is easy to see that when $|\bundlei[j']^{h-1}|=1$, if no bundle is greater than $s_i$, then after the $MOVE$ operation, there is still no bundle greater than $s_i$. When $|\bundlei[j']^{h-1}|=2$, we prove that  $\vai{\bundlei[j']^{h-1}[2]}\le \vai{H[j]}$. Suppose $\vai{\bundlei[j']^{h-1}[2]}> \vai{H[j]}$.  We prove that chore $\bundlei[j']^{h-1}[2]\notin H$. In our construction, we deal with $j$  from 1 to $|H|$. Therefore, the chores in $H$ larger than $H[j]$ have already allocated to other bundles. It means chore $\bundlei[j']^{h-1}[2]\notin H$.
 However, according to the algorithm, chore $\bundlei[j']^{h-1}[2]$  should  be allocated at  the for-loop in line \ref{inalg-pre-big}.  Because bundle  $\alloci[j']$ have enough space at the time algorithm deal with the chore $\bundlei[j']^{h-1}[2]$. Therefore, this situation cannot happen. So $\vai{\bundlei[j']^{h-1}[2]}\le \vai{H[j]}$. In this case, only bundle $\bundlei[j']^{h-1}$ will increase value. Since $\bundlei[j']^{h}=\alloci[j']$, there is no bundle greater than $s_i$. 
 
 By our construction of bundle collection $\bundles^{|H|}$, the property $P$ is proved. And so the statement of this lemma. 
 \end{proof}
 \end{comment}


\subsection{Efficient approximation algorithm}
Now we present the following approximation algorithm for \amMS{5/4} allocation.

\begin{algorithm}[H]
\KwIn{An IDO instance $\inst$}
\KwOut{An allocation  $\allocs$ of $\inst$}
\BlankLine

         \For{$i\in\agents$}
         {
         	Let $l_i=\max\left\{\vai{\items}/n,\vai{\items[1]}\right\}$ and $r_i=2l_i$.\;\label{inalg-upper-bound}
         With lower bound $l_i$ and upper bound $r_i$, binary search for the minimal integer  $s_i$  such that Algorithm \ref{alg-proper} return Yes on input $(\val,s_i)$\;

%		\While{$r_i-l_i\ge 1$}
%		{
%		 	$mid=(l_i+r_i)/2$\;
%			\eIf{Algorithm \ref{alg-proper} return Yes on input $(\val, mid)$} {$r_i= mid$\;}
%			{$l_i=mid$\;}
%		}
%		$s_i=\lceil l_i\rceil$\;
%		\If{Algorithm \ref{alg-proper} return No on input $(\val,s_i)$}{$s_i=s_i+1$\;}
%		\tcp*[h]{Binary search for the minimal integer which can pass threshold testing}\;
	
         }
         Run Algorithm \ref{alg-approx} on input $\inst,\left(\frac{5}{4}\cdot s_1,\dots,\frac{5}{4}\cdot s_n\right)$\;\label{inalg-call-approx}
         Let $\allocs$ be the output of Algorithm \ref{alg-approx}\;
	
\Return{$\allocs$}
\caption{Polynomial time algorithm for 5/4 approximation}\label{alg-poly}
\end{algorithm}

%for Algorithm \ref{alg-poly}:
{\bf Remark:}  The value $r_i=2l_i$ from line \ref{inalg-upper-bound} is an upper bound of $\mMSi$. This can be deduced from the 2 approximation algorithm of the job scheduling problem~\cite{graham1966bounds}.


To analyze the correctness of Algorithm \ref{alg-poly}, we  focus on the agent who gets the last bundle, which is denoted by $\last$. %And assume that $s_{\last}=1$.
First we argue that no small chores left unallocated. 
\begin{lemma}\label{lem-no-less-1/4}
If the threshold $s_{\last}\ge \vai[\last]{\items}/n$, then after Algorithm \ref{alg-poly} terminates, all chores $c\in \smal{\last,s_{\last}/4}$ will be allocated.
\end {lemma}
\begin{proof}
By the same argument as Lemma \ref{lem-no-less-2/9}, if there is a chore $c\in \smal{\last,s_{\last}/4}$ left, then every bundle is greater than $s_{\last}$. In the algorithm, we have set a lower bound $s_{\last}\ge \vai[\last]{\items}/n$ for the binary search. If the value of every bundle is greater than $s_{\last}$, the sum of valuations of all bundles will grater than $ \vai[\last]{\items}$. This is impossible. Thus we prove the lemma.
\end{proof}


Next we analyze what happened to the large chores in the allocation. The idea of the proof is similar to what we have done for Lemma \ref{lem-no-larger-2/9}. The key difference is that the benchmark allocation is the one generated by the threshold testing, but not a \mmax~allocation like Lemma \ref{lem-no-larger-2/9}. %on input agent $\last$ and threshold $s_{\last}$.  
We compare the output of Algorithm \ref{alg-poly} with the benchmark allocation to argue that all chores will be allocated.% And then argue that Algorithm \ref{alg-poly}  will always allocate larger and more chores than the benchmark.

%Let $\allocs$ be the allocation returned by Algorithm \ref{alg-poly}. And let bundle $\alloci^*=\alloci\cap G(\last, s_{\last}/4)$ consist of large chores from bundle $\alloci$. Let $D_k=\cup_{i\ge k}\alloci^*$ be the set of large chores from later generated bunldes. Let $\bundlei$ be the bundle which is the $i$-th bundle generated by the threshold testing algorithm on input $s_{\last}$. Let $P_k=\cup_{i\ge k}\bundlei$. We will prove the following lemma which directly imply that no chore $c\in G(\last,s_{\last}/4)$ left.
\begin{lemma}\label{lem-no-grater-1/4}
%For each $k$, there exists an injective function $f_k:D_k\rightarrow P_k$ such that $\vai[\last]{c}\le \vai[\last]{f_k(c)}$ for all  $c\in D_k$.
After Algorithm \ref{alg-poly} terminates, all chores $c\in \larg{\last,s_{\last}/4}$ will be allocated.
\end{lemma}
\begin{proof}[Proof sketch]
Please see Appendix \ref{apd-lemma-no-1/4} for the full proof.  Here we give a high level idea of the proof. After binary search, we have a threshold value $s_{\last}$ for the last agent $\last$, which is  a lower bound of $\mMSi[\last]$. Let $\bundles$ be the allocation that the threshold testing algorithm generated inside itself upon inputting agent $\last$ and value $s_{\last}$. Let $\allocs$ be the allocation returned by Algorithm \ref{alg-poly}. We will try to compare allocation $\allocs$ and allocation $\bundles$ from agent $\last$'s perspective.  

When comparing these two allocations, we observe that, for any $k$, the set of the first $k$ bundles of allocation $\allocs$  ($\bigcup_{i\le k}\alloci$) always contains larger and more chores than allocation $\bundles$ ($\bigcup_{i\le k}\bundlei$). Particularly, we prove by induction that we can maintain an injective mapping from chore set  $\bigcup_{ k<i\le n}\bundlei$ to set $\bigcup_{k< i\le n}\alloci$ such that each chore $c$ is mapped to a chore with valuation no less than $c$. 
\end{proof}

With all these lemmas, now we can prove the following theorem. 

\begin{theorem}\label{thm-poly}
%If all valuations are integers, 
For integer valuations, Algorithm \ref{alg-poly} will output a 5/4 approximation maximin share allocation in $O(nm\log m+n^2)$ time.
\end{theorem}
\begin{proof}
The correctness of Algorithm \ref{alg-poly} is directly implied by Lemma \ref{lem-no-less-1/4} and Lemma \ref{lem-no-grater-1/4}. We only need to analyze the time complexity of our algorithm. The running time of the threshold testing is about $O(m\log m +n)$. As valuations are all integers, the number of iterations of binary search depends on the length of the representation of each integer (usually it can be considered a constant). 
%the binary search could be done in a constant number of iterations. %\footnote{\label{fn-binary}Usually, in computer program, the length of the representation of a number (valuation) is a constant. After a constant times of iterations, we will reach the minimum unit of value. If there is no the issue of accuracy (e.g. all valuations are integers), then we will get an exact lower bound from binary search.} 
 And we repeat the binary search $n$ times for each agent respectively. Finally, Algorithm \ref{alg-approx} terminates in time $O(nm\log m)$. Combining all these, the total running time of our algorithm is $O(nm\log m+n^2)$.
\end{proof}


%Obviously the allocation is 5/4 approximation. The question is that  whether the algorithm can allocate all items. To answer this question, we can focus on the agent who get the last bundle.    Without loss of generality, we assume that the agent $n$ is the one who get the last bundle. The whole proof will break into two parts. In the first part, we will show that if we can allocate all big items (item valued more than 1/4) in agent $n$'s perspective, then the algorithm will allocate all items. In the second part, we will show that the algorithm can allocate all big items.







%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\begin{comment}
Obviously, for each agent, he/she gets a bundle with value no more than 5/4. The question is that  whether the algorithm can allocate all items. To answer this question, we can focus on the agent who get the last bundle. Without loss of generality, we assume that the agent $n$ is the one who get the last bundle. The proof will follow agent $n$'s view of the whole process.

We call a chore $c$ \emph{little} if $\vai[n]{c}\le1/4$. First, we prove no little chore will left.
\begin{lemma}\label{lem-no-little}
There is no little chore left after algorithm \ref{alg-5/4} stops.
\end{lemma}
\begin{proof}
Suppose there is a little chore $c$ left after algorithm stops. We prove that each bundle $\alloci$ satisfy the inequality $\vai[n]{\alloci}>1$. The argument is simple. Since chore $c$ is left, then the inequality $\vai[n]{\alloci\cup c}>5/4$ holds for all $i\in[n]$. Otherwise, chore $c$ will be allocated to the bundle which does not satisfy that inequality according to the algorithm. Therefore, $\vai[n]{\alloci}>1$ holds for all $i$. However, if \mmax is 1, then the total value should $\vai[n]{\items}\le n$. Combining these, we get a contradiction.
\end{proof}

%Give a high level overview of the lemma. intuition
Symmetrically, a chore $c$ is  \emph{big} if $\vai[n]{c}>1/4$.
For the big chores, we will compare two allocations $\allocs$ and  $\allocs^*$, where $\allocs$ is returned by the algorithm and $\allocs^*$ is some allocation that maximum bundle of $\allocs^*$ is valued equal to \mmax for agent $n$. The high level idea of the proof is that
%Notice that how little items allocated to the bundles does not influence the allocation of big items. As the big one always have the priority to be considered first.

%Define the sequence $A^*$ from largest to smallest for optimal allocation of agent $n$. Define  Define mapping function

Without loss of generality, we can assume the bundles in $\allocs$ and $\allocs^*$ are sorted as following:
\begin{itemize}
\item For any $j$, the bundle $\alloci[j]\in\allocs$ is generated by the algorithm when $k=j$ of the for loop in line \ref{inalg-loop}.
\item For any $\alloci[j]^*\in\allocs^*$, we use $b_j$ to denote the largest chore in $\alloci[j]^*$. The allocation $\allocs^*$ is sorted as $b_j\ge b_k$ if and only if $j\le k$.
\end{itemize}

Now focus on the big chores. Let $S=\{c\mid \vai[n]{c}>1/4\}$ denote the set of big chores. Define the bundle $\bundlei$ as $\alloci\cap S$ and bundle $\bundlei^*$ as $\alloci^*\cap S$. Let $G_k=\bigcup_{i\ge k}\bundlei$ and $G_k^*=\bigcup_{i\ge k}\bundlei^*$.
The following lemma will show a relationship between $G_k$ and $G_k^*$, which directly imply  no big chore will left.
\begin{lemma}\label{lem-no-big}
For each $k$, we have that $\vai[n]{G_k}\le\vai[n]{G_k^*}$.
\end{lemma}
\begin{proof}
To prove this lemma, we will prove a stronger statement. For each $k$, there exists an injective function $f_k:G_k\rightarrow G_k^*$ such that $\vai[n]{c}\le \vai[n]{f_k(c)}$ for all  $c\in G_k$. We prove this statement by induction.

When $k=1$, the identical mapping will work. Suppose when $k=l$, this statement is true. Then we prove, when $k=l+1$, the statement is also true. If $G_k=\emptyset$ or $G_k^*=\emptyset$, then we can stop here as the statement becomes trivial. Otherwise, we prove it by case analysis.
\begin{itemize}
\item $|\bundlei[k]^*|=1$: Let $b_k$ be the largest chore in $\bundlei[k]$.  Recall that $b_k^*$ is the largest chore in $\bundlei[k]^*$. Let $r=f_k^{-1}(b_k^*)$ be the inverse image of $b_k^*$. If $r=\emptyset$ or $r=b_k$, then it is easy to verify that the function $f_{k+1}(c)=f_k(c)$ for all $c\in G_{k+1}$ is a valid function. For the case $r\neq b_k$, we have that $\vai[n]{r}\le\vai[n]{b_k}\le\vai[n]{f_k(b_k)}$. Therefore, in this case, let $f_{k+1}(r)=f_k(b_k)$ if $r\in G_{k+1}$, and let $f_{k+1}(c)=f_k(c)$ for all $c\in G_{k+1}$ and $c\neq r$. We can see that $f_{k+1}$ is a valid function.

\item $|\bundlei[k]^*|=2$: Let $b_k^1$ be the largest chore in $\bundlei[k]^*$ and $b_k^2$ be the remaining chore in $\bundlei[k]^*$. First we can adjust function of $b_k$ and $b_k^1$ with the same argument as above. Let $r=f_k^{-1}(b_k^2)$. If $|\bundlei[k]|=1$, then $r$ must be $\emptyset$. Otherwise, $r$ can be allocated to $\bundlei[k]$ and then $|\bundlei[k]|$ should not be 1.

If $|\bundlei[k]|\ge 2$, then after removing $b_k^1$ and $b_k^*$, we can adjust function of $b_k^2$ and second largest chore in $\bundlei[k]$ with same argument as above. Then we can get a valid function $f_{k+1}$.

\item $|\bundlei[k]|^*=3$: Let $b_k^1$, $b_k^2$ and $b_k^3$ denote the chores in $\bundlei[k]^*$ such that $\vai[n]{b_k^1}\ge\vai[n]{b_k^2}\ge\vai[n]{b_k^3}$. We also can handle $b_k^1$ and $b_k$ with the same argument. Let  $r_2=f_k^{-1}(b_k^2)$  and  $r_3=f_k^{-1}(b_k^3)$.  If $|\bundlei[k]|=1$, then we have $r_2=r_3=\emptyset$. Then, we can construct $f_{k+1}$ by  keeping $f_{k+1}=f_k$ for other chores

 If $|\bundlei[k]|= 2$, then we must have that one of $r_2,r_3$ is $\emptyset$.  As $\vai[n]{b_k^2}>1/4$ and $\vai[n]{b_k^3}>1/4$, we have $\vai[n]{b_k^1}< 1/2$ and $\vai[n]{b_k^1\cup b_k^2}<3/4$. If $r_2,r_3$ both are not $\emptyset$, we have $\vai[n]{\bundlei[k]\cup r_2}\le\vai[n]{b_k^1\cup b_k^1\cup r_2}\le\vai[n]{b_k^1}+\vai[n]{b_k^1\cup b_k^2}<5/4$. And the same holds for $\bundle[k]\cup r_3$. This indicates that we always can add chores to make $|\bundlei[k]|\ge3$. So one of $r_2,r_3$ must be $\emptyset$. In addition, if one of $r_2,r_3$ is not $\emptyset$, then that one must be allocated to $\bundlei[k]$. So just keeping $f_{k+1}=f_k$ for all other chores is enough.

If $|\bundlei[k]|\ge 3$, then apply the argument of the case for $|\bundlei[k]^*|=2$ and $|\bundlei[k]|\ge 2$ to $b_k^2$ and $b_k^3$. After that we can obtain a valid function $f_{k+1}$.
\end{itemize}
\end{proof}

With these lemmas, we can prove the theorem.
\begin{proof}[Proof of Theorem \ref{thm-5/4-exist}]
Lemma \ref{lem-no-little} shows there is no little chore left and lemma \ref{lem-no-big} shows there is no big chore left. Therefore, at the end, all chores are allocated.
\end{proof}

\end{comment} 

==> EC 21 submission/prelim.tex <==
We introduce some basic definitions and concepts for our model here.   An instance of the problem of dividing indivisible chores is denoted as $\inst=\langle\agents,\items,\va\rangle$, where $\agents$ is the set of agents, $\items$ is the set of chores, and $\va$ is the collection of all valuations.  For simplicity, we assume that the set of agents is $\agents=[n]$ and the set of chores is $\items=\{c_1,c_2,\dots,c_m\}$, where $n$ is the number of agents and $m$ is the number of chores. The  collection of all valuations $\va$ can be equivalently written  as $\valist$. For each agent $i$, the corresponding valuation function $\val:2^{\items}\rightarrow \mathbb{R}^+$ is additive, i.e., $\vai{S}=\sum_{c\in S}\vai{c}$ for any set  $S\subseteq\items$. 

Notice here we use non-negative valuation function which is the same as goods setting. However, the meaning is the opposite. Intuitively, the value is equivalent to the workload for $S$. So each agent wants to minimize her value. An allocation $\allocs=\alloclist$ is a $n$ partition of all chores $\items$ which  allocates all chores $\alloci$ to each agent $i$. We denote all possible allocations as the set $\Pi_n(\items)$.

%\xin{Place a right position }



The \mmax~%\footnote{Based on the mathematical form, minimax would be a more proper name for this definition. Here we follow previous literatures to call it as maximin share, which is defined on negative values. It should be no confuse that they are exactly the same definition. The reason we define it like this is that the definition from positive values can help us think this problem in a different angle and easily make a connection with job scheduling and bin packing problem.  } 
of an agent $i$ is defined as  $$\mMSi=\min_{\allocs\in\Pi_n(\items)}\max_{j\in[n]}v_i(\alloci[j]).$$


Here compare to maximin share, minimax share may be a more proper name. Since we minimum the value (duty/work load) that the agent can guarantee if she is the cutter. If one use negative value for chores, it can still be called maximin share, and we follow the literature to use the term ``maximin" and use positive value for notational simplicity. 

%In the following context, when $S=\mathcal{M}$, we simply call this value $k$-maximin share of agent $i$ and denote it by \kMMS{k}{i}. With the measure of maximin share, we can define the maximin share allocation..

Following is a formal definition for \mmax~allocation.
\begin{definition} [Maximin share allocation]
 An allocation $\allocs\in\Pi_n(\items)$ is a \mmax~(\mMS) allocation  if $$\forall i\in\agents, \vai{\alloci}\le \mMSi.$$
\end{definition}
An allocation $\allocs$ is called \emph{\amMS{\alpha} allocation} if the inequality $\vai{\alloci}\le\alpha\cdot\mMSi$ holds for any agent $i$.


For the proof of our algorithm, the following is a useful definition.
\begin{definition}[Maximin share allocation for agent $i$]
 An allocation $\allocs\in\Pi_n(\items)$ is a \mmax~allocation for agent $i$,  if $$\forall j\in\agents, \vai{\alloci[j]}\le \mMSi.$$
\end{definition}



\begin{definition}[Identical ordinary preference]
An instance $\inst$ is called \emph{identical ordinary preference} (IDO) if there is a permutation $\sigma$ on $[m]$ such that, when $j\ge k$, we have the inequality $\vai{c_{\sigma(j)}}\ge\vai{c_{\sigma(k)}}$ holds for any agent $i$.
\end{definition}

As we will constantly use the notion of $j$-th largest chore of a bundle in the description of the algorithm and the proof, here we give a notation for it.

\begin{definition}\label{def-j-th}
Given an instance $\inst$ and a bundle (a set of chores) $\bundle\subseteq\items$, we denote by $\bundle[i,j]$   the $j$-th largest chore in bundle $\bundle$ from agent $i$'s perspective. For IDO instance, since every agent share the same ordinary preference, we will shortcut it as $\bundle[j]$.
\end{definition}

For example, for an IDO instance, the item $\items[1]$ and  the item $\items[2]$ would be the largest and the second largest chore of all. 

==> EC 21 submission/special.tex <==
\begin{comment}
In practical, we may face more structural instances. In this section, we try to explore the power of our algorithmic framework on some special cases. In particular, we consider the following two  cases: 1) Two-agent case.  When we consider daily life problems, two-agent case may be the most common situation. 2) All agents share the same valuation. This case is known as job scheduling/load balancing problem, which has received many attentions from optimization community.   Regardless of limitations for general instances, we prove better results for these two cases. 
%In practical, we may not need the full power of our framework. Here we show some better results on such cases. 

\subsection{Two agents}
\xin{two agent np-hard}

By our algorithmic framework we can design the following algorithm for two-agent case:
\begin{itemize}
\item Binary search
\item cut-and-choose
\end{itemize}

\begin{theorem}\label{thm-2-agent}
For two-agent case, when valuations are all integers, we can find an \amMS{8/7} allocation in $O(m\log m )$ time, where ratio $8/7$ is tight for our algorithm. 
\end{theorem}
Please refer Appendix \ref{apd-thm-2-agent} for the proof.

%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%


\subsection{Job scheduling}
\end{comment}

The job scheduling problem is one of the fundamental discrete optimization problems. Here we particularly consider the model that minimizes the execution time for scheduling $m$ jobs on $n$ identical machines. It could be viewed as a special case of chore allocation, where all agents have the same valuation. From this perspective, we show how to apply our algorithmic framework to this problem.

%There are many variants of this problem. Here we consider the model that minimize the execution time for scheduling $m$ jobs on $n$ identical machines. 
The problem of job scheduling is proved to be NP-hard in~\cite{DBLP:books/fm/GareyJ79}. And later, the polynomial time approximation scheme (PTAS) for this problem was discovered and developed~\cite{alon1998approximation,jansen2010eptas,jansen2016closing}.
To the best of our knowledge, except those PTASs, there is no algorithm approximating optimal better than 4/3. From our algorithmic framework, we demonstrate an algorithm, which is simpler  and more efficient than the best PTAS, and achieves a better approximation ratio than other heuristics. 
% Best PTAS 2^{O(1/epsilon*log(1/epsilon)^4)}+ poly(n)
%We demonstrate an easy implement and really efficient 11/9 approximation algorithm for job scheduling problem. 
%Recently, \cite{della2018longest}


\begin{theorem}\label{thm-schedul}
%Algorithm \ref{alg-special} will 
When all valuations are integers, an 11/9 approximation of optimal scheduling can be found in $O(m\log m+n)$ time. 
\end{theorem}
\begin{proof}
%By the proof of Theorem \ref{thm-exist}, the value $s^*$ in the line \ref{inalg-min-value} of Algorithm \ref{alg-special} is at most $\frac{11}{9}\cdot\mMSi[1]$. As the valuations of each agent are same, the inequality $\vai{\alloci[j]}\le\frac{11}{9}\cdot\mMSi$ holds for any agent $i$ and bundle $j$. Therefore, the final allocation is 11/9 approximation to the optimal scheduling.

We first describe the algorithm for this problem. The algorithm  is similar to Algorithm \ref{alg-poly}, except for two modifications: 
\begin{itemize}
\item Change the threshold testing algorithm in binary search from Algorithm \ref{alg-proper} to the naive test which is introduced in section \ref{subsec-failure}.
\item Delete the for-loop, and compute one proper threshold from the valuation function.
\end{itemize}

As all agents share the same valuation function, the threshold obtained by the naive test obviously can apply to all agents. Then we can get an allocation such that no bundle exceeds the threshold. And by Lemma \ref{lem-monotone} , the threshold from binary search is not greater than $\frac{11}{9}\cdot\mMS$.

The time complexity of one testing is $O(m\log m+n)$. The number of iterations of binary search depends on the length of the representation of each integer (usually it can be considered a constant). %(Please refer footnote \ref{fn-binary} for the discussion of binary search.) 
Finally, Algorithm \ref{alg-approx} will be executed one more time. Thus, the complexity of our algorithm is $O(m\log m+n)$
\end{proof}



==> EC 21 submission/store.tex <==
\begin{proof}
Suppose $\allocs$ is the allocation returned by the algorithm and $\bundles$ is a \mmax~allocation for the last agent $\last$. Now we try to swap chores in \mmax~allocation $\bundles$ so that it will become the allocation $\allocs$. The proof is to analysis what happened in this swapping process. 

As we have shown in Lemma \ref{lem-no-less-2/9}, we do not need to consider small chores. So let us define the bundle $\alloci^*$ as $\alloci\cap \larg{\last,2/9}$ and the bundle  $\bundlei^*$ as $\bundlei\cap \larg{\last,2/9}$.
For the simplicity of the proof, we assume that all bundles are ordered by the largest chore in each bundle i.e. $\alloci[i]^*[1]\ge \alloci[j]^*[1]$  for all $i<j$. Notice that for the allocation $\allocs$, this order is exactly the order from the  for loop in line \ref{inalg-loop} of Algorithm \ref{alg-approx}.

%Without loss of generality, we can assume the bundles in $\allocs$ are sorted as following: For any $j$, the bundle $\alloci[j]\in\allocs$ is generated by the algorithm when $k=j$ of the for loop in line \ref{inalg-loop}. %And define the bundle $\alloci^*$ as $\alloci\cap \larg{\last,2/9}$ and the bundle  $\bundlei^*$ as $\bundlei\cap \larg{\last,2/9}$.
%\xin{Write more explanation before the definition}

%To prove this lemma, we will start with bundles $\bundlei^*$ and then generate bundles $\bundlei$ by swapping chores between bundles.
We start with bundle collection $\bundles^{(0)}=\left(\bundlei[1]^*,\dots,\bundlei[n]^*\right)$  for our swapping process. Bundle collection $\bundles^{(0)}$ is a \mmax~allocation of large chores. There are $n$ rounds  of the swapping process in total. In each round $t$, we generate a bundle collection $\bundles^{(t)}$ by swapping some chores in bundle collection $\bundles^{(t-1)}$, so that  bundle $\bundlei[t]^{(t)}=\alloci[t]^*$. Notice that we do not need to touch bundles with index strictly less than $t$ to fix bundle $\bundlei[t]^{(t)}$.  So we have $\bundlei^{(t)}=\alloci^*$ for all $i\le t$.
%At the beginning of the swapping process, Let bundle collection $\bundles^{(0)}=\left(\bundlei[1]^*,\dots,\bundlei[n]^*\right)$ include all $\bundlei^*$. Notice that $\larg{\last,2/9}=\cup_i\bundlei^*$.  Our target is to generate bundle collection $\bundles^{(t)}$ from $\bundles^{(t-1)}$ by  swapping chores between bundles, so that $\bundlei^{(t)}=\alloci^*$ for all $i\le t$. If this process can successfully proceed, then $\bundles^{(n)}=\left(\alloci[1]^*,\dots,\alloci[n]^*\right)$ which means all chores $c\in \larg{\last,2/9}$ are allocated.

If this swapping process could success to the round $n$, then all large chores are allocated in allocation $\allocs$, which implies the lemma.   To show this, we carefully specifiy the swapping process so that bundle collection $\bundles^{(t)}$ satisfies a good property. %We will prove this by induction.
%To prove this, we will show that, for $i>t$, bundles $\bundlei^{(t)}$  satisfies a good property by induction.

%The definitions of ``good" properties are in the below. Here we give a high level intuition for why ``good" bundle is good. There are two conditions. A bundle will be considered as ``good"  if it satisfies any of two conditions. 
%\begin{itemize}
%\item The fist condition states that the value of the bundle is upper bounded. It makes sure the number of large chores would not be greater than 4. This will make the case analysis possible.  Another good thing is that all initial bundles satisfy this condition. So we have the basis for the induction. 
%\item The second condition is about the sum of the largest chore and the least chore in a bundle. This condition could help us to analyze the number of chores after swapping. And we restrict the number of chores must be 4 before swapping. These two conditions could ensure that the swapping process would always swap a less valued chore to another bundle. 
%\end{itemize}
 % 1. contains all bundles at the beginning. 2. at most 4 large chores, wouldn't cause too much trouble. The second condition 1. though the swapping process, there is only such case that bundle could larger than 1. 2. we focus on the sum of largest and smallest chores, because in this way we can make sure 3 largest + 1 smallest will not exceed 11/9.

To introduce the good property, we need some definitions. Let $$U(\bundle)=\min_{c\in \bundle} \vai[\last]{c}+\max_{c\in\bundle}\vai[\last]{c}$$ denote the sum of largest and smallest chore in the bundle.

\bigskip
{\bf Good bundle:} A bundle $\bundle$ is \emph{good} if 1) $\vai[\last]{\bundle}\le1$ or, 2) $U(\bundle)<5/9\text{ and }|\bundle|=4.$ \xin{Write down the intuition for the definition}
\bigskip

These two conditions for a good bundle are corresponding to two types swapping which are mentioned in the high level idea description. 

Here we slightly abuse the concept ``good" for bundle collection.

\bigskip
{\bf Good bundle collection:}  A bundle collection $\bundles^{(t)}$ is \emph{good} if $\bundlei^{(t)}=\alloci^*$ for all $i\le t$, and for $i>t$ each bundle $\bundlei^{(t)}$ is good.
\bigskip

Clearly, the bundle collection $\bundles^{(0)}$ is good. %Suppose when $t=k$, the bundle collection $\bundles^{(t)}$ is good. We will prove, when $t=k+1$,  by swapping some chores from $\bundles^{(k)}$, we can construct a good bundle collection $\bundles^{(k+1)}$.
This would be the basis for our induction. Now we need to describe the swapping process.
To precisely do it, we introduce two operations $SWAP$ and $MOVE$, where the operation $SWAP$ would swap two chores and the operation $MOVE$ would move a set of chores  from their original bundles to a target  bundle.
%Here we introduce two operations that are very helpful in construction $\bundles^{(k+1)}$ from $\bundles^{(k)}$.

Given a bundle collection $\bundles$ and two chores $c_1$ and $c_2$, the $SWAP$ operation will generate a new bundle collection $\bundles^{\#}=SWAP(\bundles,c_1,c_2)$ such that: If $c_1=c_2$ or, $c_1$ and $c_2$ are in the same bundle, then $\bundles^{\#}=\bundles$; Otherwise
\begin{equation*}
 \bundlei^{\#}=
  \begin{cases}
   \bundlei & \text{if } c_1,c_2\notin \bundlei  \\
   (\bundlei\setminus c_1)\cup c_2       & \text{if } c_1\in\bundlei \\
   (\bundlei\setminus c_2)\cup c_1  & \text{if } c_2\in\bundlei
  \end{cases}
\end{equation*}
%This operation swaps chore $c_1$ and $c_2$.

Given a bundle collection $\bundles$, an  index $j\in\agents$ and a subset of chores $T\subseteq\items$, the $MOVE$ operation will generate a new bundle collection $\bundles^{\#}=MOVE(\bundles,j,T)$ such that
 \begin{equation*}
  \bundlei^{\#}=
   \begin{cases}
    \bundlei\setminus T & \text{if } i\neq j \\
    \bundlei\cup T      & \text{if } i=j \\
   \end{cases}
 \end{equation*}
 Notice that chores set $T$ could contain chores from different bundles. 
%This operation moves chores set $T$ from their original bundles to the bundle indexed by $j$.

%Let bundle $\bundlei^{(k+1)}=\alloci^*$ for $i\le k+1$. We will show how to construct remaining bundles i.e. $\bundlei^{(k+1)}$ where $i>k+1$.
%\xin{Give a reminder, but simplify this paragraph} 
%contains the largest chore among chores $\cup_{i\ge k+1} \bundlei^{(k)}$ (we can rename the bundle containing the largest chore to $\bundlei[k+1]^{(k)}$). %Let $\bundle(j)$ denote the $j$-th largest chore in the $\bundle$ from agent $\last$'s view.
%It is easy to see that $\bundlei[k+1]^{(k)}[1]=\alloci[k+1]^*[1]$, as Algorithm \ref{alg-approx} always allocates the largest chore of remaining to a new bundle. So, we only need  to take care of remaining chores from both bundles.

%\xin{Define two types swapping here, make argument easy?}
Now we describe and prove the correctness of  the swapping process by induction. Suppose that bundle collection $\bundles^{(k)}$ is good. We will swap and move some chores between bundle $\bundlei[k+1]^{(k)}$ and bundles with index greater than $k+1$, so that the bundle $\bundlei[k+1]^{(k)}$ would become bundle $\alloci[k+1]^*$.  Without loss of generality, we can assume that the largest chore in  bundle $\bundlei[k+1]^{(k)}$ and  bundle $\alloci[k+1]^*$ are the same, i.e. chore $\bundlei[k+1]^{(k)}[1]=\alloci[k+1]^*[1]$. This is the largest chore among  the set $\bigcup_{i\ge k+1} \bundlei^{(k)}$ by our assumption of the order of allocation $\allocs$ (The assumption made at the beginning of the whole proof).   
 By the condition of good bundle collection and the value of large chores, we know that  bundle $\bundlei[k+1]^{(k)}$ contains at most $4$ chores.
%For each chore $c\in \cup_i\bundlei^*$, we  know the valuation $\val[\last](c)>\frac{2}{9}$ and the valuation $\vai[\last]{\bundlei^*}\leq 1$. This implies that each $\bundlei^*$ contains at most $4$ chores. %During the swapping process, we keep the property that for $i>t$ each bundle $\bundlei^{(t)}$ contains at most $4$ chores. 
  Based on the size of bundle $\bundlei[k+1]^{(k)}$, we have the following case analysis.

%Now we show a delicate to swap some chores to make $\bundlei[k+1]^{(k)}$ to become $\bundlei[k+1]$. We show it in case analysis:
\begin{itemize}
\item $|\bundlei[k+1]^{(k)}|=1,2,\mbox{ and } 4$:  Let $d=|\bundlei[k+1]^{(k)}|$ be the cardinality of the bundle. 
By Claim \ref{claim-4chores}, we have that $|\alloci[k+1]^*|\ge |\bundlei[k+1]^{(k)}|$ and $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$ for $j\le d$.  For the first $d$ chores, we swap them one by one. Since we have $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$, after these swaps, some chores become smaller for  bundles with index larger than $k+1$. A good bundle will still be a good bundle.  If the cardinality $|\alloci[k+1]^*|>d$, then we just move remaining chores  to bundle $\bundlei[k+1]^{(k)}$. After we remove some chores, a good bundle will still be a good bundle. Therefore, when we get the  bundle collection $\bundles^{(k+1)}$, it is a good bundle collection. 


Mathematically, let bundle collection $G^{(1)}=\bundles^{(k)}$. The swapping of first $d$ chores  could be represented as the following form  $G^{(j)}=SWAP\left(G^{(j-1)},\bundlei[k+1]^{(k)}[j],\alloci[k+1]^*[j]\right)$ for $2\le  j\le d$. The bundle collection $G^{(d)}$ is the resulting bundle after these swaps.  And the moving operation to generate bundle collection $\bundles^{(k+1)}$ is equivalent to 
$$\bundles^{(k+1)}=MOVE\left(G^{(d)},k+1,\alloci[k+1]^*\right).$$ 

%For chores in bundle $\alloci[k+1]^*$, we move them  from their current bundles  to  bundle $\bundlei[k+1]^{(k)}$.
%Mathematical equivalently, for the bundle collection $\bundles^{(k+1)}$, we have  %$$\bundlei^{(k+1)}=\bundlei^{(k)}\setminus \alloci[k+1]^*\text{ for } i>k+1.$$
%Formally, we have
%$$\bundles^{(k+1)}=MOVE\left(\bundles^{(k)},k+1,\alloci[k+1]^*\right).$$

%The bundle with index larger than $k+1$ either does not change or remove some chores. Thus a good bundle is still good. This gives that bundle collection $\bundles^{(k+1)}$ is good.

%\xin{Write a new statement: $|\alloci[k+1]^*|\ge |\bundlei[k+1]^{(k)}|$ and $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$ }

%\item $|\bundlei[k+1]^{(k)}|=2$: First we have the cardinality  $|\alloci[k+1]^*|\ge 2$. Because Algorithm \ref{alg-approx}  can at least allocate chore $\bundlei[k+1]^{(k)}[2]$ to bundle $\alloci[k+1]^*$ as the second chore. This observation also implies valuation $\vai[\last]{\bundlei[k+1]^{(k)}[2]}\le\vai[\last]{\alloci[k+1]^*[2]}$. If chore $\bundlei[k+1]^{(k)}[2]\neq\alloci[k+1]^*[2]$, then we swap these two chores. And if there are more chores in bundle $\alloci[k+1]^*$ i.e. $|\alloci[k+1]^*|>2$, then we just move remaining chores from their current bundles  to $\bundlei[k+1]^{(k)}$. Mathematical equivalently,% for $i>k+1$, 
%we have
\begin{comment}
\begin{equation*}
 \bundlei^{(k+1)} =
  \begin{cases}
   \bundlei^{(k)}\setminus \alloci[k+1]^* & \text{if }  \alloci[k+1]^*[2]\notin  \bundlei^{(k)}\\
   \left(\bundlei^{(k)}\cup\bundlei[k+1]^{(k)}[2]\right)\setminus \alloci[k+1]^*      & \text{if } \alloci[k+1]^*[2]\in  \bundlei^{(k)} \\
  \end{cases}
\end{equation*}
\end{comment}
%$$\bundles^{(k+1)}=MOVE\left(SWAP\left(\bundles^{(k)},\bundlei[k+1]^{(k)}[2],\alloci[k+1]^*[2]\right),k+1,\alloci[k+1]^*\right).$$

%The bundle with index larger than $k+1$ either does not change or remove some chores. Thus a good bundle is still good. This gives that bundle collection $\bundles^{(k+1)}$ is good. \xin{Is it better to make it a claim?}

\item $|\bundlei[k+1]^{(k)}|=3$: By a similar argument as the above case, we have $|\alloci[k+1]^*|\ge 2$. Let $$G=SWAP\left(\bundles^{(k)},\bundlei[k+1]^{(k)}[2],\alloci[k+1]^*[2]\right)$$ be the bundle collection that  swap chore $\bundlei[k+1]^{(k)}[2]$ and chore $\alloci[k+1]^*[2]$.  Now we consider the following inequality:
\begin{equation}\label{ineq-2-3}
\vai[\last]{\left\{\alloci[k+1]^*[1],\alloci[k+1]^*[2], \bundlei[k+1]^{(k)}[3]\right\}}\le 11/9
\end{equation}

If the Inequality \ref{ineq-2-3} holds,  then we have $|\alloci[k+1]^*|\ge 3$ and $\vai[\last]{\bundlei[k+1]^{(k)}[3]}\le\vai[\last]{\alloci[k+1]^*[3]}$. For this case, we will swap chore $\bundlei[k+1]^{(k)}[3]$ and chore $\alloci[k+1]^*[3]$ and move remaining chores in bundle $\alloci[k+1]^*$ to bundle $\bundlei[k+1]^{(k)}$, i.e.
$$\bundles^{(k+1)}=MOVE\left(SWAP\left(G,\bundlei[k+1]^{(k)}[3],\alloci[k+1]^*[3]\right),k+1,\alloci[k+1]^*\right).$$

In this subcase, the bundle with index larger than $k+1$ either does not change or remove some chores. Thus a good bundle is still good. This gives that bundle collection $\bundles^{(k+1)}$ is good.

If the Inequality \ref{ineq-2-3} does not hold, then we move $\bundlei[k+1]^{(k)}[3]$ to the bundle where $\alloci[k+1]^*[2]$ comes from and then move  other chores in $\alloci[k+1]^*$  to $\bundlei[k+1]^{(k)}$. Let $j$ be an index of a bundle such that $\alloci[k+1]^*[2]\in\bundlei[j]^{(k)}$. Then, formally this process is
$$\bundles^{(k+1)}=MOVE\left(MOVE\left(G,j,\bundlei[k+1]^{(k)}[3]\right),k+1,\alloci[k+1]^*\right).$$

This is the most complicated case since $\bundlei[j]^{(k+1)}$ contains more item than $\bundlei[j]^{(k)}$. 
We prove that  bundle $\bundlei[j]^{(k+1)}$ is good in Claim \ref{claim-two-one}. And for other bundles with index larger than $k+1$, it either does not change or remove some chores.  Therefore, bundle collection $\bundles^{(k+1)}$ is good.

%\item $|\bundlei[k+1]^{(k)}|=4$:
%Using the property of good bundle,  we prove that $|\alloci[k+1]^*|\ge 4$ and $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$ for $j\le4$ in Claim \ref{claim-4chores}. For the first 4 chores, we swap them one by one. If the cardinality $|\alloci[k+1]^*|>4$, then we just move remaining chores from their original bundles  to $\bundlei[k+1]^{(k)}$.

%Formally the process is described as following.Let bundle collection $G^{(0)}=\bundles^{(k)}$ and bundle collection  $G^{(j)}=SWAP\left(G^{(j-1)},\bundlei[k+1]^{(k)}[j],\alloci[k+1]^*[j]\right)$ for $1\le  j\le 4$. We have
%$$\bundles^{(k+1)}=MOVE\left(G^{(4)},k+1,\alloci[k+1]^*\right).$$ 

%The bundle with index larger than $k+1$ either does not change or remove some chores. Thus a good bundle is still good. This gives that bundle collection $\bundles^{(k+1)}$ is good.
\end{itemize}

\begin{claim}\label{claim-4chores}
For the cases $|\bundlei[k+1]^{(k)}|=1,2,\mbox{ and }4$, we have the inequalities $|\alloci[k+1]^*|\ge |\bundlei[k+1]^{(k)}|$ and $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$ for $j\le|\bundlei[k+1]^{(k)}|$.
\end{claim}
\begin{proof}
For the case $|\bundlei[k+1]^{(k)}|=1$, it is trivial. For the case  $|\bundlei[k+1]^{(k)}|=2$, we notice that Algorithm \ref{alg-approx}  can at least allocate chore $\bundlei[k+1]^{(k)}[2]$ to bundle $\alloci[k+1]^*$ as the second chore. This would imply the cardinality  $|\alloci[k+1]^*|\ge 2$ and the valuation $\vai[\last]{\bundlei[k+1]^{(k)}[2]}\le\vai[\last]{\alloci[k+1]^*[2]}$.


For the case $|\bundlei[k+1]^{(k)}|=4$, first we prove that the inequality  $U(\bundlei[k+1]^{(k)})<5/9$ is true. Since bundle $\bundlei[k+1]^{(k)}$ is good, we have the condition $U(\bundlei[k+1]^{(k)})<5/9$ or  $\vai[\last]{\bundlei[k+1]^{(k)}}\le1$.
If the valuation $\vai[\last]{\bundlei[k+1]^{(k)}}\le1$, then as  any chores in the bundle is greater than 2/9,  we have $$U(\bundlei[k+1]^{(k)})=1-\text{value of the other two chores}<1-2\cdot 2/9=5/9.$$

Now we prove the inequality $$3\cdot \vai[\last]{\bundlei[k+1]^{(k)}[1]}+\vai[\last]{\bundlei[k+1]^{(k)}[4]}\le11/9.$$
Suppose $3\cdot \vai[\last]{\bundlei[k+1]^{(k)}[1]}+\vai[\last]{\bundlei[k+1]^{(k)}[4]}>11/9$. Let $x$ be the value of $\vai[\last]{\bundlei[k+1]^{(k)}[4]}$. Then we have
\begin{align*}
11/9&<3\cdot \vai[\last]{\bundlei[k+1]^{(k)}[1]}+\vai[\last]{\bundlei[k+1]^{(k)}[4]}\\
&<3\cdot(5/9-x)+x \tag{by $U(\bundlei[k+1]^{(k)})<5/9$}
\end{align*}
This implies $x<2/9$. This contradicts our assumption that $c\in \larg{\last,2/9}$.

Notice that $\vai[\last]{\bundlei[k+1]^{(k)}[1]}$ is the value of largest chore among the remaining. So the inequality suggests that even if we allocate 3 largest chores, there is still a space for the chore $\bundlei[k+1]^{(k)}[4]$. So the first 3 chores being allocated to bundle  $\alloci[k+1]^*$ must be the largest 3 chores. So  $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$ for $j\le3$.

As we have $|\bundlei[k+1]^{(k)}|=4$, the chore $\bundlei[k+1]^{(k)}[4]$ would not be one of first 3 chores allocated to bundle  $\alloci[k+1]^*$. Since there is a space for  the chore $\bundlei[k+1]^{(k)}[4]$, the forth chore being allocated to bundle  $\alloci[k+1]^*$ should at least as large as  the chore $\bundlei[k+1]^{(k)}[4]$.  Combining all these, we have $|\alloci[k+1]^*|\ge 4$ and $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$ for $j\le4$.
\end{proof}


\begin{claim}\label{claim-two-one}
For the case $|\bundlei[k+1]^{(k)}|=3$ and Inequality \ref{ineq-2-3} does not hold, %$\vai[\last]{\alloci[k+1]^*[1]\cup\alloci[k+1]^*[2]\cup \bundlei[k+1]^{(k)}[3]}> 11/9$,
after all $SWAP$ and $MOVE$ operations, bundle $\bundlei[j]^{(k+1)}$ is good, where $j$ is the index such that the chore $\alloci[k+1]^*[2]\in\bundlei[j]^{(k)}$.
\end{claim}
\begin{proof}
%Suppose  bundle $\bundlei[j]^{(k)}$ contains the chore $\alloci[k+1]^*[2]$. We prove that if $\bundlei[j]^{(k)}$ is good, then after remove $\alloci[k+1]^*[2]$ and  then add $\bundlei[k+1]^{(k)}[2]$ and  $\bundlei[k+1]^{(k)}[3]$, $\bundlei[j]^{(k)}$ is good is still good.
We first prove two useful observations.
\begin{observation}\label{obser-2is-largest}
The chore $\alloci[k+1]^*[2]$ must be the largest chore in the bundle $\bundlei[j]^{(k)}$.

\begin{proof}
Because $|\bundlei[k+1]^{(k)}|=3$ and it is good, so $\vai[\last]{\bundlei[k+1]^{(k)}}\le1$, which means $\bundlei[k+1]^{(k)}[1]< 1-2/9-2/9=5/9$. This implies all remaining chores are less than $5/9$. Therefore, add the second largest chore, it is still less than $11/9$. We have  $\alloci[k+1]^*[2]$ must be the largest chore in the bundle $\bundlei[j]^{(k)}$.
\end{proof}
\end{observation}


\begin{observation}\label{obser-greater-4/9}
For the valuation of chore $\alloci[k+1]^*[2]$, we have  $\vai[\last]{\alloci[k+1]^*[2]}>4/9$.
\begin{proof}
As Inequality \ref{ineq-2-3} does not hold, we have
\begin{align*}
%\begin{split}
\vai[\last]{\left\{\alloci[k+1]^*[1],\alloci[k+1]^*[2], \bundlei[k+1]^{(k)}[3]\right\}}&> 11/9\\
&\ge2/9+\vai[\last]{\bundlei[k+1]^{(k)}}\\
&=2/9+\vai[\last]{\left\{\bundlei[k+1]^{(k)}[1],\bundlei[k+1]^{(k)}[2], \bundlei[k+1]^{(k)}[3]\right\}}
%\end{split}
\end{align*}
By the assumption that $\alloci[k+1]^*[1]=\bundlei[k+1]^{(k)}[1]$, we get $$\vai[\last]{\alloci[k+1]^*[2]}>2/9+\vai[\last]{\bundlei[k+1]^{(k)}[2]}>4/9.$$
\end{proof}

\end{observation}

Now we prove the statement by case analysis on the number of chores in the  bundle $\bundlei[j]^{(k)}$

For the case that bundle $\bundlei[j]^{(k)}$ only contains the chore $\alloci[k+1]^*[2]$ i.e. $|\bundlei[j]^{(k)}|=1$, it is easy to see bundle $\bundlei[j]^{(k+1)}$ is good after replacing the chore $\alloci[k+1]^*[2]$ with chores $\bundlei[k+1]^{(k)}[2]$ and $\bundlei[k+1]^{(k)}[3]$.

If bundle $\bundlei[j]^{(k)}$ contains two chores i.e. $|\bundlei[j]^{(k)}|=2$, we prove the valuation $\vai[\last]{\bundlei[j]^{(k+1)}}\le 1$. First we have following inequality
\begin{align*}
\vai[\last]{\left\{\bundlei[k+1]^{(k)}[2], \bundlei[k+1]^{(k)}[3]\right\}}&\le1-\vai[\last]{\bundlei[k+1]^{(k)}[1]}\\
&\le1-\vai[\last]{\alloci[k+1]^*[2]}.
\end{align*}
For the valuation of bundle $\bundlei[j]^{(k+1)}$, we have
\begin{align*}
\vai[\last]{\bundlei[j]^{(k+1)}}& = \vai[\last]{\left(\bundlei[j]^{(k)}\setminus \alloci[k+1]^*[2]\right)\bigcup\left(\left\{\bundlei[k+1]^{(k)}[2], \bundlei[k+1]^{(k)}[3]\right\}\right) }\\
&\le\vai[\last]{\alloci[k+1]^*[2]}+\vai[\last]{\left\{\bundlei[k+1]^{(k)}[2], \bundlei[k+1]^{(k)}[3]\right\}}\\
&\le \vai[\last]{\alloci[k+1]^*[2]}+1-\vai[\last]{\alloci[k+1]^*[2]}\\
&=1.
\end{align*}
The first inequality is due to the chore $\alloci[k+1]^*[2]$ is no less than the other chore in bundle $\bundlei[j]^{(k)}$. The second inequality is just follow the above inequality.
Thus, bundle $\bundlei[j]^{(k+1)}$ is  still good.

Now let us look at the case $|\bundlei[j]^{(k)}|=3$. Since bundle $\bundlei[j]^{(k)}$ is good, we have $\vai[\last]{\bundlei[j]^{(k)}}\le1$.  By Observation \ref{obser-greater-4/9}, we have  $\vai[\last]{\alloci[k+1]^*[2]}>4/9$.
Therefore, except the chore $\alloci[k+1]^*[2]$, the valuation of the remaining two chores in bundle $\bundlei[j]^{(k)}$ is $$\vai[\last]{\bundlei[j]^{(k)}\setminus \alloci[k+1]^*[2]}\le 1-\vai[\last]{\alloci[k+1]^*[2]}<5/9.$$
%,  the sum of remaining two in $\bundlei[j]^{(k)}$ is less than 5/9.
As the valuation $\vai[\last]{\bundlei[k+1]^{(k)}[1]}\ge\vai[\last]{\alloci[k+1]^*[2]}>4/9$ and bundle $\bundlei[k+1]^{(k)}$ is good,   we have $$\vai[\last]{\left\{\bundlei[k+1]^{(k)}[2], \bundlei[k+1]^{(k)}[3]\right\}}\le1-\vai[\last]{\bundlei[k+1]^{(k)}[1]}<5/9.$$
For the bundle $\bundlei[j]^{(k+1)}$, the largest chore is either in the set  $\bundlei[j]^{(k)}\setminus \alloci[k+1]^*[2]$ or in the set $\bundlei[k+1]^{(k)}[2]\cup \bundlei[k+1]^{(k)}[3].$ Therefore, the valuation $$U\left(\bundlei[j]^{(k+1)}\right)\le\max\left\{\vai[\last]{\bundlei[j]^{(k)}\setminus \alloci[k+1]^*[2]},\vai[\last]{\left\{\bundlei[k+1]^{(k)}[2],\bundlei[k+1]^{(k)}[3]\right\}}\right\}<5/9.$$
It is easy to see, in this case, the cardinality $|\bundlei[j]^{(k+1)}|=4$. Thus, bundle $\bundlei[j]^{(k+1)}$ is good.
%Let $\bundlei[j]^{(k)*}$ be the bundle after swapping. Combining these, we have $U(\bundlei[j]^{(k)*})<5/9$, which means it is still good.

It is impossible that $|\bundlei[j]^{(k)}|=4$. Since bundle $\bundlei[j]^{(k)}$ is good, if $|\bundlei[j]^{(k)}|=4$, then we have $U\left(\bundlei[j]^{(k)}\right)<5/9.$ As bundle $\bundlei[j]^{(k)}\subseteq \larg{\last,2/9}$, it implies that the valuation of the largest chore $$\vai[\last]{\alloci[k+1]^*[2]}=\vai[\last]{\bundlei[j]^{(k)}[1]}\le U\left(\bundlei[j]^{(k)}\right)-2/9<1/3.$$  This contradicts to  Observation \ref{obser-greater-4/9} i.e. $\vai[\last]{\alloci[k+1]^*[2]}>4/9$. So it is impossible.

\end{proof}


It is easy to see that, for a good bundle, if we replace one chore with a smaller chore, it is still good. The only case, which may increase the number of chores or increase the value of chores, is concluded in claim \ref{claim-two-one}. Thus we can keep this process to $\bundles^{(n)}$.
\end{proof}




















\begin{proof}
Let $\allocs$ be the allocation returned by Algorithm \ref{alg-poly}. And let bundle $\alloci^*=\alloci\cap \larg{\last, s_{\last}/4}$ consist of large chores from bundle $\alloci$. Let $D_k= \larg{\last, s_{\last}/4}\setminus\left( \cup_{i< k}\alloci^*\right)$ be the set of  large chores that have not been allocated in first $k-1$ rounds. Let $\bundlei$ be the bundle which is the $i$-th bundle generated by the threshold testing algorithm on input $s_{\last}$. Let chore set  $P_k=\cup_{i\ge k}\bundlei$. We will prove the following property which directly imply that no chore $c\in \larg{\last,s_{\last}/4}$ left.

\bigskip
{\bf Property $T$:} For each $k$, there exists an injective function $f_k:D_k\rightarrow P_k$ such that $\vai[\last]{c}\le \vai[\last]{f_k(c)}$ for all  $c\in D_k$.
\bigskip

When $k=n$, the property $T$ implies the total value of large chores in the last round is no grater than $\vai[\last]{\bundlei[n]}$, which is less than 5/4. Therefore, all large chores will be allocated. 

We will prove the property $T$ by induction. When $k=1$, the identical mapping will work. Now we prove that if the statement holds for $k$, then we can construct a suitable mapping for $k+1$. For this, it is sufficient to prove we can drop $\alloci[k]^*$ and $\bundlei[k]$ from the domain at the same time.

Here we introduce the swap operation for the function first. Given a function $f:D\rightarrow P$, chore $d\in D$ and chore $p\in P$, the operation $f^*=\text{Swap}(f,d,p)$ is defined as
\begin{equation*}
 f^*(c) =
  \begin{cases}
   f(c) & \text{for } c\neq d \text{ or } f^{-1}(p)  \\
   p       & \text{if } c=d  \\
   f(d)  & \text{if } c=f^{-1}(p)
  \end{cases}
\end{equation*}
 %$f^*(c)=f(c)$ for $\{c\in D_k\mid c\neq d \text{ and } c\neq f^{-1}(p)\}$
 Intuitively, this operation just swaps the mapping images of $d$ and $f^{-1}(p)$. If $f^{-1}(p)=\emptyset$, then this operation just change the image of $d$ to $p$.

Let $q=\min\{|\alloci[k]^*|,|\bundlei[k]|\}$. Let $g_0=f_k$ be a mapping function. For $1\le t\le q$, we iteratively construct mapping $$g_t=\text{Swap}(g_{t-1},\alloci[k]^*[t],\bundlei[k][t]).$$  Then let $f_{k+1}(c)=g_q(c)$ for all $c\in D_{k+1}$. Now we show that such construction will satisfy the condition in the statement.

\begin{claim}\label{claim-all-large}
For each $k$ and $1\le j<|\bundlei[k]|$, we have $\bundlei[k][j]=P_k[j]$ i.e. except the smallest chore in bundle $\bundlei[k]$, other chores are the largest chores in the remaining. 
\end{claim}
\begin{proof}
In threshold testing, the bundle is constructed in two stages. We first consider the bundle $\bundlei[k]$  is constructed before the for-loop in line \ref{inalg-after-big}. We have $|\bundlei[k]|\le 2$ and $\bundlei[k][1]=P_k[1]$.  So all bundles, which are constructed in this stage, satisfy the statement.

Now consider the bundle $\bundlei[k]$  is constructed in the for-loop of line \ref{inalg-after-big}. The bundle $\bundlei[k]$ is constructed by adding chores one by one from largest to smallest. Suppose that $j^*<|\bundlei[k]|$ is the first index that $\bundlei[k][j^*]\neq P_k[j^*]$. Notice that in this stage, for any chore $c$ we have $\frac{s_{\last}}{4}<\vai[\last]{c}\le \frac{s_{\last}}{2}.$  This implies  
\begin{align*}
\vai[\last]{\left\{\bundlei[k][j^*],\bundlei[k][j^*+1]\right\}}&>\frac{s_{\last}}{4}+\frac{s_{\last}}{4}\\
%&=\frac{s_{\last}}{2}\\
&>\vai[\last]{P_k[j^*]}.
\end{align*} 
So there is enough space for chore $P_k[j^*]$ to put into bundle $\bundlei[k]$. According to the threshold testing algorithm, chore $P_k[j^*]$ should be put into bundle $\bundlei[k]$
 %should be put into $\bundlei[k]$ and then $\bundlei[k][j^*]=P_k[j^*]$. 
 This is a contradiction. Therefore, we have $\bundlei[k][j]=P_k[j]$ for $1\le j<|\bundlei[k]|$.

 %Once we add one chore $c$ such that $\vai[\last]{c}<\vai[\last]{p}$ for some $p\in P_k\setminus\bundlei[k]$, then we cannot add another smaller chore $c'$. Otherwise, we have $\vai[\last]{c\cup c'}>\vai[\last]{p}$, which means the chore $p$ should be added into $\bundlei[k]$. Because there is enough space when algorithm considers to add $p$ into $\bundlei[k]$.
\end{proof}

 \begin{claim}\label{claim-not-bad}
 Recall that $q=\min\{|\alloci[k]^*|,|\bundlei[k]|\}$. For mapping $g_q$, we have $\vai[\last]{c}\le \vai[\last]{g_q(c)}$ for any chore $c\in D_k\setminus \alloci[k]^*$.
 \end{claim}
 \begin{proof}
We first prove that, for $1\le t<q$, the statement $$\forall c\in D_k, \vai[\last]{c}\le \vai[\last]{g_t(c)}$$ is true. We prove it by induction. Suppose the statement $\forall c\in D_k, \vai[\last]{c}\le \vai[\last]{g_{t-1}(c)}$ is true.
In each swap operation, we map chore $\alloci[k]^*[t]$ to chore $\bundlei[k][t]$ and chore $g_{t-1}^{-1}(\bundlei[k][t])$ to chore $g_{t-1}(\alloci[k]^*[t])$. 
%What happened to chore $\alloci[k]^*[t]$ does not influence the statement. It is sufficient to argue that $$\vai[\last]{g_{t-1}^{-1}(\bundlei[k][t])}\le \vai[\last]{g_{t-1}(\alloci[k]^*[t])}.$$
%If the 
%Recall   the construction of bundle $\alloci[k]$. When we allocate the  chore $\alloci[k]^*[t]$ to the bundle $\alloci[k]$, if there is enough space to allocate the chore $g_{t-1}^{-1}(\bundlei[k][t])$ but we 
 Since bundle $\alloci[k]^*\subseteq P_k$, by Claim \ref{claim-all-large}, we have $$\vai[\last]{\alloci[k]^*[t]}\le\vai[\last]{P_k[t]}= \vai[\last]{\bundlei[k][t]}.$$ 
 
 
Now we will prove $\vai[\last]{g_{t-1}^{-1}(\bundlei[k][t])}\le \vai[\last]{g_{t-1}(\alloci[k]^*[t])}$. If  chore $g_{t-1}^{-1}(\bundlei[k][t])=\alloci[k]^*[t]$, then this is the above case.  If chore $g_{t-1}^{-1}(\bundlei[k][t])\neq\alloci[k]^*[t])$, recall  the construction of bundle $\alloci[k]$. When we allocate the  chore $\alloci[k]^*[t]$ to the bundle $\alloci[k]$, if there is enough space to allocate the chore $g_{t-1}^{-1}(\bundlei[k][t])$ but algorithm does not do that, it means $$\vai[\last]{g_{t-1}^{-1}(\bundlei[k][t])}\le\vai[\last]{\alloci[k]}\le \vai[\last]{g_{t-1}(\alloci[k]^*[t])}.$$ So we only need to prove that there is enough space for chore $g_{t-1}^{-1}(\bundlei[k][t])$.
Notice that 
\begin{align*}
\vai[\last]{\left(\cup_{h<t}\alloci[k]^*[h]\right)\cup g_{t-1}^{-1}(\bundlei[k][t])}&\le\vai[\last]{\left(\cup_{h<t} g_{t-1}(\alloci[k]^*[h])\right)\cup \bundlei[k][t]}\\
&\le\vai[\last]{\cup_{h\le t}P_k[h]}\\
&=\vai[\last]{\cup_{h\le t}\bundlei[k][h]}\\
&<5/4
\end{align*}
The equality in the third line is by Claim \ref{claim-all-large}.   This means that there is enough space for chore $\bundlei[k][t]$ to be allocated when algorithm allocates the  chore $\alloci[k]^*[t]$ to the bundle $\alloci[k]$. As $\vai[\last]{g_{t-1}^{-1}(\bundlei[k][t])}\le\vai[\last]{\bundlei[k][t]}$, there is enough space for chore $g_{t-1}^{-1}(\bundlei[k][t])$. Therefore, we have $\vai[\last]{g_{t-1}^{-1}(\bundlei[k][t])}\le \vai[\last]{g_{t-1}(\alloci[k]^*[t])}$.


For $g_q$, what happened to chore $\alloci[k]^*[q]$ is not our concern.  We only need to argue that $$\vai[\last]{g_{t-1}^{-1}(\bundlei[k][q])}\le \vai[\last]{g_{t-1}(\alloci[k]^*[q])}.$$ The remaining proof is similar to the above case. Recall  the construction of bundle $\alloci[k]$, when we allocate the  chore $\alloci[k]^*[q]$ to the bundle $\alloci[k]$,  there is enough space to allocate the chore $g_{t-1}^{-1}(\bundlei[k][q])$. Because
\begin{align*}
\vai[\last]{\left(\cup_{h<q}\alloci[k]^*[h]\right)\cup g_{t-1}^{-1}(\bundlei[k][q])}&\le\vai[\last]{\left(\cup_{h<q} f_k(\alloci[k]^*[h])\right)\cup\bundlei[k][q]}\\
&\le\vai[\last]{\left(\cup_{h<q}P_k[h]\right)\cup\bundlei[k][q]}\\
&\le\vai[\last]{\bundlei[k]}\\
&<5/4
\end{align*}


%From the construction of bundle $\alloci[k]$, we could conclude that chore $\alloci[k]^*[h]=D_k[h]$ for $h<q$. This implies $\alloci[k]^*[t]$ is the $t$'th largest chore in set $D_k$.
%By the construction of mapping function, it is easy to see that $g_{t-1}(\alloci[k]^*[h])=\bundlei[k][h]$ for $h\le t-1$. Therefore, chore $g_{t-1}^{-1}(\bundlei[k][t])$ would not be chore $\alloci[k]^*[h]$ for any $h\le t-1$, which means  chore $g_{t-1}^{-1}(\bundlei[k][t])$ is not one of largest $t-1$ chores among set $D_k$.
%We have $$\vai[\last]{g_{t-1}^{-1}(\bundlei[k][t])}\le\vai[\last]{\alloci[k]^*[t]}\le \vai[\last]{g_{t-1}(\alloci[k]^*[t])}.$$



  %From the construction of bundle $\alloci[k]$, we have $\vai[\last]{g_{t-1}^{-1}(\bundlei[k][t])}\le\vai[\last]{\alloci[k]^*[t]}\le \vai[\last]{g_{t-1}(\alloci[k]^*[t])}$.
%By Claim \ref{claim-all-large}, we have $\vai[\last]{\alloci[k]^*[t]}\le \vai[\last]{\bundlei[k][t]}$ for $t<\min$
 \end{proof}

By Claim \ref{claim-not-bad}, we have $\vai[\last]{c}\le\vai[\last]{g_q(c)} $ for all $c\in D_{k+1}$. The remaining to prove is that $g_q(D_{k+1})\subseteq P_{k+1}$. So we have the following lemma.

\begin{claim}\label{claim-no-more}
If the cardinality $|\alloci[k]^*|<|\bundlei[k]|$, then for $|\alloci[k]^*|<j\le|\bundlei[k]|$, we have $g_q^{-1}(\bundlei[k][j])=\emptyset$.
\end{claim}
\begin{proof}
For the valuation of bundle $\alloci[k]^*$, we have
\begin{align*}
\vai[\last]{\alloci[k]^*}&\le \vai[\last]{\bigcup_{1\le t\le|\alloci[k]|}\bundlei[k][t]}\\
&\le \frac{11}{9}-\vai[\last]{\bundlei[k][j]}\\
&\le \frac{5}{4}-\vai[\last]{\bundlei[k][j]},
\end{align*}
where $|\alloci[k]^*|<j\le|\bundlei[k]|$. The first inequality is implied by Claim \ref{claim-all-large} and Claim \ref{claim-not-bad}. This means that if there is a chore mapping to  chore $\bundlei[k][j]$, then this chore can be added into $\alloci[k]^*$.
\end{proof}

By Claim \ref{claim-no-more} and the construction of mapping function $g_q$, we have $g_q(D_{k+1})\subseteq P_{k+1}$. And by Claim \ref{claim-not-bad}, we have $\vai[\last]{c}\le \vai[\last]{g_q(c)}$ for $c\in D_{k+1}$. Combining these, our construction of $f_{k+1}$ is valid.


\end{proof}

==> limit.tex <==
In this section, we discuss the limitation of our framework.  %The previous best known result is 4/3 approximation~\cite{barman2017approximation}. We show that their technique cannot give a ratio better than 4/3. 
For our algorithm framework, we show a 20/17 lower bound. In section \ref{sec-poly}, we design a threshold testing algorithm. At the first look, people may wonder is there a more natural approach to do threshold testing.  Here we give an example to show that, for Algorithm \ref{alg-approx}, suppose  a set of $\{\alpha_i\}$ make the algorithm allocate all chores,   if we increase the value of $\alpha_i$, it is possible that chores cannot be all allocated. 


% The lower bound   Please refer the literature of LPT algorithm for load balancing 
%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
Define base allocation and show that such base allocation cannot break 4/3 barrier. 
\begin{exmp}
Set $\epsilon=\frac{1}{6(n-1)}$.

Base allocation  $\{2/3-2\epsilon, 1/3\}$, $\{2/3-3\epsilon,1/3+\epsilon\}$,$\dots$ $\{1/2,1/2-2\epsilon\}$ and $\{1/2,1/2-\epsilon\}$, and $1/3-\epsilon$ remaining

Optimal allocation $\{1/3-\epsilon,1/3,1/3+\epsilon\}$, $\{2/3-2\epsilon,1/3+2\epsilon\}$, $\{2/3-3\epsilon,1/3+3\epsilon\}$, $\dots$, $\{1/2+\epsilon,1/2-\epsilon\}$ and $\{1/2,1/2\}$
\end{exmp}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%


For the lower bound of our algorithmic framework, we give the following example. 
\begin{exmp}
In this example, we consider an instance of 14 chores and 4 agents with an identical valuation (not just ordinal, but cardinal is also same). The valuation of each chore is demonstrated by the optimal allocation. 
%Their valuations are: one chore is valued as $\frac{9}{17}$, one chore is valued as $\frac{7}{17}$, one chore is valued as $\frac{6}{17}$ and two chores are valued as $\frac{5}{17}$ and 9 chores are valued as $\frac{4}{17}$.

An optimal allocation of this instance is that $$\alloci[1]=\{\frac{9}{17},\frac{4}{17},\frac{4}{17}\}, \alloci[2]=\{\frac{7}{17},\frac{6}{17},\frac{4}{17}\}\text{ and }\alloci[3]=\alloci[4]= \{\frac{5}{17},\frac{4}{17},\frac{4}{17},\frac{4}{17}\},$$ where the numbers are valuations of each chore. Obviously, the \mmax~of each agent is 1. However, if we input $\alpha_i<20/17$ to Algorithm \ref{alg-approx}, then not all chores could be allocated. 
\end{exmp}

\begin{theorem}\label{thm-lower-bound}
Algorithm \ref{alg-approx} cannot show the existence of \amMS{\alpha} for $\alpha<20/17$.
\end{theorem}



Intuitively, people may think if Algorithm \ref{alg-approx} can allocate all chores on input of threshold values $\{\alpha_i\}$, then  Algorithm \ref{alg-approx} should allocate all chores with larger threshold values. Here we give a counter example for this monotonicity. 
\begin{exmp}\label{exm-no-monoton}
In this example, we consider an instance of 17 chores and 4 agents with an identical valuation. The valuation of each chore is demonstrated by the optimal allocation. 

An optimal allocation of this instance is that $$\alloci[1]=\{5.1,1.2,1.2\}, \alloci[2]=\alloci[3]=\{2.75,2.75,1,1\}\text{ and }\alloci[4]=\{2.5,1,1,1,1,1\},$$ where the numbers are valuations of each chore.  The \mmax~of each agent is 7.5. You can verity that if we input threshold value $7.5$ to Algorithm \ref{alg-approx}, all chores will be allocated. And the allocation is exactly the optimal allocation we give here. 

However, if we input threshold value  7.6 to Algorithm \ref{alg-approx}, we have $$\alloci[1]=\{5.1,2.5\}, \alloci[2]=\alloci[3]=\{2.75,2.75,1.2\}\text{ and }\alloci[4]=\{1,1,1,1,1,1,1,1,1\}.$$ There are 2 chores remained. 
\end{exmp}



==> store.tex <==
\begin{proof}
Suppose $\allocs$ is the allocation returned by the algorithm and $\bundles$ is a \mmax~allocation for the last agent $\last$. Now we try to swap chores in \mmax~allocation $\bundles$ so that it will become the allocation $\allocs$. The proof is to analysis what happened in this swapping process. 

As we have shown in Lemma \ref{lem-no-less-2/9}, we do not need to consider small chores. So let us define the bundle $\alloci^*$ as $\alloci\cap \larg{\last,2/9}$ and the bundle  $\bundlei^*$ as $\bundlei\cap \larg{\last,2/9}$.
For the simplicity of the proof, we assume that all bundles are ordered by the largest chore in each bundle i.e. $\alloci[i]^*[1]\ge \alloci[j]^*[1]$  for all $i<j$. Notice that for the allocation $\allocs$, this order is exactly the order from the  for loop in line \ref{inalg-loop} of Algorithm \ref{alg-approx}.

%Without loss of generality, we can assume the bundles in $\allocs$ are sorted as following: For any $j$, the bundle $\alloci[j]\in\allocs$ is generated by the algorithm when $k=j$ of the for loop in line \ref{inalg-loop}. %And define the bundle $\alloci^*$ as $\alloci\cap \larg{\last,2/9}$ and the bundle  $\bundlei^*$ as $\bundlei\cap \larg{\last,2/9}$.
%\xin{Write more explanation before the definition}

%To prove this lemma, we will start with bundles $\bundlei^*$ and then generate bundles $\bundlei$ by swapping chores between bundles.
We start with bundle collection $\bundles^{(0)}=\left(\bundlei[1]^*,\dots,\bundlei[n]^*\right)$  for our swapping process. Bundle collection $\bundles^{(0)}$ is a \mmax~allocation of large chores. There are $n$ rounds  of the swapping process in total. In each round $t$, we generate a bundle collection $\bundles^{(t)}$ by swapping some chores in bundle collection $\bundles^{(t-1)}$, so that  bundle $\bundlei[t]^{(t)}=\alloci[t]^*$. Notice that we do not need to touch bundles with index strictly less than $t$ to fix bundle $\bundlei[t]^{(t)}$.  So we have $\bundlei^{(t)}=\alloci^*$ for all $i\le t$.
%At the beginning of the swapping process, Let bundle collection $\bundles^{(0)}=\left(\bundlei[1]^*,\dots,\bundlei[n]^*\right)$ include all $\bundlei^*$. Notice that $\larg{\last,2/9}=\cup_i\bundlei^*$.  Our target is to generate bundle collection $\bundles^{(t)}$ from $\bundles^{(t-1)}$ by  swapping chores between bundles, so that $\bundlei^{(t)}=\alloci^*$ for all $i\le t$. If this process can successfully proceed, then $\bundles^{(n)}=\left(\alloci[1]^*,\dots,\alloci[n]^*\right)$ which means all chores $c\in \larg{\last,2/9}$ are allocated.

If this swapping process could success to the round $n$, then all large chores are allocated in allocation $\allocs$, which implies the lemma.   To show this, we carefully specifiy the swapping process so that bundle collection $\bundles^{(t)}$ satisfies a good property. %We will prove this by induction.
%To prove this, we will show that, for $i>t$, bundles $\bundlei^{(t)}$  satisfies a good property by induction.

%The definitions of ``good" properties are in the below. Here we give a high level intuition for why ``good" bundle is good. There are two conditions. A bundle will be considered as ``good"  if it satisfies any of two conditions. 
%\begin{itemize}
%\item The fist condition states that the value of the bundle is upper bounded. It makes sure the number of large chores would not be greater than 4. This will make the case analysis possible.  Another good thing is that all initial bundles satisfy this condition. So we have the basis for the induction. 
%\item The second condition is about the sum of the largest chore and the least chore in a bundle. This condition could help us to analyze the number of chores after swapping. And we restrict the number of chores must be 4 before swapping. These two conditions could ensure that the swapping process would always swap a less valued chore to another bundle. 
%\end{itemize}
 % 1. contains all bundles at the beginning. 2. at most 4 large chores, wouldn't cause too much trouble. The second condition 1. though the swapping process, there is only such case that bundle could larger than 1. 2. we focus on the sum of largest and smallest chores, because in this way we can make sure 3 largest + 1 smallest will not exceed 11/9.

To introduce the good property, we need some definitions. Let $$U(\bundle)=\min_{c\in \bundle} \vai[\last]{c}+\max_{c\in\bundle}\vai[\last]{c}$$ denote the sum of largest and smallest chore in the bundle.

\bigskip
{\bf Good bundle:} A bundle $\bundle$ is \emph{good} if 1) $\vai[\last]{\bundle}\le1$ or, 2) $U(\bundle)<5/9\text{ and }|\bundle|=4.$ \xin{Write down the intuition for the definition}
\bigskip

These two conditions for a good bundle are corresponding to two types swapping which are mentioned in the high level idea description. 

Here we slightly abuse the concept ``good" for bundle collection.

\bigskip
{\bf Good bundle collection:}  A bundle collection $\bundles^{(t)}$ is \emph{good} if $\bundlei^{(t)}=\alloci^*$ for all $i\le t$, and for $i>t$ each bundle $\bundlei^{(t)}$ is good.
\bigskip

Clearly, the bundle collection $\bundles^{(0)}$ is good. %Suppose when $t=k$, the bundle collection $\bundles^{(t)}$ is good. We will prove, when $t=k+1$,  by swapping some chores from $\bundles^{(k)}$, we can construct a good bundle collection $\bundles^{(k+1)}$.
This would be the basis for our induction. Now we need to describe the swapping process.
To precisely do it, we introduce two operations $SWAP$ and $MOVE$, where the operation $SWAP$ would swap two chores and the operation $MOVE$ would move a set of chores  from their original bundles to a target  bundle.
%Here we introduce two operations that are very helpful in construction $\bundles^{(k+1)}$ from $\bundles^{(k)}$.

Given a bundle collection $\bundles$ and two chores $c_1$ and $c_2$, the $SWAP$ operation will generate a new bundle collection $\bundles^{\#}=SWAP(\bundles,c_1,c_2)$ such that: If $c_1=c_2$ or, $c_1$ and $c_2$ are in the same bundle, then $\bundles^{\#}=\bundles$; Otherwise
\begin{equation*}
 \bundlei^{\#}=
  \begin{cases}
   \bundlei & \text{if } c_1,c_2\notin \bundlei  \\
   (\bundlei\setminus c_1)\cup c_2       & \text{if } c_1\in\bundlei \\
   (\bundlei\setminus c_2)\cup c_1  & \text{if } c_2\in\bundlei
  \end{cases}
\end{equation*}
%This operation swaps chore $c_1$ and $c_2$.

Given a bundle collection $\bundles$, an  index $j\in\agents$ and a subset of chores $T\subseteq\items$, the $MOVE$ operation will generate a new bundle collection $\bundles^{\#}=MOVE(\bundles,j,T)$ such that
 \begin{equation*}
  \bundlei^{\#}=
   \begin{cases}
    \bundlei\setminus T & \text{if } i\neq j \\
    \bundlei\cup T      & \text{if } i=j \\
   \end{cases}
 \end{equation*}
 Notice that chores set $T$ could contain chores from different bundles. 
%This operation moves chores set $T$ from their original bundles to the bundle indexed by $j$.

%Let bundle $\bundlei^{(k+1)}=\alloci^*$ for $i\le k+1$. We will show how to construct remaining bundles i.e. $\bundlei^{(k+1)}$ where $i>k+1$.
%\xin{Give a reminder, but simplify this paragraph} 
%contains the largest chore among chores $\cup_{i\ge k+1} \bundlei^{(k)}$ (we can rename the bundle containing the largest chore to $\bundlei[k+1]^{(k)}$). %Let $\bundle(j)$ denote the $j$-th largest chore in the $\bundle$ from agent $\last$'s view.
%It is easy to see that $\bundlei[k+1]^{(k)}[1]=\alloci[k+1]^*[1]$, as Algorithm \ref{alg-approx} always allocates the largest chore of remaining to a new bundle. So, we only need  to take care of remaining chores from both bundles.

%\xin{Define two types swapping here, make argument easy?}
Now we describe and prove the correctness of  the swapping process by induction. Suppose that bundle collection $\bundles^{(k)}$ is good. We will swap and move some chores between bundle $\bundlei[k+1]^{(k)}$ and bundles with index greater than $k+1$, so that the bundle $\bundlei[k+1]^{(k)}$ would become bundle $\alloci[k+1]^*$.  Without loss of generality, we can assume that the largest chore in  bundle $\bundlei[k+1]^{(k)}$ and  bundle $\alloci[k+1]^*$ are the same, i.e. chore $\bundlei[k+1]^{(k)}[1]=\alloci[k+1]^*[1]$. This is the largest chore among  the set $\bigcup_{i\ge k+1} \bundlei^{(k)}$ by our assumption of the order of allocation $\allocs$ (The assumption made at the beginning of the whole proof).   
 By the condition of good bundle collection and the value of large chores, we know that  bundle $\bundlei[k+1]^{(k)}$ contains at most $4$ chores.
%For each chore $c\in \cup_i\bundlei^*$, we  know the valuation $\val[\last](c)>\frac{2}{9}$ and the valuation $\vai[\last]{\bundlei^*}\leq 1$. This implies that each $\bundlei^*$ contains at most $4$ chores. %During the swapping process, we keep the property that for $i>t$ each bundle $\bundlei^{(t)}$ contains at most $4$ chores. 
  Based on the size of bundle $\bundlei[k+1]^{(k)}$, we have the following case analysis.

%Now we show a delicate to swap some chores to make $\bundlei[k+1]^{(k)}$ to become $\bundlei[k+1]$. We show it in case analysis:
\begin{itemize}
\item $|\bundlei[k+1]^{(k)}|=1,2,\mbox{ and } 4$:  Let $d=|\bundlei[k+1]^{(k)}|$ be the cardinality of the bundle. 
By Claim \ref{claim-4chores}, we have that $|\alloci[k+1]^*|\ge |\bundlei[k+1]^{(k)}|$ and $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$ for $j\le d$.  For the first $d$ chores, we swap them one by one. Since we have $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$, after these swaps, some chores become smaller for  bundles with index larger than $k+1$. A good bundle will still be a good bundle.  If the cardinality $|\alloci[k+1]^*|>d$, then we just move remaining chores  to bundle $\bundlei[k+1]^{(k)}$. After we remove some chores, a good bundle will still be a good bundle. Therefore, when we get the  bundle collection $\bundles^{(k+1)}$, it is a good bundle collection. 


Mathematically, let bundle collection $G^{(1)}=\bundles^{(k)}$. The swapping of first $d$ chores  could be represented as the following form  $G^{(j)}=SWAP\left(G^{(j-1)},\bundlei[k+1]^{(k)}[j],\alloci[k+1]^*[j]\right)$ for $2\le  j\le d$. The bundle collection $G^{(d)}$ is the resulting bundle after these swaps.  And the moving operation to generate bundle collection $\bundles^{(k+1)}$ is equivalent to 
$$\bundles^{(k+1)}=MOVE\left(G^{(d)},k+1,\alloci[k+1]^*\right).$$ 

%For chores in bundle $\alloci[k+1]^*$, we move them  from their current bundles  to  bundle $\bundlei[k+1]^{(k)}$.
%Mathematical equivalently, for the bundle collection $\bundles^{(k+1)}$, we have  %$$\bundlei^{(k+1)}=\bundlei^{(k)}\setminus \alloci[k+1]^*\text{ for } i>k+1.$$
%Formally, we have
%$$\bundles^{(k+1)}=MOVE\left(\bundles^{(k)},k+1,\alloci[k+1]^*\right).$$

%The bundle with index larger than $k+1$ either does not change or remove some chores. Thus a good bundle is still good. This gives that bundle collection $\bundles^{(k+1)}$ is good.

%\xin{Write a new statement: $|\alloci[k+1]^*|\ge |\bundlei[k+1]^{(k)}|$ and $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$ }

%\item $|\bundlei[k+1]^{(k)}|=2$: First we have the cardinality  $|\alloci[k+1]^*|\ge 2$. Because Algorithm \ref{alg-approx}  can at least allocate chore $\bundlei[k+1]^{(k)}[2]$ to bundle $\alloci[k+1]^*$ as the second chore. This observation also implies valuation $\vai[\last]{\bundlei[k+1]^{(k)}[2]}\le\vai[\last]{\alloci[k+1]^*[2]}$. If chore $\bundlei[k+1]^{(k)}[2]\neq\alloci[k+1]^*[2]$, then we swap these two chores. And if there are more chores in bundle $\alloci[k+1]^*$ i.e. $|\alloci[k+1]^*|>2$, then we just move remaining chores from their current bundles  to $\bundlei[k+1]^{(k)}$. Mathematical equivalently,% for $i>k+1$, 
%we have
\begin{comment}
\begin{equation*}
 \bundlei^{(k+1)} =
  \begin{cases}
   \bundlei^{(k)}\setminus \alloci[k+1]^* & \text{if }  \alloci[k+1]^*[2]\notin  \bundlei^{(k)}\\
   \left(\bundlei^{(k)}\cup\bundlei[k+1]^{(k)}[2]\right)\setminus \alloci[k+1]^*      & \text{if } \alloci[k+1]^*[2]\in  \bundlei^{(k)} \\
  \end{cases}
\end{equation*}
\end{comment}
%$$\bundles^{(k+1)}=MOVE\left(SWAP\left(\bundles^{(k)},\bundlei[k+1]^{(k)}[2],\alloci[k+1]^*[2]\right),k+1,\alloci[k+1]^*\right).$$

%The bundle with index larger than $k+1$ either does not change or remove some chores. Thus a good bundle is still good. This gives that bundle collection $\bundles^{(k+1)}$ is good. \xin{Is it better to make it a claim?}

\item $|\bundlei[k+1]^{(k)}|=3$: By a similar argument as the above case, we have $|\alloci[k+1]^*|\ge 2$. Let $$G=SWAP\left(\bundles^{(k)},\bundlei[k+1]^{(k)}[2],\alloci[k+1]^*[2]\right)$$ be the bundle collection that  swap chore $\bundlei[k+1]^{(k)}[2]$ and chore $\alloci[k+1]^*[2]$.  Now we consider the following inequality:
\begin{equation}\label{ineq-2-3}
\vai[\last]{\left\{\alloci[k+1]^*[1],\alloci[k+1]^*[2], \bundlei[k+1]^{(k)}[3]\right\}}\le 11/9
\end{equation}

If the Inequality \ref{ineq-2-3} holds,  then we have $|\alloci[k+1]^*|\ge 3$ and $\vai[\last]{\bundlei[k+1]^{(k)}[3]}\le\vai[\last]{\alloci[k+1]^*[3]}$. For this case, we will swap chore $\bundlei[k+1]^{(k)}[3]$ and chore $\alloci[k+1]^*[3]$ and move remaining chores in bundle $\alloci[k+1]^*$ to bundle $\bundlei[k+1]^{(k)}$, i.e.
$$\bundles^{(k+1)}=MOVE\left(SWAP\left(G,\bundlei[k+1]^{(k)}[3],\alloci[k+1]^*[3]\right),k+1,\alloci[k+1]^*\right).$$

In this subcase, the bundle with index larger than $k+1$ either does not change or remove some chores. Thus a good bundle is still good. This gives that bundle collection $\bundles^{(k+1)}$ is good.

If the Inequality \ref{ineq-2-3} does not hold, then we move $\bundlei[k+1]^{(k)}[3]$ to the bundle where $\alloci[k+1]^*[2]$ comes from and then move  other chores in $\alloci[k+1]^*$  to $\bundlei[k+1]^{(k)}$. Let $j$ be an index of a bundle such that $\alloci[k+1]^*[2]\in\bundlei[j]^{(k)}$. Then, formally this process is
$$\bundles^{(k+1)}=MOVE\left(MOVE\left(G,j,\bundlei[k+1]^{(k)}[3]\right),k+1,\alloci[k+1]^*\right).$$

This is the most complicated case since $\bundlei[j]^{(k+1)}$ contains more item than $\bundlei[j]^{(k)}$. 
We prove that  bundle $\bundlei[j]^{(k+1)}$ is good in Claim \ref{claim-two-one}. And for other bundles with index larger than $k+1$, it either does not change or remove some chores.  Therefore, bundle collection $\bundles^{(k+1)}$ is good.

%\item $|\bundlei[k+1]^{(k)}|=4$:
%Using the property of good bundle,  we prove that $|\alloci[k+1]^*|\ge 4$ and $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$ for $j\le4$ in Claim \ref{claim-4chores}. For the first 4 chores, we swap them one by one. If the cardinality $|\alloci[k+1]^*|>4$, then we just move remaining chores from their original bundles  to $\bundlei[k+1]^{(k)}$.

%Formally the process is described as following.Let bundle collection $G^{(0)}=\bundles^{(k)}$ and bundle collection  $G^{(j)}=SWAP\left(G^{(j-1)},\bundlei[k+1]^{(k)}[j],\alloci[k+1]^*[j]\right)$ for $1\le  j\le 4$. We have
%$$\bundles^{(k+1)}=MOVE\left(G^{(4)},k+1,\alloci[k+1]^*\right).$$ 

%The bundle with index larger than $k+1$ either does not change or remove some chores. Thus a good bundle is still good. This gives that bundle collection $\bundles^{(k+1)}$ is good.
\end{itemize}

\begin{claim}\label{claim-4chores}
For the cases $|\bundlei[k+1]^{(k)}|=1,2,\mbox{ and }4$, we have the inequalities $|\alloci[k+1]^*|\ge |\bundlei[k+1]^{(k)}|$ and $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$ for $j\le|\bundlei[k+1]^{(k)}|$.
\end{claim}
\begin{proof}
For the case $|\bundlei[k+1]^{(k)}|=1$, it is trivial. For the case  $|\bundlei[k+1]^{(k)}|=2$, we notice that Algorithm \ref{alg-approx}  can at least allocate chore $\bundlei[k+1]^{(k)}[2]$ to bundle $\alloci[k+1]^*$ as the second chore. This would imply the cardinality  $|\alloci[k+1]^*|\ge 2$ and the valuation $\vai[\last]{\bundlei[k+1]^{(k)}[2]}\le\vai[\last]{\alloci[k+1]^*[2]}$.


For the case $|\bundlei[k+1]^{(k)}|=4$, first we prove that the inequality  $U(\bundlei[k+1]^{(k)})<5/9$ is true. Since bundle $\bundlei[k+1]^{(k)}$ is good, we have the condition $U(\bundlei[k+1]^{(k)})<5/9$ or  $\vai[\last]{\bundlei[k+1]^{(k)}}\le1$.
If the valuation $\vai[\last]{\bundlei[k+1]^{(k)}}\le1$, then as  any chores in the bundle is greater than 2/9,  we have $$U(\bundlei[k+1]^{(k)})=1-\text{value of the other two chores}<1-2\cdot 2/9=5/9.$$

Now we prove the inequality $$3\cdot \vai[\last]{\bundlei[k+1]^{(k)}[1]}+\vai[\last]{\bundlei[k+1]^{(k)}[4]}\le11/9.$$
Suppose $3\cdot \vai[\last]{\bundlei[k+1]^{(k)}[1]}+\vai[\last]{\bundlei[k+1]^{(k)}[4]}>11/9$. Let $x$ be the value of $\vai[\last]{\bundlei[k+1]^{(k)}[4]}$. Then we have
\begin{align*}
11/9&<3\cdot \vai[\last]{\bundlei[k+1]^{(k)}[1]}+\vai[\last]{\bundlei[k+1]^{(k)}[4]}\\
&<3\cdot(5/9-x)+x \tag{by $U(\bundlei[k+1]^{(k)})<5/9$}
\end{align*}
This implies $x<2/9$. This contradicts our assumption that $c\in \larg{\last,2/9}$.

Notice that $\vai[\last]{\bundlei[k+1]^{(k)}[1]}$ is the value of largest chore among the remaining. So the inequality suggests that even if we allocate 3 largest chores, there is still a space for the chore $\bundlei[k+1]^{(k)}[4]$. So the first 3 chores being allocated to bundle  $\alloci[k+1]^*$ must be the largest 3 chores. So  $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$ for $j\le3$.

As we have $|\bundlei[k+1]^{(k)}|=4$, the chore $\bundlei[k+1]^{(k)}[4]$ would not be one of first 3 chores allocated to bundle  $\alloci[k+1]^*$. Since there is a space for  the chore $\bundlei[k+1]^{(k)}[4]$, the forth chore being allocated to bundle  $\alloci[k+1]^*$ should at least as large as  the chore $\bundlei[k+1]^{(k)}[4]$.  Combining all these, we have $|\alloci[k+1]^*|\ge 4$ and $\vai[\last]{\bundlei[k+1]^{(k)}[j]}\le\vai[\last]{\alloci[k+1]^*[j]}$ for $j\le4$.
\end{proof}


\begin{claim}\label{claim-two-one}
For the case $|\bundlei[k+1]^{(k)}|=3$ and Inequality \ref{ineq-2-3} does not hold, %$\vai[\last]{\alloci[k+1]^*[1]\cup\alloci[k+1]^*[2]\cup \bundlei[k+1]^{(k)}[3]}> 11/9$,
after all $SWAP$ and $MOVE$ operations, bundle $\bundlei[j]^{(k+1)}$ is good, where $j$ is the index such that the chore $\alloci[k+1]^*[2]\in\bundlei[j]^{(k)}$.
\end{claim}
\begin{proof}
%Suppose  bundle $\bundlei[j]^{(k)}$ contains the chore $\alloci[k+1]^*[2]$. We prove that if $\bundlei[j]^{(k)}$ is good, then after remove $\alloci[k+1]^*[2]$ and  then add $\bundlei[k+1]^{(k)}[2]$ and  $\bundlei[k+1]^{(k)}[3]$, $\bundlei[j]^{(k)}$ is good is still good.
We first prove two useful observations.
\begin{observation}\label{obser-2is-largest}
The chore $\alloci[k+1]^*[2]$ must be the largest chore in the bundle $\bundlei[j]^{(k)}$.

\begin{proof}
Because $|\bundlei[k+1]^{(k)}|=3$ and it is good, so $\vai[\last]{\bundlei[k+1]^{(k)}}\le1$, which means $\bundlei[k+1]^{(k)}[1]< 1-2/9-2/9=5/9$. This implies all remaining chores are less than $5/9$. Therefore, add the second largest chore, it is still less than $11/9$. We have  $\alloci[k+1]^*[2]$ must be the largest chore in the bundle $\bundlei[j]^{(k)}$.
\end{proof}
\end{observation}


\begin{observation}\label{obser-greater-4/9}
For the valuation of chore $\alloci[k+1]^*[2]$, we have  $\vai[\last]{\alloci[k+1]^*[2]}>4/9$.
\begin{proof}
As Inequality \ref{ineq-2-3} does not hold, we have
\begin{align*}
%\begin{split}
\vai[\last]{\left\{\alloci[k+1]^*[1],\alloci[k+1]^*[2], \bundlei[k+1]^{(k)}[3]\right\}}&> 11/9\\
&\ge2/9+\vai[\last]{\bundlei[k+1]^{(k)}}\\
&=2/9+\vai[\last]{\left\{\bundlei[k+1]^{(k)}[1],\bundlei[k+1]^{(k)}[2], \bundlei[k+1]^{(k)}[3]\right\}}
%\end{split}
\end{align*}
By the assumption that $\alloci[k+1]^*[1]=\bundlei[k+1]^{(k)}[1]$, we get $$\vai[\last]{\alloci[k+1]^*[2]}>2/9+\vai[\last]{\bundlei[k+1]^{(k)}[2]}>4/9.$$
\end{proof}

\end{observation}

Now we prove the statement by case analysis on the number of chores in the  bundle $\bundlei[j]^{(k)}$

For the case that bundle $\bundlei[j]^{(k)}$ only contains the chore $\alloci[k+1]^*[2]$ i.e. $|\bundlei[j]^{(k)}|=1$, it is easy to see bundle $\bundlei[j]^{(k+1)}$ is good after replacing the chore $\alloci[k+1]^*[2]$ with chores $\bundlei[k+1]^{(k)}[2]$ and $\bundlei[k+1]^{(k)}[3]$.

If bundle $\bundlei[j]^{(k)}$ contains two chores i.e. $|\bundlei[j]^{(k)}|=2$, we prove the valuation $\vai[\last]{\bundlei[j]^{(k+1)}}\le 1$. First we have following inequality
\begin{align*}
\vai[\last]{\left\{\bundlei[k+1]^{(k)}[2], \bundlei[k+1]^{(k)}[3]\right\}}&\le1-\vai[\last]{\bundlei[k+1]^{(k)}[1]}\\
&\le1-\vai[\last]{\alloci[k+1]^*[2]}.
\end{align*}
For the valuation of bundle $\bundlei[j]^{(k+1)}$, we have
\begin{align*}
\vai[\last]{\bundlei[j]^{(k+1)}}& = \vai[\last]{\left(\bundlei[j]^{(k)}\setminus \alloci[k+1]^*[2]\right)\bigcup\left(\left\{\bundlei[k+1]^{(k)}[2], \bundlei[k+1]^{(k)}[3]\right\}\right) }\\
&\le\vai[\last]{\alloci[k+1]^*[2]}+\vai[\last]{\left\{\bundlei[k+1]^{(k)}[2], \bundlei[k+1]^{(k)}[3]\right\}}\\
&\le \vai[\last]{\alloci[k+1]^*[2]}+1-\vai[\last]{\alloci[k+1]^*[2]}\\
&=1.
\end{align*}
The first inequality is due to the chore $\alloci[k+1]^*[2]$ is no less than the other chore in bundle $\bundlei[j]^{(k)}$. The second inequality is just follow the above inequality.
Thus, bundle $\bundlei[j]^{(k+1)}$ is  still good.

Now let us look at the case $|\bundlei[j]^{(k)}|=3$. Since bundle $\bundlei[j]^{(k)}$ is good, we have $\vai[\last]{\bundlei[j]^{(k)}}\le1$.  By Observation \ref{obser-greater-4/9}, we have  $\vai[\last]{\alloci[k+1]^*[2]}>4/9$.
Therefore, except the chore $\alloci[k+1]^*[2]$, the valuation of the remaining two chores in bundle $\bundlei[j]^{(k)}$ is $$\vai[\last]{\bundlei[j]^{(k)}\setminus \alloci[k+1]^*[2]}\le 1-\vai[\last]{\alloci[k+1]^*[2]}<5/9.$$
%,  the sum of remaining two in $\bundlei[j]^{(k)}$ is less than 5/9.
As the valuation $\vai[\last]{\bundlei[k+1]^{(k)}[1]}\ge\vai[\last]{\alloci[k+1]^*[2]}>4/9$ and bundle $\bundlei[k+1]^{(k)}$ is good,   we have $$\vai[\last]{\left\{\bundlei[k+1]^{(k)}[2], \bundlei[k+1]^{(k)}[3]\right\}}\le1-\vai[\last]{\bundlei[k+1]^{(k)}[1]}<5/9.$$
For the bundle $\bundlei[j]^{(k+1)}$, the largest chore is either in the set  $\bundlei[j]^{(k)}\setminus \alloci[k+1]^*[2]$ or in the set $\bundlei[k+1]^{(k)}[2]\cup \bundlei[k+1]^{(k)}[3].$ Therefore, the valuation $$U\left(\bundlei[j]^{(k+1)}\right)\le\max\left\{\vai[\last]{\bundlei[j]^{(k)}\setminus \alloci[k+1]^*[2]},\vai[\last]{\left\{\bundlei[k+1]^{(k)}[2],\bundlei[k+1]^{(k)}[3]\right\}}\right\}<5/9.$$
It is easy to see, in this case, the cardinality $|\bundlei[j]^{(k+1)}|=4$. Thus, bundle $\bundlei[j]^{(k+1)}$ is good.
%Let $\bundlei[j]^{(k)*}$ be the bundle after swapping. Combining these, we have $U(\bundlei[j]^{(k)*})<5/9$, which means it is still good.

It is impossible that $|\bundlei[j]^{(k)}|=4$. Since bundle $\bundlei[j]^{(k)}$ is good, if $|\bundlei[j]^{(k)}|=4$, then we have $U\left(\bundlei[j]^{(k)}\right)<5/9.$ As bundle $\bundlei[j]^{(k)}\subseteq \larg{\last,2/9}$, it implies that the valuation of the largest chore $$\vai[\last]{\alloci[k+1]^*[2]}=\vai[\last]{\bundlei[j]^{(k)}[1]}\le U\left(\bundlei[j]^{(k)}\right)-2/9<1/3.$$  This contradicts to  Observation \ref{obser-greater-4/9} i.e. $\vai[\last]{\alloci[k+1]^*[2]}>4/9$. So it is impossible.

\end{proof}


It is easy to see that, for a good bundle, if we replace one chore with a smaller chore, it is still good. The only case, which may increase the number of chores or increase the value of chores, is concluded in claim \ref{claim-two-one}. Thus we can keep this process to $\bundles^{(n)}$.
\end{proof}




















\begin{proof}
Let $\allocs$ be the allocation returned by Algorithm \ref{alg-poly}. And let bundle $\alloci^*=\alloci\cap \larg{\last, s_{\last}/4}$ consist of large chores from bundle $\alloci$. Let $D_k= \larg{\last, s_{\last}/4}\setminus\left( \cup_{i< k}\alloci^*\right)$ be the set of  large chores that have not been allocated in first $k-1$ rounds. Let $\bundlei$ be the bundle which is the $i$-th bundle generated by the threshold testing algorithm on input $s_{\last}$. Let chore set  $P_k=\cup_{i\ge k}\bundlei$. We will prove the following property which directly imply that no chore $c\in \larg{\last,s_{\last}/4}$ left.

\bigskip
{\bf Property $T$:} For each $k$, there exists an injective function $f_k:D_k\rightarrow P_k$ such that $\vai[\last]{c}\le \vai[\last]{f_k(c)}$ for all  $c\in D_k$.
\bigskip

When $k=n$, the property $T$ implies the total value of large chores in the last round is no grater than $\vai[\last]{\bundlei[n]}$, which is less than 5/4. Therefore, all large chores will be allocated. 

We will prove the property $T$ by induction. When $k=1$, the identical mapping will work. Now we prove that if the statement holds for $k$, then we can construct a suitable mapping for $k+1$. For this, it is sufficient to prove we can drop $\alloci[k]^*$ and $\bundlei[k]$ from the domain at the same time.

Here we introduce the swap operation for the function first. Given a function $f:D\rightarrow P$, chore $d\in D$ and chore $p\in P$, the operation $f^*=\text{Swap}(f,d,p)$ is defined as
\begin{equation*}
 f^*(c) =
  \begin{cases}
   f(c) & \text{for } c\neq d \text{ or } f^{-1}(p)  \\
   p       & \text{if } c=d  \\
   f(d)  & \text{if } c=f^{-1}(p)
  \end{cases}
\end{equation*}
 %$f^*(c)=f(c)$ for $\{c\in D_k\mid c\neq d \text{ and } c\neq f^{-1}(p)\}$
 Intuitively, this operation just swaps the mapping images of $d$ and $f^{-1}(p)$. If $f^{-1}(p)=\emptyset$, then this operation just change the image of $d$ to $p$.

Let $q=\min\{|\alloci[k]^*|,|\bundlei[k]|\}$. Let $g_0=f_k$ be a mapping function. For $1\le t\le q$, we iteratively construct mapping $$g_t=\text{Swap}(g_{t-1},\alloci[k]^*[t],\bundlei[k][t]).$$  Then let $f_{k+1}(c)=g_q(c)$ for all $c\in D_{k+1}$. Now we show that such construction will satisfy the condition in the statement.

\begin{claim}\label{claim-all-large}
For each $k$ and $1\le j<|\bundlei[k]|$, we have $\bundlei[k][j]=P_k[j]$ i.e. except the smallest chore in bundle $\bundlei[k]$, other chores are the largest chores in the remaining. 
\end{claim}
\begin{proof}
In threshold testing, the bundle is constructed in two stages. We first consider the bundle $\bundlei[k]$  is constructed before the for-loop in line \ref{inalg-after-big}. We have $|\bundlei[k]|\le 2$ and $\bundlei[k][1]=P_k[1]$.  So all bundles, which are constructed in this stage, satisfy the statement.

Now consider the bundle $\bundlei[k]$  is constructed in the for-loop of line \ref{inalg-after-big}. The bundle $\bundlei[k]$ is constructed by adding chores one by one from largest to smallest. Suppose that $j^*<|\bundlei[k]|$ is the first index that $\bundlei[k][j^*]\neq P_k[j^*]$. Notice that in this stage, for any chore $c$ we have $\frac{s_{\last}}{4}<\vai[\last]{c}\le \frac{s_{\last}}{2}.$  This implies  
\begin{align*}
\vai[\last]{\left\{\bundlei[k][j^*],\bundlei[k][j^*+1]\right\}}&>\frac{s_{\last}}{4}+\frac{s_{\last}}{4}\\
%&=\frac{s_{\last}}{2}\\
&>\vai[\last]{P_k[j^*]}.
\end{align*} 
So there is enough space for chore $P_k[j^*]$ to put into bundle $\bundlei[k]$. According to the threshold testing algorithm, chore $P_k[j^*]$ should be put into bundle $\bundlei[k]$
 %should be put into $\bundlei[k]$ and then $\bundlei[k][j^*]=P_k[j^*]$. 
 This is a contradiction. Therefore, we have $\bundlei[k][j]=P_k[j]$ for $1\le j<|\bundlei[k]|$.

 %Once we add one chore $c$ such that $\vai[\last]{c}<\vai[\last]{p}$ for some $p\in P_k\setminus\bundlei[k]$, then we cannot add another smaller chore $c'$. Otherwise, we have $\vai[\last]{c\cup c'}>\vai[\last]{p}$, which means the chore $p$ should be added into $\bundlei[k]$. Because there is enough space when algorithm considers to add $p$ into $\bundlei[k]$.
\end{proof}

 \begin{claim}\label{claim-not-bad}
 Recall that $q=\min\{|\alloci[k]^*|,|\bundlei[k]|\}$. For mapping $g_q$, we have $\vai[\last]{c}\le \vai[\last]{g_q(c)}$ for any chore $c\in D_k\setminus \alloci[k]^*$.
 \end{claim}
 \begin{proof}
We first prove that, for $1\le t<q$, the statement $$\forall c\in D_k, \vai[\last]{c}\le \vai[\last]{g_t(c)}$$ is true. We prove it by induction. Suppose the statement $\forall c\in D_k, \vai[\last]{c}\le \vai[\last]{g_{t-1}(c)}$ is true.
In each swap operation, we map chore $\alloci[k]^*[t]$ to chore $\bundlei[k][t]$ and chore $g_{t-1}^{-1}(\bundlei[k][t])$ to chore $g_{t-1}(\alloci[k]^*[t])$. 
%What happened to chore $\alloci[k]^*[t]$ does not influence the statement. It is sufficient to argue that $$\vai[\last]{g_{t-1}^{-1}(\bundlei[k][t])}\le \vai[\last]{g_{t-1}(\alloci[k]^*[t])}.$$
%If the 
%Recall   the construction of bundle $\alloci[k]$. When we allocate the  chore $\alloci[k]^*[t]$ to the bundle $\alloci[k]$, if there is enough space to allocate the chore $g_{t-1}^{-1}(\bundlei[k][t])$ but we 
 Since bundle $\alloci[k]^*\subseteq P_k$, by Claim \ref{claim-all-large}, we have $$\vai[\last]{\alloci[k]^*[t]}\le\vai[\last]{P_k[t]}= \vai[\last]{\bundlei[k][t]}.$$ 
 
 
Now we will prove $\vai[\last]{g_{t-1}^{-1}(\bundlei[k][t])}\le \vai[\last]{g_{t-1}(\alloci[k]^*[t])}$. If  chore $g_{t-1}^{-1}(\bundlei[k][t])=\alloci[k]^*[t]$, then this is the above case.  If chore $g_{t-1}^{-1}(\bundlei[k][t])\neq\alloci[k]^*[t])$, recall  the construction of bundle $\alloci[k]$. When we allocate the  chore $\alloci[k]^*[t]$ to the bundle $\alloci[k]$, if there is enough space to allocate the chore $g_{t-1}^{-1}(\bundlei[k][t])$ but algorithm does not do that, it means $$\vai[\last]{g_{t-1}^{-1}(\bundlei[k][t])}\le\vai[\last]{\alloci[k]}\le \vai[\last]{g_{t-1}(\alloci[k]^*[t])}.$$ So we only need to prove that there is enough space for chore $g_{t-1}^{-1}(\bundlei[k][t])$.
Notice that 
\begin{align*}
\vai[\last]{\left(\cup_{h<t}\alloci[k]^*[h]\right)\cup g_{t-1}^{-1}(\bundlei[k][t])}&\le\vai[\last]{\left(\cup_{h<t} g_{t-1}(\alloci[k]^*[h])\right)\cup \bundlei[k][t]}\\
&\le\vai[\last]{\cup_{h\le t}P_k[h]}\\
&=\vai[\last]{\cup_{h\le t}\bundlei[k][h]}\\
&<5/4
\end{align*}
The equality in the third line is by Claim \ref{claim-all-large}.   This means that there is enough space for chore $\bundlei[k][t]$ to be allocated when algorithm allocates the  chore $\alloci[k]^*[t]$ to the bundle $\alloci[k]$. As $\vai[\last]{g_{t-1}^{-1}(\bundlei[k][t])}\le\vai[\last]{\bundlei[k][t]}$, there is enough space for chore $g_{t-1}^{-1}(\bundlei[k][t])$. Therefore, we have $\vai[\last]{g_{t-1}^{-1}(\bundlei[k][t])}\le \vai[\last]{g_{t-1}(\alloci[k]^*[t])}$.


For $g_q$, what happened to chore $\alloci[k]^*[q]$ is not our concern.  We only need to argue that $$\vai[\last]{g_{t-1}^{-1}(\bundlei[k][q])}\le \vai[\last]{g_{t-1}(\alloci[k]^*[q])}.$$ The remaining proof is similar to the above case. Recall  the construction of bundle $\alloci[k]$, when we allocate the  chore $\alloci[k]^*[q]$ to the bundle $\alloci[k]$,  there is enough space to allocate the chore $g_{t-1}^{-1}(\bundlei[k][q])$. Because
\begin{align*}
\vai[\last]{\left(\cup_{h<q}\alloci[k]^*[h]\right)\cup g_{t-1}^{-1}(\bundlei[k][q])}&\le\vai[\last]{\left(\cup_{h<q} f_k(\alloci[k]^*[h])\right)\cup\bundlei[k][q]}\\
&\le\vai[\last]{\left(\cup_{h<q}P_k[h]\right)\cup\bundlei[k][q]}\\
&\le\vai[\last]{\bundlei[k]}\\
&<5/4
\end{align*}


%From the construction of bundle $\alloci[k]$, we could conclude that chore $\alloci[k]^*[h]=D_k[h]$ for $h<q$. This implies $\alloci[k]^*[t]$ is the $t$'th largest chore in set $D_k$.
%By the construction of mapping function, it is easy to see that $g_{t-1}(\alloci[k]^*[h])=\bundlei[k][h]$ for $h\le t-1$. Therefore, chore $g_{t-1}^{-1}(\bundlei[k][t])$ would not be chore $\alloci[k]^*[h]$ for any $h\le t-1$, which means  chore $g_{t-1}^{-1}(\bundlei[k][t])$ is not one of largest $t-1$ chores among set $D_k$.
%We have $$\vai[\last]{g_{t-1}^{-1}(\bundlei[k][t])}\le\vai[\last]{\alloci[k]^*[t]}\le \vai[\last]{g_{t-1}(\alloci[k]^*[t])}.$$



  %From the construction of bundle $\alloci[k]$, we have $\vai[\last]{g_{t-1}^{-1}(\bundlei[k][t])}\le\vai[\last]{\alloci[k]^*[t]}\le \vai[\last]{g_{t-1}(\alloci[k]^*[t])}$.
%By Claim \ref{claim-all-large}, we have $\vai[\last]{\alloci[k]^*[t]}\le \vai[\last]{\bundlei[k][t]}$ for $t<\min$
 \end{proof}

By Claim \ref{claim-not-bad}, we have $\vai[\last]{c}\le\vai[\last]{g_q(c)} $ for all $c\in D_{k+1}$. The remaining to prove is that $g_q(D_{k+1})\subseteq P_{k+1}$. So we have the following lemma.

\begin{claim}\label{claim-no-more}
If the cardinality $|\alloci[k]^*|<|\bundlei[k]|$, then for $|\alloci[k]^*|<j\le|\bundlei[k]|$, we have $g_q^{-1}(\bundlei[k][j])=\emptyset$.
\end{claim}
\begin{proof}
For the valuation of bundle $\alloci[k]^*$, we have
\begin{align*}
\vai[\last]{\alloci[k]^*}&\le \vai[\last]{\bigcup_{1\le t\le|\alloci[k]|}\bundlei[k][t]}\\
&\le \frac{11}{9}-\vai[\last]{\bundlei[k][j]}\\
&\le \frac{5}{4}-\vai[\last]{\bundlei[k][j]},
\end{align*}
where $|\alloci[k]^*|<j\le|\bundlei[k]|$. The first inequality is implied by Claim \ref{claim-all-large} and Claim \ref{claim-not-bad}. This means that if there is a chore mapping to  chore $\bundlei[k][j]$, then this chore can be added into $\alloci[k]^*$.
\end{proof}

By Claim \ref{claim-no-more} and the construction of mapping function $g_q$, we have $g_q(D_{k+1})\subseteq P_{k+1}$. And by Claim \ref{claim-not-bad}, we have $\vai[\last]{c}\le \vai[\last]{g_q(c)}$ for $c\in D_{k+1}$. Combining these, our construction of $f_{k+1}$ is valid.


\end{proof}
